Sur les corrections de la g\'eom\'etrie thermodynamique des trous noirs

We study thermodynamic geometry of certain black holes and black branes with and without generalized uncertainty principle or stringy $ \alpha^{\prime} $-corrections to the entropy. From this perspective, we analyze Ruppenier geometry of Reissner-Nordstr\"om black holes and show that it is well defined and corresponds to a non-interacting statistical system. We investigate that the Weinhold geometry of dilatonic black holes is regular everywhere and that of large mass Reissner-Nordstr\"om black holes in the Poincar\'e patch of $ AdS_4 $ contains certain narrow range of thermodynamically unstable regions in the statespace. We obtain that the generalized uncertainty principle corrected Ruppenier geometry of Reissner-Nordstr\"om black holes correspond to a non-interacting statistical system unlike the magnetically charged black holes. We show that the stringy $ \alpha^{\prime} $-corrections do not introduce singularity in the statespace geometry of non-supersymmetric extremal black holes in $ D= 4 $. Interestingly, the degree of scalar curvature and that of the determinant of this Ruppenier geometry can be written as an integer multiple of the order of $ \alpha^{\prime} $-correction. We further show that the statespace geometry of Gauss- Bonnet corrected supersymmetric extremal black holes in $ D=4 $ as well as non-extremal $D_1D_5$ and $D_2D_6NS_5$ black branes in $ D=10 $ is regular everywhere. Furthermore, the thermodynamic geometry of four dimensional rotating Kerr-Newman extremal black holes in Einstein-Maxwell theory is everywhere ill-defined and that of the Kaluza-Klein black holes in Einstein-Maxwell theory or the one arrising from heterotic string compactification is ill-defined only at the points of the ergo-branch.

==> blank2.tex <==
%\documentclass[a4paper,10pt]{article}
%\usepackage[utf8x]{inputenc}

%opening
%\title{}
%\author{}

%\begin{document}

%\maketitle

%\begin{abstract}

%\end{abstract}

%\section{}

\thispagestyle{plain}
\thispagestyle{empty}
\newpage  {\color{white} . }
%\end{document}


==> chap12.tex <==
\chapter{chap12}

\section{Les trous noirs dilatoniques}


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{diltopSS.ps}\vspace*{-3.0cm}
\caption{La composante $SS$ de la m\'etrique tenseure trac\'e comme la 
fonction de $Q, S$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs dilatonics.} \label{diltopSS}\vspace*{0.5cm}
\end{figure}

% The SS component of the metric tensor plotted as the
% function of $Q, S$, describing the fluctuations in the dilatonic black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{diltopQQ.ps}\vspace*{-3.0cm}
\caption{La composante $QQ$ de la m\'etrique tenseure trac\'e comme la 
fonction de $Q, S$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs dilatonics.} \label{diltopQQ}\vspace*{0.5cm}
\end{figure}

% The QQ component of the metric tensor plotted as the
% function of $Q, S$, describing the fluctuations in the dilatonic black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{diltopSQ.ps}\vspace*{-3.0cm}
\caption{La composante $SQ$ de la m\'etrique tenseure trac\'e comme la 
fonction de $Q, S $, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs dilatonics.} \label{diltopSQ}\vspace*{0.5cm}
\end{figure}

% The SQ component of the metric tensor plotted as the
% function of $Q, S$, describing the fluctuations in the dilatonic black hole configuration.

% For the value of $n=3$, $k=-1$, $b= 1$, $a= 2$and $L= -3$, the
%Figs.(\ref{diltopSS}, \ref{diltopQQ}) show the nature of
% the the components $\{g_{SS}, g_{QQ}\}$of the Wienhold metric
% tensor. In the regime of $Q \in (0,1)$and $S \in (0,1)$, we find
% that the amplitude of $\{g_{SS}\}$take the value of the order
% $2.5 \times 10^{+06}$. In this range of the $S, Q$, we observe that
% the component $\{ g_{QQ}\}$lies in the range of $(0, 1000)$.
% In this case, we see that the range of the growth of the amplitudes
% of $\{g_{SS}\}$and $\{g_{QQ}\}$remains in the same limit of $S$.
% Explicitly, the Figs.(\ref{diltopSS}, \ref{diltopQQ}) indicate that
% the growth of the first takes place in the limit of a small $S$.
% This signifies that the dilatonic black holes are thermodynamically
% unstable in the limit of small entropy. Similarly, the Fig.(\ref{diltopSQ})
% shows that the nature of $\{ g_{SQ}\}$component of the thermodynamic
% metric tensor. We find that the mix component $\{ g_{SQ}\}$takes a
% large value of order $-6000$in the limit of a large $Q$and small $S$.
% Thus, the heat compressibilities as depicted in the Figs.(\ref{diltopSS},
% \ref{diltopQQ}, \ref{diltopSQ}) illustrate the parametric fluctuation
% properties of the dilatonic black holes. Hereby, we notice that the
% self pair fluctuations involving $\{S, Q\}$, as defined by the metric
% tensor $\{g_{ij}\ |\ i, j= S, Q\}$, have positive numerical values,
% while the mix component $\{ g_{SQ}\}$does not.

Pour la valeur de $n=3$, $k=-1$, $b= 1$, $a= 2$ et $L= -3$, les Figs.
(\ref{diltopSS}, \ref{diltopQQ}) montrent la nature des composantes 
$\{g_{SS}, g_{QQ}\}$ de la m\'etrique tenseure de Wienhold. Dans le r\'egime 
de $Q \in (0,1)$ et $S \in (0,1)$, on trouve que l'amplitude de $\{g_{SS}\}$ 
prend la valeur \`a l'ordre de $2.5 \times 10^{+06}$. Dans cette gamme de 
$\{S, Q\}$, on observe que la composante $\{g_{QQ}\}$ se situe dans la gamme 
de $(0, 1000)$. Dans ce cas, nous voyons que la gamme de la croissance des amplitudes
de $\{g_{SS}\}$ et $\{g_{QQ}\}$ reste dans la m\^{e}me limite de $S$.
Explicitement, les Figs. (\ref{diltopSS}, \ref{diltopQQ}) indiquent que
la croissance de la premi\`ere composante est \`a lieu dans la limite d'une petite $S$.
Cela signifie que les trous noirs dilatonics sont thermodynamiquement instables 
dans la limite d'une petite \'entropie. Du fait m\^{e}me, la Fig. (\ref{diltopSQ})
montre que la nature de la composante $\{g_{SQ}\}$ de la m\'etrique tenseure thermodynamique. 
Nous constatons que la composante mixe $\{g_{SQ}\}$ prend une grande valeur \`a l'ordre 
de $-6000 $ dans la limite d'une grande $Q$ et une petite $S$. Ainsi, les compressibilit\'es 
de chaleurs, telle que repr\'esent\'ees dans les Figs. (\ref{diltopSS}, \ref{diltopQQ}, \ref{diltopSQ}) 
illustrent les propri\'et\'es param\'etrique des fluctuations de la configuration des trous noirs dilatonics. 
Par la pr\'esente, nous remarquons que les fluctuations d'auto-paires en impliquant $\{S, Q\}$, 
qui sont d\'efinies par la m\'etrique tenseure $\{g_{ii} \ | \ i = S, Q\}$, 
ont des valeurs num\'eriques positives, tandis que cela ne marche pas pour 
la composante mixe $\{g_{SQ}\}$. 


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{diltopdetg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, S $, en d\'ecrivant les fluctuations de la 
configuration des trous noirs dilatonics.} \label{diltopdetg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the
% function of $Q, S$, describing the fluctuations in the dilatonic 
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{diltopminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etriquetenseure trac\'ee comme la
fonction de $Q, S$, en d\'ecrivant les fluctuations de la 
configuration des trous noirs dilatonics.} \label{diltopminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $Q, S$, describing the fluctuations in the dilatonic 
% black hole configuration.


% At this juncture, we find that the ensemble stability of the
% dilatonic black holes can be determined in terms of the values
% of the parameters $S, Q$. This follows from the behavour of the
% determinant of thermodynamic metric tensor. In this case, we find
% that the determinant of the metric tensor tends to a negative value.
% For the case of $Q \in (0, 1)$and $S \in (0,1)$, the
% Fig.(\ref{diltopdetg}) shows that the determinant of the metric
% tensor lies in the interval $(0, -1.2 \times 10^{09})$. Notice
% that the negativity of $g$increases as the value of $Q$is
% increased from zero to $1$. Also, the surface defined by
% the fluctuations of $(S,Q)$is unstable because of a negative
% value of the corresponding determinant of the metric tensor.
% When only the parameter $S$is allowed to vary, thestability
% of the dilatonic black hole configuration is determined by the
% positivity of the first principle minor $p_1:= g_{SS}$. A rotated
% view of $p_1$is shown in the Fig.(\ref{diltopminor1}). Hereby,
% for a small value of $S$, we see that $p_1$increases as the function
% of the electric charge $Q$. The above mentioned graphical properties and 
% the positivity of the principle minors provide the qualitative notion 
% of the statistical stability of two parameter dilatonic black holes.

\`A ce stade, nous constatons que la stabilit\'e d'un ensemble des 
trous noirs dilatonics peut \^{e}tre d\'etermin\'e en termes des valeurs
de param\`etres $\{S, Q\}$. Cela d\'ecoule du comportement de d\'eterminant 
de la m\'etrique tenseure thermodynamique. Dans ce cas, nous trouvons que 
le d\'eterminant de la m\'etrique tenseure tend vers une valeure n\'egative.
Pour le cas de $Q \in (0, 1)$ et $S \in (0, 1)$, la Fig.(\ref{diltopdetg}) 
montre que le d\'eterminant de la m\'etrique tenseure r\'eside dans l'intervalle 
$(-1.2 \times 10^{09}, 0)$. Avis que la n\'egativit\'e de $g$ augmente \`a mesure 
que la valeur de $Q$ est augment\'e, en passant de z\'ero \`a $1$. En outre, 
la surface d\'efinie par les fluctuations de $(S, Q)$ est instable en raison d'une 
valeur n\'egative du d\'eterminant de la m\'etrique tenseure correspondante. 
Lorsque seul le param\`etre $S$ est autoris\'e \`a varier, la stabilit\'e des 
configurations trous noirs dilatonics est d\'etermin\'e par la positivit\'e du 
premier mineur principe $p_1: = g_{SS}$. Une vue rotat\'ee de $p_1$ est montr\'e 
dans la Fig. (\ref{diltopminor1}). Par la pr\'esente, pour une petite valeur de $S$, 
nous voyons que $p_1$ augmente \'a mesure que la fonction de la charge \'electrique $Q$. 
Les propri\'et\'es graphiques, mentionn\'ees ci-dessus, et la positivit\'e des mineurs 
principaux fournent la notion qualitative de la stabilit\'e statistiqu des trous noirs 
dilatonics de deux param\`etres $\{S, Q\}$.



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{diltopcur.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee en fonction de $Q, S$,
d\'ecrivant les variations dans la configuration des trous noirs dilatonics
dans la gamme $S, Q \in (0,1) $.} \label{diltopcur}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, S$, 
% describing the fluctuations in the dilatonic black hole configuration
% in the range $S, Q \in (0,1)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{diltopcur2.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee en fonction de $Q, S$,
d\'ecrivant les variations dans la configuration des trous noirs dilatonics
dans la gamme $S, Q \in (-2, 2)$.} \label{diltopcur2}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, M$, 
% describing the fluctuations in the dilatonic black hole configuration
% in the range $S, Q \in (-2, 2)$.

% The global stability properties of the dilatonic black holes
% follows from the behaviour of the thermodynamic scalar curvature.
% In particular, in the range of $S \in (0,1)$and $Q \in (0,1)$,
% the Fig.(\ref{diltopcur}) shows that the scalar curvature has
% a large positive amplitude of order $300000$. This shows that
% the underlying black hole configuration is a strongly interacting
% statistical system. The positive sign of the scalar curvature
% signifies a repulsive nature of the statistical interactions.
% The Fig.(\ref{diltopcur2}) signifies the nature of the above
% % scalar curvature in an equal range of the parameters $S,
% Q \in (-2,2)$. In this case, we notice from the Fig.(\ref{diltopcur2})
% that there exists many regions of global statistical interactions.
% In comparison with the interactions appearing in the range of $S, Q \in
% (-2,2)$, the amplitude of the global statistical interactions
% appears to be much smaller than those appearing in the range
% of $S, Q \in (0,1)$. Further, we see that the typical value
% of the ratio of the state-space scalar curvatures appears is
% of order $150$. In short, the aboveindicate that the
% dilatonic black holes are unstable statistical configurations
% when both the parameter $\{S, Q\}$are allowed to fluctuate.

Les propri\'et\'es de la stabilit\'e globale des trous noirs dilatonics
d\'ecoulent par le comportement de la courbure scalaire thermodynamique.
En particulier, dans la gamme de $S \in (0,1) $ et $Q \in (0,1)$, la
Fig. (\ref{diltopcur}) montre que la courbure scalaire a une grande 
amplitude positive \`a l'ordre de $300 000 $. Cela montre que la configuration 
sous-jacente de ces trous noirs est un syst\`eme statistique fortement r\'epulsif. 
Le signe positif de la courbure scalaire signifie la nature r\'epulsive 
des interactions statistiques. La Fig. (\ref{diltopcur2}) signifie 
la nature de ce qui pr\'ec\`ede de la courbure scalaire dans une range 
\'egale des param\`etres $S, Q \in (-2, 2)$. Dans ce cas, nous remarquons 
de la Fig. (\ref{diltopcur2}) qu'il existe des nombreuses r\'egions globale 
des interactions statistiques. En comparaison des interactions apparaissant 
dans la gamme de $S, Q \in (-2, 2) $, l'amplitude des interactions statistiques 
globales semble \^{e}tre beaucoup plus petites que cele qui figure dans la gamme de 
$S, Q \in (0, 1) $. De plus, nous voyons que la valeur typique du ratio des courbures 
scalaires de l'espace des \'etats qui appara\^{i}t est \`a l'ordre de $150 $. 
En bref, les chiffres ci-dessus indiquent que les trous noirs dilatonics correspondent 
\`a une configuration statistique instable, lorsque les deux param\`etres $\{S, Q\}$ 
sont autoris\'es \`a fluctuer.


\section{Les trous noirs de RN-AdS4}



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4SS.ps}\vspace*{-3.0cm}
\caption{La composante $SS $ de la m\'etrique tenseure trac\'ee en 
fonction de $Q, M $, en d\'ecrivant les fluctuations dans la configuration 
des trous noirs RN-$AdS_4$.} \label{RNADS4SS}\vspace*{0.5cm}
\end{figure}

% The $SS$component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4Q1Q1.ps}\vspace*{-3.0cm}
\caption{La composante $Q_1Q_1$ de la m\'etrique tenseure trac\'ee en 
fonction de $Q, M $, en d\'ecrivant les fluctuations dans la configuration 
des trous noirs RN-$AdS_4$.} \label{RNADS4Q1Q1}\vspace*{0.5cm}
\end{figure}

% The $Q_1Q_1$component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$ 
% black hole configuration.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4Q2Q2.ps}\vspace*{-3.0cm}
\caption{La composante $Q_2Q_2$ de la m\'etrique tenseure trac\'ee en 
fonction de $Q, M $, en d\'ecrivant les fluctuations dans la configuration 
des trous noirs RN-$AdS_4$.} \label{RNADS4Q2Q2}\vspace*{0.5cm}
\end{figure}

% The $Q_2Q_2$ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$
% black hole configuration.



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4SQ1.ps}\vspace*{-3.0cm}
\caption{La composante $SQ_1$ de la m\'etrique tenseure trac\'ee en 
fonction de $Q, M $, en d\'ecrivant les fluctuations dans la configuration 
des trous noirs RN-$AdS_4$.} \label{RNADS4SQ1}\vspace*{0.5cm}
\end{figure}

% The $SQ_1$ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4SQ2.ps}\vspace*{-3.0cm}
\caption{La composante $SQ_2$ de la m\'etrique tenseure trac\'ee en 
fonction de $Q, M $, en d\'ecrivant les fluctuations dans la configuration 
des trous noirs RN-$AdS_4$.} \label{RNADS4SQ2}\vspace*{0.5cm}
\end{figure}

% The $SQ_2$ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$ 
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4Q1Q2.ps}\vspace*{-3.0cm}
\caption{La composante $Q_1Q_2$ de la m\'etrique tenseure trac\'ee en 
fonction de $Q, M $, en d\'ecrivant les fluctuations dans la configuration 
des trous noirs RN-$AdS_4$.} \label{RNADS4Q1Q2}\vspace*{0.5cm}
\end{figure}

% The $Q_1Q_2$ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$
% black hole configuration.


% For $L= -3$, $Q_1= Q$and $Q_2= Q$, we find in the range of $Q \in
% (0,1)$and $S \in (0,1)$that the component $\{g_{SS}\}$takes a
% maximum value of the order $1600$. While, the components $\{
% g_{Q_1 Q_1}, g_{Q_2 Q_2}\}$take a typical value between the
% interval $(0,4)$. This shows that the RN-$AdS_4$black holes are
% locally stable statistical configurations. In fact, the range of
% the growth of $\{g_{SS}\}$and $\{ g_{Q_1 Q_1}, g_{Q_2 Q_2}\}$
% happens to be in the opposite limit of the parameters $\{S, Q\}$.
% Explicitly, from the Figs.(\ref{RNADS4SS}, \ref{RNADS4Q1Q1},
% \ref{RNADS4Q2Q2}), we observe that that the of growth of the $
% g_{SS}$takes place in the limit of a large $Q$and small $S$. On
% the other hand, the Figs.(\ref{RNADS4Q1Q1}, \ref{RNADS4Q2Q2})
% show that the growth of $\{ g_{Q_1Q_1}, g_{Q_2 Q_2}\}$takes
% place in the limit of small $Q$and small $S$. Similarly, the heat
% compressibilities involving two distinct parameters of the
% RN-$AdS_4$black hole have been depicted in the
% Figs.(\ref{RNADS4SQ1}, \ref{RNADS4SQ2}, \ref{RNADS4Q1Q2}). In this
% case, we notice that the Fig. \ref{RNADS4Q1Q2} shows an unique
% feature of $Q_1 Q_2$-component of the thermodynamic fluctuations.
% for a given RN-$AdS_4$black holes, the components of the metric
% tensor $\{g_{ij}\ |\ i, j= S, Q_1, Q_2\}$indicate that the
% fluctuations involving the charges $\{Q_1, Q_2\}$have relatively
% positive numerical values with respect to those involving the
% entropy $S$of the black hole.

Pour $L = -3$, $Q_1 = Q$ et $Q_2 = Q$, on retrouve dans la gamme de $Q \in
(0,1) $ et $S \in (0,1)$ que la composante $\{g_{SS}\}$ prend une valeur 
maximale \`a l'ordre de $1600 $. Alors, les composantes $\{ g_{Q_1 Q_1}, g_{Q_2 Q_2}\}$ 
prendent une valeur typique dans l'intervalle $(0,4) $. Cela montre que 
les trous noirs RN-$AdS_4$ correspondent localement \`a une configuration 
statistique stable. En fait, la gamme de la croissance de $\{g_{SS}\}$ et 
$\{g_{Q_1 Q_1}, g_{Q_2 Q_2}\}$ se trouve \^{e}tre \`a la limite oppos\'ee 
des param\`etres $\{S, Q\}$. Explicitement, par les Figs. (\ref{RNADS4SS}, 
\ref{RNADS4Q1Q1}, \ref{RNADS4Q2Q2}), on observe que la croissance de
$g_{SS}$ est a lieu dans la limite d'une grande $Q$ et d'une petite $S$. 
D'autre part, les Figs. (\ref{RNADS4Q1Q1}, \ref{RNADS4Q2Q2})
montrent que la croissance de $\{g_{Q_1Q_1}, g_{Q_2 Q_2}\}$ est plac\'ee
dans la limite d'une petite $Q$ et une petite $S$. Du fait m\^{e}me, les 
compressibilit\'es de chaleurs en impliquant deux param\`etres distincts 
de la configuration des trous noirs de RN-$AdS_4$ ont \'et\'e repr\'esent\'es 
par les Fig. (\ref{RNADS4SQ1}, \ref{RNADS4SQ2}, \ref{RNADS4Q1Q2}). Dans ce
cas, nous remarquons que la Fig. (\ref{RNADS4Q1Q2}) montre une caract\'eristique 
unique de la composante $Q_1Q_2$ des fluctuations thermodynamiques.
Pour des trous noirs RN-$AdS_4$ donn\'es, les composantes de la m\'etrique
tenseure $\{g_{ij} \ | \ i, j = S, Q_1, Q_2\}$ indiquent que ces fluctuations 
en impliquant des charges $\{Q_1, Q_2\}$ prennent relativement des valeurs 
num\'eriques positives \`a l'\'egard de ceux en impliquant l'entropie $S$ 
des trous noirs de RN-$AdS_4$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4det.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs RN-$AdS_4$.} \label{RNADS4det}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$ 
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4minor.ps}\vspace*{-3.0cm}
\caption{Le mineur de surface de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs RN-$AdS_4$.} \label{RNADS4minor}\vspace*{0.5cm}
\end{figure}

% The surface minor of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$ 
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4minor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs RN-$AdS_4$.} \label{RNADS4minor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN-$AdS_4$ 
% black hole configuration.

% As the function of $S, Q$, the ensemble stability condition of
% RN-$AdS_4$black holes follows from the positivity of the
% determinant of the metric tensor. In this case, we find that the
% determinant of the metric tensor generically tends to a negative
% value. For a typical value of $S \in (0,1)$and $Q \in (0,1)$, the
% Fig.(\ref{RNADS4det}) shows that the determinant of the metric
% tensor lies in the interval $(0,-12000)$. Hereby, for a small $S$,
% we observe that the determinant of the metric tensor has an
% approximate value of $-12000$. In the limit of a large $Q$, the
% determinant of the metric tensor firstly remains to a nearly
% constant small value and then, in the limit of small $S$, it
% increases sharply to a large negative value of order $-12000$. The
% corresponding stability of the surface defined by a constant value
% of the charge is shown in the Fig.(\ref{RNADS4minor}). In this
% range of $S, Q$, we see that the minor $p_2$lies in the range of
% $(-2500, 0)$. In the limit of a small $S$, we find that the
% negativity of $p_3$increases as the value of $Q$is increased
% from zero to $1$. When $S$is only the parameter which is allowed
% to vary, the stability of the configuration is determined by the
% positivity of the first principle minor $p_1:= g_{SS}$. In this
% case, we observe from the Fig.(\ref{RNADS4minor1}) that $p_1$has
% a positive amplitude of the order $2000$. In fact, for a small
% value of $S$, thefirst principle minor $p_1$increases
% continuously as the function of the charge $Q$. Thus, the above
% graphical descriptions of the principle minors provide qualitative
% notion of the stability of the RN-$ADS_4$black holes.

Comme une fonction de $\{S, Q\}$, la condition de la stabilit\'e d'un ensemble 
des trous noirs de RN-$AdS_4$ d\'ecoule par la positivit\'e du d\'eterminant 
de la m\'etrique tenseure. Dans ce cas, nous constatons que le d\'eterminant 
de la m\'etrique tenseure g\'en\'eriquement tend vers une valeur n\'egative. 
Pour une valeur typique de $S \in (0, 1)$ et $Q \in (0, 1) $, la Fig. 
(\ref{RNADS4det}) montre que le d\'eterminant de la m\'etrique tenseure 
r\'eside dans l'intervalle $(0, -12 000)$. Donc, pour une petite $S$,
nous observons que le d\'eterminant de la m\'etrique tenseure a une valeur 
approximative \`a l'ordre de $-12000$. Dans la limite d'une grande $Q$, 
le d\'eterminant de la m\'etrique reste tout d'abord \`a pr\`es d'une constante 
valeur petite, puis, dans la limite de la petite $S$, il augmente brusquement \`a 
une grande valeur n\'egative \`a l'ordre de $-12000 $. La stabilit\'e correspondante 
de la surface d\'efinie par une valeur constante de la charge $Q_2$ est montr\'e 
dans la Fig. (\ref{RNADS4minor}). Dans cette gamme de $\{S, Q\}$, nous voyons que le 
mineur principe $p_2 $ r\'eside dans la gamme de $(-2500, 0)$. Dans la limite d'une petite $S$, 
nous constatons que la n\'egativit\'e de $p_2$ augmente \`a la mesure que la valeur de 
$Q$ est augment\'e de z\'ero \`a $1$. Lorsque $S$ est le seul param\`etre qui est permis
de varier, la stabilit\'e de la configuration sous-jacente est d\'etermin\'ee par la
positivit\'e du premier mineur principe $p_1: = g_{SS} $. Dans ce cas, nous observons 
de la Fig. (\ref{RNADS4minor1}) que $p_1$ a une amplitude positive \`a l'ordre de $2000$. 
En fait, pour une petite valeur de $S$, le premier mineur principe $p_1$ augmente 
continuousement comme la fonction de la charge $Q$. Ainsi, les descriptions graphiques 
ci-dessus des mineurs principaux fournent la notion qualitative de la stabilit\'e 
statistique des trous noirs de RN-$ADS_4$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4cur.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee en fonction de $Q, M $,
d\'ecrivant les variations dans la configuration des trous noirs
RN-$AdS_4$ dans la gamme $S, Q \in (0,1) $.} \label{RNADS4cur}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, M$, 
% describing the fluctuations in the RN-$AdS_4$black hole configuration
% in the range $S, Q \in (0,1)$.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNADS4cur2.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee en fonction de $Q, M $,
d\'ecrivant les variations dans la configuration des trous noirs
RN-$AdS_4$ dans la gamme $S, Q \in (-2, 2)$.} \label{RNADS4cur2}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, M$, 
% describing the fluctuations in the RN-$AdS_4$black hole configuration
% in the range $S, Q \in (-2, 2)$.

% Under fluctuation of the charges $\{Q_1, Q_2\}$and entropy $S$,
% the global stability properties of the RN-$AdS_4$black holes are
% shown in the Figs. (\ref{RNADS4cur}, \ref{RNADS4cur2}). In the
% range of $S \in (0,1)$and $Q \in (0,1)$, it follows from the
% Figs. (\ref{RNADS4cur}) that the Winhold scalar curvature acquires
% a large positive peak. In fact,in the limit of small $Q$, the
% Figs. (\ref{RNADS4cur}) shows that the scalar curvature has
% certain highly interacting domain. In particular, in the small
% value of $Q$, the Fig.(\ref{RNADS4cur}) shows that the scalar
% curvature has a large positive amplitude of the order $800000$.
% Thus, we may note that the underlying black hole configuration is
% a strongly interacting statistical system in this limit of the
% charges and entropy. As mentioned in the case of he dilatonic
% black holes, the fluctuations of the charges and entropy yield the
% positive sign to the scalar curvature. This signifies that the
% RN-$ADS_4$black holes are repulsive in their nature. The
% Fig.(\ref{RNADS4cur2}) describes the nature of the Wienhold scalar
% curvature in an equal range of the parameters $S, Q \in (-2, 2)$.
% Namely, we see from the Fig.(\ref{RNADS4cur2}) that there is a
% half cut negative amplitude peak of the global interactions. In
% comparison with the interactions appearing in the range of $S \in
% (0,1)$and $Q \in (0,1)$, the interactions change their nature and
% they become rather attractive in the range of $S, Q \in (-2,2)$.
% The typical value of the amplitude of the corresponding scalar
% curvatures appears to be of the order $-2 \times 10^{+13}$. The
% graphical properties of the comparison follows from the Figs.
% (\ref{RNADS4cur}, \ref{RNADS4cur2}). Qualitatively, the above
% graphical depictions of the scalar curvatures indicate that the
% RN-$ADS_4$black holes are unstable configurations in the small
% change limit. As expected, we find that RN-$ADS_4$black holes are
% well-behaved, weakly interacting and relatively stable
% configurations in the large charge limit.

Sous la fluctuation des charges $\{Q_1, Q_2\}$ et de l'entropie $S$,
les propri\'et\'es de la stabilit\'e globale des trous noirs de RN-$AdS_4$
sont montr\'ees dans les Figs. (\ref{RNADS4cur}, \ref{RNADS4cur2}). 
Dans la gamme de $S \in (0, 1)$ et $Q \in (0, 1) $, il r\'esulte de la
Fig. (\ref{RNADS4cur}) que la courbure scalaire de Winhold acquiert
un grand pic positif. En fait, dans la limite d'une petite $Q$, la
Fig. (\ref{RNADS4cur}) montre que la courbure scalaire a certaines domaines
tr\`es interagissantes. En particulier, dans une petite valeur de $Q$, 
la Fig. (\ref{RNADS4cur}) montre que la courbure scalaire de Winhold a une 
grande amplitude positive \`a l'ordre de $800 000 $. Ainsi, on peut noter que 
la configuration des trous noirs sous-jacente est un syst\`eme statistiques 
interagissant fortement, dans cette limite des charges et de l'entropie. 
Comme mentionn\'e dans le cas de celle des trous noirs dilatonics, 
les fluctuations des charges et de l'entropie rendent un signe positif 
\`a la courbure scalaire. Cela signifie que les trous noirs de RN-$ADS_4$ 
sont r\'epulsive dans la leur nature. La Fig. (\ref{RNADS4cur2}) d\'ecrit 
la nature de la courbure scalaire de Wienhold dans une range \'egale des 
param\`etres $S, Q \in (-2, 2) $. Notamment, nous voyons de la Fig. (\ref{RNADS4cur2}) 
qu'il y a une moiti\'e coup\'ee pique n\'egative de l'amplitude des interactions globales. 
\`A la comparaison avec des interactions apparaissant dans la gamme de $S \in
(0, 1)$ et $Q \in (0, 1) $, les interactions changent leurs natures et ainsi
ces trous noirs deviennent plut\^{o}t attractifs dans la gamme de $S, Q \in (-2, 2)$.
La valeur typique de l'amplitude des courbures scalaires correspondantes  
semble \^{e}tre \`a l'ordre de $-2\times 10^{13} $. Les propri\'et\'es 
graphiques de cette comparaison suivent des Figs. (\ref{RNADS4cur}, \ref{RNADS4cur2}). 
Qualitativement, les repr\'esentations graphiques ci-dessus des courbures scalaires 
indiquent que les trous noirs de RN-$ADS_4$ sont des configurations instables dans 
la limite des petites param\'etres. Comme pr\'evu, nous constatons que les 
trous noirs de RN-$ADS_4$ sont bien comport\'es, faiblement interactifs, et 
ainsi il s'av\`ere que ces trous noirs correspondent \`a une configuration 
relativement stable dans la limite des grandes charges.


\section{Les corrections de $l_P $}


\subsection{RN GUP}

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNgupMM.ps}\vspace*{-3.0cm}
\caption{La composante $MM$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la 
configuration des trous noirs de RN.} \label{RNgupMM}\vspace*{0.5cm}
\end{figure}

% The MM component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN 
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNgupQQ.ps}\vspace*{-3.0cm}
\caption{La composante $QQ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la 
configuration des trous noirs de RN.} \label{RNgupQQ}\vspace*{0.5cm}
\end{figure}

% The QQ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN 
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNgupMQ.ps}\vspace*{-3.0cm}
\caption{La composante $MQ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la 
configuration des trous noirs de RN.} \label{RNgupMQ}\vspace*{0.5cm}
\end{figure}

% The MQ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN 
% black hole configuration.

% For $L=0.01$, theFigs.(\ref{RNgupMM}, \ref{RNgupQQ}) show
% the nature of the the heat capacities $\{g_{MM}, g_{QQ}\}$of the
% state-space metric tensor. In the regime of $M \in (0,1)$and $Q
% \in (-1,2)$, we observe that the amplitude of $\{g_{MM}\}$takes
% a value of the order $10^{+15}$. In this range of the parameters
% $\{M, Q\}$, we find that the component $\{ g_{MM}\}$lies in the
% range of $(-5 \times 10^{+15}, 0)$. In this case, we see that the
% range of the growth of the amplitude of $\{g_{QQ}\}$remains
% almost in the same limit of $\{Q, M\}$. Explicitly, this signifies
% that the RN black holes are thermodynamically unstable in the
% limit of small charge and mass. Similarly, the Fig.(\ref{RNgupMQ})
% shows that the nature of $\{ g_{MQ}\}$ component of the
% state-space metric tensor. We find that the mix component $\{
% g_{MQ}\}$takes a large value of order $\pm 10^{+15}$in the limit
% of a small $Q$and small $M$. In this limit of $\{M, Q\}$, the
% heat compressibilities as depicted in the Figs.(\ref{RNgupMM},
% \ref{RNgupQQ}, \ref{RNgupMQ}) illustrate the fluctuation
% properties of the RN black holes. In short, the self pair
% fluctuations involving $\{M, Q\}$, as defined by the metric tensor
% $\{g_{ij}\ |\ i, j= M, Q\}$, have positive numerical values,
% while the mix component $\{ g_{MQ}\}$has the both signatures.

Pour $L = 0.01 $, les Figs. (\ref{RNgupMM}, \ref{RNgupQQ}) montrent
la nature des capacit\'es de chaleurs $\{g_{MM}, g_{QQ}\}$ de la m\'etrique
tenseure de l'espace des \'etats. Dans le r\'egime de $M \in (0, 1)$ et 
$Q \in (-1, 2) $, on observe que l'amplitude de $\{g_{MM}\}$ prend
une valeur \`a l'ordre de $10^{+15} $. Dans cette gamme des param\`etres
$\{M, Q\}$, nous constatons que la composante $\{g_{MM}\}$ r\'eside dans la
gamme de $(-5 \times 10^{+15}, 0)$. Dans ce cas, nous voyons que la
gamme de la croissance de l'amplitude de $\{g_{QQ}\}$ reste presque dans 
la m\^{e}me limite de $\{Q, M\}$. Explicitement, cela signifie que 
les trous noirs de RN sont thermodynamiquement instables dans la
limite de petite charge et de petite masse. Du fait m\^{e}me, la Fig. (\ref{RNgupMQ})
montre que la nature de la composante $\{g_{MQ}\}$ de la m\'etrique tenseure
de l'\'espace des \'etats. Nous constatons que la composante mixe $\{g_{MQ}\}$ 
prend une grande valeur \`a l'ordre de $\pm 10^{+15}$ dans la limite
d'une petite $Q$ et une petite $M$. Dans cette limite de $\{M, Q\}$, 
les compressibilit\'es de chaleurs, telle que repr\'esent\'ee dans les
Figs. (\ref{RNgupMM}, \ref{RNgupQQ}, \ref{RNgupMQ}) illustrent 
les propri\'et\'es de la fluctuation des trous noirs de RN. En bref, 
les paires pures des fluctuations en impliquant $\{M, Q\}$, tel que 
d\'efinies par la m\'etrique tenseure $\{g_{ii} \ | \ i = M, Q\}$, 
ont des valeurs num\'eriques positives, tandis que la composante mixe 
$\{g_{MQ}\}$ prend les deux signatures.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNgupdet.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee 
comme la fonction de $Q, M$, en d\'ecrivant les fluctuations de la 
configuration des trous noirs de RN.} \label{RNgupdet} \vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN 
% black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{RNgupminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la configuration 
des trous noirs de RN.} \label{RNgupminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the RN 
% black hole configuration.


% Notice that the ensemble stability of the RN black holes can be
% determined in terms of the values of the mass and charge $M, Q$.
% This follows from the behavour of the determinant of state-space
% metric tensor. In this case, we find that the determinant of the
% metric tensor tends to a large negative value. For the case of $M
% \in (0,1)$and $Q \in (-1,2)$, the Fig.(\ref{RNgupdet}) shows that
% the determinant of the metric tensor lies in the interval $(0, -6
% \times 10^{17})$. In fact, we find that the negativity of $g$
% increases as the values of $Q, M$ are increased from $1$ to zero.
% Thus, the surface defined by the fluctuations of $\{M, Q\}$ is
% unstable because of a negative value of the determinant of the
% metric tensor. When only the parameter $M$is allowed to vary, the
% stability of the RN black hole configuration is determined by the
% positivity of the first principle minor $p_1:= g_{MM}$. A rotated
% view of the $p_1$is shown in the Fig.(\ref{RNgupminor1}). The
% above graphical properties and positivity of the state-space
% quantities provide the qualitative notion of the statistical
% stability of two parameter RN black holes under the generalized
% uncertainty principle corrections.

Notez bien que la stabilit\'e d'un ensemble des trous noirs de RN peut \^{e}tre
d\'etermin\'e en termes des valeurs de la masse $M$ et de la charge $Q$.
Cela d\'ecoule du comportement de d\'eterminant de la m\'etrique tenseure
de l'espace des \'etats. Dans ce cas, nous constatons que le d\'eterminant 
de la m\'etrique tenseure tend vers une grande valeur n\'egative. Pour le cas 
de $M \in (0, 1)$ et $Q \in (-1, 2)$, la Fig. (\ref{RNgupdet}) montre que
le d\'eterminant de la m\'etrique tenseure r\'eside dans l'intervalle 
$(-6 \times 10^{+17}, 0)$. En fait, nous constatons que la n\'egativit\'e 
de $g$ augmente \`a mesure que les valeurs de $Q, M$ sont vari\'ees de 
$1$ \`a z\'ero. Ainsi, la surface d\'efinie par les fluctuations de $\{M, Q\}$ 
est instables en raison d'une valeur n\'egative du d\'eterminant de la
m\'etrique tenseure. Lorsque le seul param\`etre $M$ est autoris\'e \`a varier, 
la stabilit\'e de la configuration des trous noirs de RN est d\'etermin\'e par 
la positivit\'e du premier mineur principe $p_1: = g_{MM}$. Une vue rotat\'ee 
de $p_1$ est montr\'ee dans la Fig. (\ref{RNgupminor1}). Ci-dessus, 
les propri\'et\'es graphiques et la positivit\'e des mineurs principaux,
comme les quantit\'es de l'espace des \'etats fournent la notion qualitative 
de la stabilit\'e statistique des trous noirs de RN de deux param\`etres 
sous les corrections du principe d'incertitude g\'en\'eralis\'e.

% The global stability properties of the RN black holes follows from
% the state-space scalar curvature. In general, it turns out that
% the scalar curvature vanishes identically for all values of the
% mass and charge. This shows that the generalized uncertainty
% principle corrected RN black holes correspond to a noninteracting
% statistical configurations. In short, the above observations of
% the state-space geometry indicates that the RN black holes are
% although noninteracting but unstable statistical configurations
% when the parameter $\{M, Q\}$are allowed to fluctuate. It is
% worth mentioning that the instability survives even at the local
% level of the heat capacities.

Les propri\'et\'es globales de la stabilit\'e des trous noirs de RN 
d\'ecoulent de la courbure scalaire de l'espace des \'etats. En g\'en\'eral, 
il s'av\`ere que la courbure scalaire est identiquement nulle pour toute 
valeur de la masse et de la charge. Cela montre que les trous noirs de RN 
sous les corrections du principe d'incertitude g\'en\'eralis\'ee correspondent 
\`a une configuration statistique non-interagissante. En bref, les observations 
ci-dessus de la g\'eom\'etrie de l'espace des \'etats indiquent que les trous noirs 
de RN sont, bien que non-interagissants, mais correspondent \`a une configuration 
statistiquement instable, lorsque les param\`etres $\{M, Q\}$ sont autoris\'es \`a fluctuer. 
Il est convient de mentionner que l'instabilit\'e survit m\^{e}me \`a l'\'echelle 
locale au niveau des capacit\'es de chaleurs.


\subsection{Magnetic GUP}


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{maggupMM.ps}\vspace*{-3.0cm}
\caption{La composante $MM$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la configuration 
des trous noirs charg\'ee magn\'etiquement.} \label{maggupMM}\vspace*{0.5cm}
\end{figure}

% The MM component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the 
% magnetically charged black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{maggupQQ.ps}\vspace*{-3.0cm}
\caption{La composante $QQ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la configuration 
des trous noirs charg\'ee magn\'etiquement.} \label{maggupQQ}\vspace*{0.5cm}
\end{figure}

% The QQ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the magnetically 
% charged black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{maggupMQ.ps}\vspace*{-3.0cm}
\caption{La composante $MQ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la configuration 
des trous noirs charg\'ee magn\'etiquement.} \label{maggupMQ}\vspace*{0.5cm}
\end{figure}

% The MQ component of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the magnetically 
% charged black hole configuration.


% The nature of the the heat capacities $\{g_{MM}, g_{QQ}\}$of the
% state-space metric tensor is depictedin the 
% Figs.(\ref{maggupMM}, \ref{maggupQQ}). In the regime of $M \in (0,
% 1)$and $Q \in (-1, 1)$, we see that the amplitude of $\{g_{MM}
% \}$takes a value of the order $10^{+06}$. In this range of the
% parameters $\{M, Q\}$, we find that the component $\{ g_{MM}\}$
% lies in the range of $(-8 \times 10^{06}, 0)$. In this case, we
% observe that the range of the growth of the amplitude of $\{g_{QQ}
% \}$is rather distinct in the same limit of $\{Q, M\}$. This
% signifies that the generalized uncertainty principle corrected
% magnetically charged black holes are thermodynamically unstable in
% the limit of small charge and mass. Further, we notice from the
% Fig.(\ref{maggupMQ}) that the mixcomponent $\{ g_{MQ}\}$of the
% state-space metric tensor has both the positive and negative
% values under the fluctuation. In the limit of a small $M$, we find
% that $\{ g_{MQ}\}$takes a large positive value of order $100000$
% and a large negative value of the order $-60000$. In this limit,
% we see that the heat compressibilities depicted in the
% Figs.(\ref{maggupMM}, \ref{maggupQQ}, \ref{maggupMQ}) illustrate
% the fluctuation properties of the magnetically charged black
% holes. In fact, the self pair fluctuations involving $\{M, Q\}$,
% as defined by the metric tensor $\{g_{ij}\ |\ i, j= M, Q\}$, have
% only the negative numerical values, while the mix component $\{
% g_{MQ}\}$has the both.

La nature des capacit\'es de chaleurs $\{g_{MM}, {g_QQ}\}$ de la
m\'etrique tenseure de l'espace des \'etats est repr\'esent\'ee 
dans les Figs. (\ref{maggupMM}, \ref{maggupQQ}). Dans le r\'egime de 
$M \in (0, 1)$ et $Q \in (-1, 1) $, nous voyons que l'amplitude de 
$\{g_{MM}\}$ prend une valeur \`a l'ordre de $10^{+06}$. Dans cette gamme 
de param\`etres $\{M, Q\}$, nous constatons que la composante $\{g_{MM}\}$ 
r\'eside dans la gamme de $(-8 \times 10^{+06}, 0)$. Dans ce cas, nous
observons que la gamme de la croissance de l'amplitude de $\{g_{QQ} \}$ 
est assez distinctes, dans la m\^{e}me limite de $\{Q, M\}$. \c{C}a
signifie que les trous noirs charg\'es magn\'etiquement sous les corrections
du principe d'incertitude g\'en\'eralis\'ee sont thermodynamiquement instable 
dans la limite d'une petite charge et une petite masse. De plus, nous remarquons 
de la Fig. (\ref{maggupMQ}) que la composante mixe $\{g_{MQ}\}$ de la m\'etrique 
tenseure de l'espace des \'etats a \`a la fois les des valeurs positifs et n\'egatifs, 
sous les fluctuations de $\{M, Q\}$. Dans la limite d'une petite $M$, nous trouvons que 
$\{g_{MQ}\}$ prend une grande valeur positive \`a l'ordre de $100000$ et une grande 
valeur n\'egative \`a l'ordre de $-60000$. Dans cette limite des param\`etres, 
nous voyons que les compressibilit\'es thermiques, d\'ecritent dans les Figs. 
(\ref{maggupMM}, \ref{maggupQQ}, \ref{maggupMQ}), illustrent les propri\'et\'es 
graphiques des fluctuations d'un ensemble des trous noirs charg\'es magn\'etiquements. 
En fait, les fluctuations d'auto-paires en impliquant $\{M, Q\}$, tel que d\'efini 
par la m\'etrique tenseure $\{g_{ii} \ | \ i = M, Q\}$, ont seulement certaine valeur 
n\'egative num\'erique, tandis que la composante mixe $\{g_{MQ}\}$ a \`a la fois les 
deux valeurs.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{maggupdet.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la configuration 
de trous noirs charg\'eemagn\'etiquement.} \label{maggupdet}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the magnetically 
% charged black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{maggupminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, M $, en d\'ecrivant les fluctuations de la configuration 
de trous noirs charg\'eemagn\'etiquement.} \label{maggupminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $Q, M$, describing the fluctuations in the magnetically 
% charged black hole configuration.

% As in the case of RN- black holes, the ensemble stability of the
% generalized uncertainty principle corrected magnetically charged
% black holes can be also determined in terms of the values of the
% mass and charge $M, Q$. Furthermore, this follows from the
% behaviour of the determinant of state-space metric tensor. Notice
% that the determinant of the metric tensor tends to a large
% negative value of the order $10^{09}$. For the case of $M \in (-1,
% 1)$and $Q \in (-1, 2)$, the Fig.(\ref{maggupdet}) shows that the
% determinant of the metric tensor lies in the interval $(-3.5
% \times 10^{09}, 0)$. In this case, we find that the negativity of
% $g$increases as the values of $Q$is increased from $-1$to $2$.
% Thus, the surface defined by the fluctuations of $\{M, Q\}$is
% unstable because of a negative value of the determinant of the
% metric tensor. When only the parameter $M$is allowed to vary, the
% stability of the magnetically charged black holes is determined by
% the positivity of the first principle minor $p_1:= g_{MM}$. We
% offer a rotated view of $p_1$in the Fig.(\ref{maggupminor1}).
% Physically, the above graphical properties of the state-space
% quantities illustrate qualitative picture of the statistical
% stability of two parameter magnetically charged black holes under
% the generalized uncertainty principle corrections.

Comme dans le cas des trous noirs de RN, la stabilit\'e d'un ensemble 
des trous noirs charg\'esmagn\'etiquement et corrig\'ees par le principe 
d'incertitude g\'en\'eralis\'ee peuvent \^{e}tre \'egalement d\'etermin\'ee 
en termes des valeurs de la masse $M$ et de la charge $Q$. Par ailleurs, 
cela d\'ecoule du comportement de d\'eterminant de la m\'etrique tenseure
de l'espace des \'etats. Avis que le d\'eterminant de la m\'etrique tenseure 
tend \`a une grande valeur n\'egative \`a l'ordre de $10^{09}$. Pour le cas de 
$M \in (-1, 1)$ et $Q \in (-1, 2)$, la Fig. (\ref{maggupdet}) montre que le 
d\'eterminant de la m\'etrique tenseure r\'eside dans l'intervalle 
$(-3,5 \times 10^{+09}, 0)$. Dans ce cas, nous constatons que la n\'egativit\'e 
de $g$ augmente, quand la valeur de $Q$ est pass\'e de $-1$ \`a $2$.
Ainsi, la surface d\'efinie par les fluctuations de $\{M, Q\}$ est instables 
en raison d'une valeur n\'egative du d\'eterminant de la m\'etrique tenseure. 
Lorsque le seul param\`etre $M$ est autoris\'e \`a varier, la stabilit\'e des 
trous noirs charg\'es magn\'etiquement et corrig\'ees par le principe 
d'incertitude g\'en\'eralis\'ee est d\'etermin\'ee par la positivit\'e 
du premier mineur principe $p_1:= g_{MM}$. Nous offrons une vue rotat\'ee de 
$p_1$ dans la Fig. (\ref{maggupminor1}). Physiquement, les propri\'et\'es graphiques
ci-dessus des quantit\'es de l'espace des \'etat, en invoquant les deux param\`etres $\{M, Q\}$,
illustrent l'image qualitative de la stabilit\'e statistique des trous noirs charg\'ees 
magn\'etiquement sous les corrections du principe d'incertitude g\'en\'eralis\'ee.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{maggupcur.ps}\vspace*{-3.0cm}
\caption{Le courbure scalaire trac\'ee en fonction de $Q, M $, d\'ecrivant 
les variations dans la configuration des trous noirs charg\'es magn\'etiquement 
dans la gamme $M\in (0, 1)$ et $Q \in (-1, 1) $.} \label{maggupcur}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, M$, 
% describing the fluctuations in the magnetically charged black hole configuration
% in the range $M \in (0, 1)$and $Q \in (-1, 1)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{maggupcur1.ps}\vspace*{-3.0cm}
\caption{Le courbure scalaire trac\'ee en fonction de $Q, M $, d\'ecrivant 
les variations dans la configuration des trous noirs charg\'es magn\'etiquement 
dans la gamme $M \in (-1,1)$ et $Q \in (-2, 2)$.} \label{maggupcur1}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, M$, 
% describing the fluctuations in the magnetically charged black hole configuration
% in the range $M \in (-1,1)$ and $Q \in (-2, 2)$.

% The global stability properties of the magnetically charged black
% holes follows from the corresponding state-space scalar curvature.
% In particular, in the range of $M \in (0, 1)$and $Q \in (-1, 1)$,
% the Fig.(\ref{maggupcur}) shows that the scalar curvature has a
% negative amplitude of order $70$. This shows that the underlying
% black hole configuration is an interacting statistical system. The
% negative sign of the scalar curvature signifies an attractive
% nature of the statistical interactions. The Fig.(\ref{maggupcur1})
% signifies the nature of the above scalar curvature in an equal
% range of the parameters. For the case of $M \in (-1,1)$and $Q \in
% (-2, 2)$, we notice from the Fig.(\ref{maggupcur1}) that there
% exists two identical regions of the global statistical interactions. 
% In comparison with the interactions appearing in the range of 
% $M \in (0, 1)$and $Q \in (-1, 1)$, the amplitude of the global 
% statistical interactions appears to be much smaller in the range 
% $M \in (-1, 1)$and $Q \in (-2,2)$. Further, we see that the ratio 
% of a typical value of state-space scalar curvatures appears is of 
% the order $10$. In short, when the parameter $\{M, Q\}$are 
% allowed to fluctuate, the aboveindicate that the 
% generalized uncertainty principle corrected magnetically 
% charged black holes correspond to an unstable interacting 
% statistical configuration.

Les propri\'et\'es globales de la stabilit\'e des trous noirs charg\'es
magn\'etiquements et corrig\'ees par le principe d'incertitude g\'en\'eralis\'ee 
d\'ecoulent de la courbure scalaire correspondante de l'espace des \'etats. 
En particulier, dans la gamme de $M \in (0, 1)$ et $Q \in (-1, 1)$, 
la Fig. (\ref{maggupcur}) montre que la courbure scalaire a une amplitude 
n\'egative \`a l'ordre de $70$. Cela montre que la configuration des trous noirs
sous-tendents correspond \`a un syst\`eme statistique interactif. Le signe n\'egatif 
de la courbure scalaire signifie la nature attractive des interactions statistiques. 
La Fig. (\ref{maggupcur1}) signifie la nature de la courbure scalaire ci-dessus 
dans une range \'egale des param\`etres $\{M, Q\}$. Pour le cas de $M \in (-1,1)$ et $Q \in (-2, 2)$, 
on constate de la Fig. (\ref{maggupcur1}) qu'il y existe deux r\'egions identiques 
des interactions statistiques globales. De plus, en comparaison des interactions apparaissant 
dans la gamme de $M \in (0, 1)$ et $Q \in (-1, 1)$, nous voyons que l'amplitude de 
l'\'echelle des interactions statistiques semble \^{e}tre beaucoup plus petite dans 
la gamme de $M \in (-1, 1)$ et $Q \in (-2,2) $. En outre, nous constatons que le ratio 
d'une valeur typique de ces courbures scalaires de l'espace des \'etats qui apparaissent 
ci-dessus, est \`a l'ordre de $10$. En bref, lorsque les param\`etres $\{M, Q\}$ sont 
autoris\'es \`a fluctuer, l'analyse ci-dessus de la g\'eom\'etrie thermodynamique d'une 
configuration des trous noirs charg\'es magn\'etiquement et corrig\'ees par le principe 
d'incertitude g\'en\'eralis\'ee correspondent \`a un syst\`eme statistique interactive 
et globalement instable.


\section{Les corrections d'$\alpha^{\prime} $}



\subsection{GB}



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBnn1.ps}\vspace*{-3.0cm}
\caption{La composante $nn$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBnn1}\vspace*{0.5cm}
\end{figure}

% The nn component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBww5.ps}\vspace*{-3.0cm}
\caption{La composante $ww$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBww5}\vspace*{0.5cm}
\end{figure}

% The ww component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBNN8.ps}\vspace*{-3.0cm}
\caption{La composante $NN$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBNN8}\vspace*{0.5cm}
\end{figure}

% The NN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBWW10.ps}\vspace*{-3.0cm}
\caption{La composante $WW$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBWW10}\vspace*{0.5cm}
\end{figure}

% The WW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBnw2.ps}\vspace*{-3.0cm}
\caption{La composante $nw$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBnw2}\vspace*{0.5cm}
\end{figure}

% The nw component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBnN3.ps}\vspace*{-3.0cm}
\caption{La composante $nN$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBnN3}\vspace*{0.5cm}
\end{figure}

% The nN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBnW4.ps}\vspace*{-3.0cm}
\caption{La composante $nW$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBnW4}\vspace*{0.5cm}
\end{figure}

% The nW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBwN6.ps}\vspace*{-3.0cm}
\caption{La composante $wN$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBwN6}\vspace*{0.5cm}
\end{figure}

% The wN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBwW7.ps}\vspace*{-3.0cm}
\caption{La composante $wW$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBwW7}\vspace*{0.5cm}
\end{figure}

% The wW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBNW9.ps}\vspace*{-3.0cm}
\caption{La composante $NW$ de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBNW9}\vspace*{0.5cm}
\end{figure}

% The NW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric black hole configuration.


% Since there are four number of independent variables, thus in
% order to offer three dimensional , we shall work in the
% limit of $n=w$, $N= W$. For a given Gauss-Bonnet corrected 
% supersymmetric extremal black hole, we shall choose the value 
% of the higher derivative stringy correction parameter to be
% $\widehat{\alpha}=0.1$throughout the present chapter. Thus, 
% in the regime of $n \in (-10, 0)$and $N \in (0, 10)$, we observe 
% that the amplitudes of the $\alpha^{\prime}$-corrected heat capacities 
% $\{g_{nn}, g_{ww}\}$take a value of the order $10^{+17}$. In this 
% range of $n, N$, the heat capacities $\{ g_{NN}, g_{WW}\}$in the 
% range of $(0,10)$. As per the prediction of the state-space geometry, 
% we find that the range of the growth of the first and the second sets 
% of the heat capacities remains in the opposite limit of the parameters
% $\{n, N\}$. Namely, the first set of heat capacities increase for
% the increasing value of $N$, while the other decreases. Also, the
% Figs.(\ref{alphaGBnn1}, \ref{alphaGBww5}), show that that the
% growth of the first sets of heat capacities $\{ g_{nn}, g_{ww}\}$
% takes place in the limit of a large $N$and small $n$. Similarly,
% the Figs.(\ref{alphaGBNN8}, \ref{alphaGBWW10}) show that the
% growth of the $\{ g_{NN}, g_{WW}\}$takes place in the limit of a
% small $N$and a large $n$. Similarly, the heat compressibilities
% involving two distinct parameters of the black hole are depicted
% in the Figs.(\ref{alphaGBnw2},\ref{alphaGBnN3}, \ref{alphaGBnW4},
% \ref{alphaGBwN6}, \ref{alphaGBwW7}, \ref{alphaGBNW9}). In fact,
% the fluctuations involving the parameters $\{n, w\}$, as defined
% via the state-space metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W
% \}$, have relatively larger numerical values than those involving
% the parameters $\{N, W\}$.
 
Puisqu'il y a des quatre variables ind\'ependantes, en particulier les nombres de branes
$\{n, w, N, W \}$, donc en afin d'offrir leur vue graphique en trois dimensions, 
nous allons consid\'ere la limite $n = w $ et $N = W $. Pour une correction  donn\'ee
de Gauss-Bonnet aux trous noirs extr\^{e}maux supersym\'etriques, nous allons choisir 
la valeur du param\`etre des corrections d\'eriv\'ees sup\'erieures de la th\'eorie 
des cordes d'\^{e}tre $\widehat{\alpha}= 0.1$ tout au long du pr\'esent chapitre. 
Ainsi, dans le r\'egime de $n \in (-10, 0)$ et $N \in (0, 10)$, nous observons
que l'amplitude des capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ corrig\'ees par
les $\alpha^{\prime}$ prend une valeur \`a l'ordre de $10^{17}$. Dans cette gamme de 
$n, N$, les capacit\'es de chaleurs $\{g_{NN}, g_{WW}\}$ relient dans la gamme de 
$(0, 10)$. En conform\'ement \`a la pr\'ediction de la g\'eom\'etrie de l'espace des \'etats,
nous constatons que la gamme de croissance de la premi\`ere ensemble et de la deuxi\`eme 
ensemble des capacit\'es de chaleur reste dans la limite oppos\'ee des param\`etres
$\{n, N\}$. \`A savoir, la premi\`ere s\'erie de capacit\'es de chaleurs augmente 
avec la valeur de $N$, tandis que l'autre croissante diminue. Du fait m\^{e}me, les Figs. 
(\ref{alphaGBnn1}, \ref{alphaGBww5}) montrent que la croissance de premier ensemble 
des capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ prend place dans la limite d'un grand 
$N$ et un petit $n$. En outre, les Figs. (\ref{alphaGBNN8}, \ref{alphaGBWW10}) 
montrent que la croissance de $\{g_{NN}, g_{WW}\}$ a lieu dans la limite d'un
petit $N$ et un grand $n$. De plus, les compressibilit\'es de chaleurs, 
en impliquant deux param\`etres distincts de la configuration de ces trous noirs,
sont repr\'esent\'es dans les Figs. (\ref{alphaGBnw2},\ref{alphaGBnN3}, \ref{alphaGBnW4},
\ref{alphaGBwN6}, \ref{alphaGBwW7}, \ref{alphaGBNW9}). En fait, les fluctuations en
impliquant les param\`etres $\{n, w\}$, tel que d\'efini par la m\'etrique tenseure de 
l'espace des \'etats $\{g_{ij} \ | \ i, j = n, w \}$, ont relativement des plus grande 
valeurs num\'eriques en comparaison de celles qui impliquant les param\`etres $\{N, W\}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBdetg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBdetg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric charged black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBminor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBminor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric charged black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'e comme la 
fonction de $\{n, N\}$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs supersym\'etriques corrig\'es par 
les termes de Gauss-Bonnet.} \label{alphaGBminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the Gauss-Bonnet 
% corrected supersymmetric charged black hole configuration.


% As the function of $\{N, W\}$, the ensemble stability of the 
% Gauss-Bonnet corrected supersymmetric extremal black holes follows 
% from the positivity of the determinant of the metric tensor. 
% In this case, we notice that the determinant of the metric 
% tensor $g$does not depend on the parameters $\{n, w\}$. Indeed,
% we find that $g \in (-100, 0)$. For a typical value of $N \in (0, 10)$
% and $W \in (0,10)$, the Fig.(\ref{alphaGBdetg}) offers the graphical
% nature of the determinant of the metric tensor $g$. For the choice
% of $n=w$, $N= W$, the stability of the hypersurface defined by a constant
% value of $W$is shown in the Fig.(\ref{alphaGBminor3}). Hereby, we
% see that the minor $p_3$lies in the range of $(-1.2 \times
% 10^{18}, 0)$. Notice that the negativity of $p_3$increases as the
% value of $N$is increased from zero to $10$. Furthermore, the
% surface defined by the fluctuations of $(n,w)$is unstable because
% the corresponding principle minor vanishes identically, viz., we
% have $p_2=0$. Finally, when only the parameter $n$is allowed to
% vary, the stability of the black hole is given by the positivity
% of the first principle minor $p_1:= g_{nn}$. A rotated view of
% $p_1$is shown in the Fig.(\ref{alphaGBminor1}). The above
% state-space properties and positivity of the concerned principle
% minors provide the qualitative notion of the statistical stability
% of Gauss-Bonnet corrected black holes.

Comme une fonction des param\`etres $\{N, W\}$, la stabilit\'e d'un ensemble 
des trous noirs supersym\'etriques extr\'emaux, corrig\'ees par les termes de
Gauss-Bonnet, suivit de la positivit\'e du d\'eterminant de la m\'etrique tenseure.
Dans ce cas, nous remarquons que le d\'eterminant de la m\'etrique tenseure 
$g$ est ind\'epend des param\`etres $\{n, w\}$. En effet, nous constatons que 
$g \in (-100, 0)$ pour une valeur typique de $N \in (0, 10)$ et $W \in (0, 10)$. 
En ce cas, la Fig. (\ref{alphaGBdetg}) offre la nature graphique du d\'eterminant 
de la m\'etrique tenseure $g$. Pour le choix de $n= w $, $N= W$, la stabilit\'e de 
l'hypersurface d\'efinie par une constante valeur de $W$ est montr\'e dans la 
Fig. (\ref{alphaGBminor3}). Par la pr\'esente, nous pouvons voir que le mineur $p_3$ 
r\'eside dans la gamme de $(-1.2 \times 10^{+18}, 0)$. Notez bien en cas de $n \in (-10, 0)$ 
et $N \in (0, 10)$ que la n\'egativit\'e de $p_3$ augmente \`a mesure que la valeur 
de $N$ est pass\'ee de z\'ero \`a $10$. En outre, la surface d\'efinie par les 
fluctuations de $(n, w)$ est instable \`a cause du fait m\^eme que le mineur 
principe correspondant est identiquement nulle, \`a savoir que nous avons $p_2= 0$. 
Enfin, lorsque le seul param\`etre $n$ est autoris\'e \`a varier, 
la stabilit\'e de la configuration des trous noirs sous-jacents est donn\'ee 
par la positivit\'e du premier mineur principe $p_1:= g_{nn}$. Une vue rotat\'ee
de $p_1$ est montr\'ee dans la Fig. (\ref{alphaGBminor1}). Les propri\'et\'es 
ci-dessus de l'espace de l'\'etat et la positivit\'e des mineurs principes 
concern\'es fournent la notion qualitative de la stabilit\'e statistique
des trous noirs supersym\'etriques extr\'emaux corrig\'ees par les termes 
de Gauss-Bonnet.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBR.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'e comme la fonction de $\{n, N\}$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
supersym\'etriques corrig\'es par les termes de Gauss-Bonnet dans la gamme
$n \in (-10, 0)$ et $N \in (0,10) $.} \label{alphaGBR}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the Gauss-Bonnet corrected 
% supersymmetric charged black hole configuration in the range 
% $n \in (-10,0)$and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{alphaGBR30.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'e comme la fonction de $\{n, N\}$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
supersym\'etriques corrig\'es par les termes de Gauss-Bonnet dans la gamme
$n, N \in (-30,30) $.} \label{alphaGBR30}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the Gauss-Bonnet corrected 
% supersymmetric charged black hole configuration in the range 
% $n, N \in (-30,30)$.

% The global statistical properties follows from the behaviour of
% the state-space scalar curvature. In the range of $n \in (-10,0)$
% and $N \in (0,10)$, the Fig.(\ref{alphaGBR}) shows that the scalar
% curvature has a large positive amplitude of the order $10^{08}$. We
% observe that the underlying black hole configuration is a strongly
% interacting statistical system in this range of the parameters.
% Physically, the positive sign of the scalar curvature signifies
% that the statistical interactions are repulsive in their nature.
% The Fig.(\ref{alphaGBR30}) illustrates the behaviour of the above
% scalar curvature for range of the parameters $n, N \in (-30,30)$.
% In fact, when the range of $n$and $N$is taken in the multiple of
% $3$, then we notice from the Fig.(\ref{alphaGBR30}) that there exists
% four similar disjoint regions of the global statistical interactions. 
% In comparison with the interactions appearing in the range of 
% $n \in (-10,0)$and $N \in (0,10)$, the amplitude of the
% global statistical interactions turn out to be much smaller in the
% range of $n, N \in (-30,30)$. Under the higher derivative stringy
% $\alpha^{\prime}$-corrections, we find that the ratio of the
% typical value of the amplitude of state-space scalar curvatures is
% of the order $10^{-10}$. The graphical view of the above mentioned
% comparison is apparent from the plots of the scalar curvatures
% Figs.(\ref{alphaGBR}, \ref{alphaGBR30}). Qualitatively, in the small 
% values of the $n, N$, the state-space depictions indicate that the
% Gauss-Bonnet corrected black holes are globally unstable
% statistical configurations under the variation of the black hole
% parameters $\{n, w, N, W\}$.

Les propri\'et\'es statistiques globales d\'ecoulent du comportement de
la courbure scalaire de l'espace des \'etats. Dans la gamme de $n \in (-10, 0)$
et $N \in (0, 10)$, la Fig. (\ref{alphaGBR}) montre que la courbure scalaire 
a une grande amplitude positive \`a l'ordre de $10^{+08} $. Nous observons que 
la configuration sous-jacente des trous noirs est un syst\`eme statistique 
fortement interagissant dans cette gamme des param\`etres. Physiquement, 
le signe positif de la courbure scalaire signifie que les interactions 
statistiques sont r\'epulsives dans la leur nature. La Fig. (\ref{alphaGBR30}) 
illustre le comportement de ce qui pr\'ec\`ede de la courbure scalaire dans
la gamme des param\`etres $n, N \in (-30, 30)$. En fait, lorsque la gamme de 
$n$ et $N$ est prise dans le multiple de $3$, alors nous remarquons de la 
Fig. (\ref{alphaGBR30}) qu'il existe quatre r\'egions disjointes similaires 
des interactions statistiques globales. En comparaison des interactions 
apparaissant dans la gamme de $n \in (-10, 0)$ et $N \in (0, 10)$, l'amplitude 
des interactions statistiques globales se r\'ev\`ele \^{e}tre beaucoup plus petite
dans la gamme de $n, N \in (-30,30) $. Sous les corrections de d\'eriv\'ees
sup\'erieures de $\alpha^{\prime}$, nous constatons que le ratio des valeurs 
typiques de l'amplitude de ces courbures scalaires de l'espace des \'etats est
\`a l'ordre de $10^{-10}$. La vue graphique de la comparaison mentionn\'ee ci-dessus
de la courbure scalaire est apparente dans les Figs. (\ref{alphaGBR}, \ref{alphaGBR30}). 
Qualitativement, en cas de petite valeur des param\`etres $\{n, N\}$, nous voyons par
les repr\'esentations de l'espace des \'etats indiquent que la configuration 
des trous noirs supersym\'etriques extr\'emaux corrig\'ees par les termes de 
Gauss-Bonnet correspond \`a un syst\`eme statistique globalement instable
en vertu des variations de param\`etres $\{n, w, N, W\}$.


\subsection{Non-susy 0}



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0nn1.ps}\vspace*{-3.0cm}
\caption{La composante $nn$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0nn1}\vspace*{0.5cm}
\end{figure}

% The nn component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0ww5.ps}\vspace*{-3.0cm}
\caption{La composante $ww$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0ww5}\vspace*{0.5cm}
\end{figure}

% The ww component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0NN8.ps}\vspace*{-3.0cm}
\caption{La composante $NN$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0NN8}\vspace*{0.5cm}
\end{figure}

% The NN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0WW10.ps}\vspace*{-3.0cm}
\caption{La composante $WW$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0WW10}\vspace*{0.5cm}
\end{figure}

% The WW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0nw2.ps}\vspace*{-3.0cm}
\caption{La composante $nw$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0nw2}\vspace*{0.5cm}
\end{figure}

% The nw component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0nN3.ps}\vspace*{-3.0cm}
\caption{La composante $nN$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0nN3}\vspace*{0.5cm}
\end{figure}

% The nN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0nW4.ps}\vspace*{-3.0cm}
\caption{La composante $nW$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0nW4}\vspace*{0.5cm}
\end{figure}

% The nW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0wN6.ps}\vspace*{-3.0cm}
\caption{La composante $wN$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0wN6}\vspace*{0.5cm}
\end{figure}

% The wN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0wW7.ps}\vspace*{-3.0cm}
\caption{La composante $wW$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0wW7}\vspace*{0.5cm}
\end{figure}

% The wW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0NW9.ps}\vspace*{-3.0cm}
\caption{La composante $NW$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0NW9}\vspace*{0.5cm}
\end{figure}

% The NW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.


% In the limit of $n=w$and $N= W$, we observe in the interval of
% $n \in (-10,0)$and $N \in (0,10)$that the amplitudes of the heat
% capacities $\{g_{nn}, g_{ww}\}$take a maximum value of the order
% $2 e+09$. Similarly, the heat capacities $\{ g_{NN}, g_{WW}\}$
% take a typical value between $(0,40)$. We observe that the range
% of the growth of the first and the second sets of the heat
% capacities happens to be in the opposite limit of the parameters
% $\{n, N\}$. Explicitly, from the Figs.(\ref{nonsusy0nn1},
% \ref{nonsusy0ww5}), we find that that the of growth of the heat
% capacities $\{ g_{nn}, g_{ww}\}$takes place in the limit of a
% large $N$and small $n$. On the other hand, from the
% Figs.(\ref{nonsusy0NN8}, \ref{nonsusy0WW10}), we see that the
% growth of the $\{ g_{NN}, g_{WW}\}$takes place in the limit of a
% small $N$and a large $n$. Similarly, the heat compressibilities
% involving two distinct parameters of the non-supersymmetric black
% hole have been depicted in the Figs.(\ref{nonsusy0nw2},
% \ref{nonsusy0nN3}, \ref{nonsusy0nW4}, \ref{nonsusy0wN6},
% \ref{nonsusy0wW7}, \ref{nonsusy0NW9}). From the definition of the
% state-space metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W\}$, we
% observe that the fluctuations involving $\{n, w\}$have a larger
% relative numerical values than those involving the parameters
% $\{N, W\}$.

\`A la limite de $n= w$ et $N= W$, on observe dans l'intervalle de
$n \in (-10, 0)$ et $N \in (0, 10)$ que l'amplitudes des capacit\'es 
de chaleures $\{g_{nn}, g_{ww}\}$ prendent la valeur maximale \`a l'ordre
de $2 \times 10^{09}$. Du fait m\^{e}me, les capacit\'es de chaleurs $\{g_{NN}, g_{WW}\}$ 
prendent une valeur typique entre $(0, 40)$. Nous observons que la gamme
de croissance de la premi\`ere ensemble et celle de la deuxi\`eme ensemble 
des capacit\'es de chaleurs se trouve \^{e}tre \`a la limite oppos\'ee 
des param\`etres $\{n, N\}$. Explicitement, par les Figs. (\ref{nonsusy0nn1},
\ref{nonsusy0ww5}), nous constatons que la croissance des capacit\'es 
de chaleurs $\{g_{nn}, g_{ww}\}$ a lieu dans la limite d'un grand $N$
et d'un petit $n$. D'autre part, par les Figs. (\ref{nonsusy0NN8}, \ref{nonsusy0WW10}), 
nous voyons que la croissance de $\{g_{NN}, g_{WW}\}$ a lieu dans la limite d'un
petit $N$ et un grand $n$. De plus, les compressibilit\'es de chaleures en
impliquant deux param\`etres distincts de la configuration de ces trous noirs 
non-supersym\'etriques ont repr\'esent\'ees dans les Figs. (\ref{nonsusy0nw2},
\ref{nonsusy0nN3}, \ref{nonsusy0nW4}, \ref{nonsusy0wN6}, \ref{nonsusy0wW7}, 
\ref{nonsusy0NW9}). Par la d\'efinition de la m\'etrique tenseure de l'espace
des \'etats $\{g_{ij} \ | \ i, j = n, w, N, W\}$, nous observer que les fluctuations 
en impliquant $\{n, w\}$ ont relativement une plus grande valeur num\'erique 
de celles qui impliquant $\{N, W\}$.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0minor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0minor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0minor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee 
comme la fonction de $\{n, N\}$, d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es non-supersym\'etriques 
\`a l'ordre dominant.} \label{nonsusy0minor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order.


% As the function of $n, N$, the ensemble stability condition
% follows from the positivity of the determinant of the metric
% tensor. In this case, we see that the determinant of the metric
% tensor tends to a negative value of -$\pi^4$. For a typical value
% of $n \in (-10,0)$ and $N \in (0,10)$, the stability of the
% hypersurface defined by a constant value of $W$is shown in the
% Fig.(\ref{nonsusy0minor3}). From the Fig.(\ref{nonsusy0minor3}),
% we see that the minor $p_3$ lies in the interval $(0, -2\times
% 10^{10})$. Notice that the negativity of the minor $p_3$increases
% as the value of $N$is increased from zero to $10$. Moreover, the
% surface defined by the fluctuations of $(n,w)$is unstable because
% of the corresponding principle minor vanishes identically, viz.,
% we have $p_2=0$. When only the parameter $n$ is allowed to vary,
% we find that the stability of the concerned black hole
% configuration is given by the positivity of the first principle
% minor $p_1:=g_{nn}$. As shown in the Fig. \ref{nonsusy0minor1}),
% we observe that $p_1$lies in the range of $(0, 2 \times 10^{19})
% $. The above graphical properties of the components and positivity
% of the state-space principle minors provide the qualitative notion
% of the statistical stability of non-supersymmetric black holes at
% the leading order.

Comme une fonction de $\{n, N\}$, la condition de la stabilit\'e d'un 
ensemble de ces trous noirs non-supersymmetriques d\'ecoule de la positivit\'e 
du d\'eterminant de la m\'etrique tenseure. Dans ce cas, nous voyons que 
le d\'eterminant de la m\'etrique tenseure prend la valeur n\'egative de $-\pi^4$. 
Pour une valeur typique de $n \in (-10, 0)$ et $N \in (0, 10) $, la stabilit\'e 
de l'hypersurface d\'efinie par une valeur constante de $W$ est pr\'esent\'ee 
dans la Fig. (\ref{nonsusy0minor3}). De la Fig. (\ref{nonsusy0minor3}), nous voyons 
que le mineur $p_3$ r\'eside dans l'intervalle $(0, -2 \times 10^{10})$. 
Notez bien que la n\'egativit\'e du mineur $p_3$ augmente quand la valeur de 
$N$ est pass\'ee de z\'ero \`a $10$. Par ailleurs, le surface d\'efinie par 
des fluctuations de $\{n, w\}$ est instable \`a cause du fait que le mineur 
principe correspondant est identiquement nulle, \`a savoir que nous avons $p_2= 0$. 
Lorsque le seul param\`etre $n$ est autoris\'e \`a varier, nous constatons que 
la stabilit\'e de la configuration de ces trous noirs concern\'es est donn\'ee par 
la positivit\'e du premier mineur principe $p_1:= g_{nn}$. Comme montr\'e dens
la Fig. (\ref{nonsusy0minor1}), nous observons que le premier mineur principe $p_1$ 
r\'eside dans la gamme de $(0, 2 \times 10^{19})$. Les propri\'et\'es graphiques 
ci-dessus des composantes et la positivit\'e des mineurs principaux de l'espace 
des \'etats fournent la notion qualitative de la stabilit\'e statistique des 
trous noirs non-supersym\'etriques \`a l'ordre dominant.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0R.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee en fonction de $\{n, N\}$,
d\'ecrivant les fluctuations de la configuration des trous noirs 
charg\'es non-supersym\'etriques \`a l'ordre dominant dans la gamme
$n \in (-10, 0)$ et $N \in (0, 10)$.} \label{nonsusy0R}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order in the range 
% $n \in (-10,0)$and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy0R30.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee en fonction de $\{n, N\}$,
d\'ecrivant les fluctuations de la configuration des trous noirs 
charg\'es non-supersym\'etriques \`a l'ordre dominant dans la gamme
$n, N \in (-30,30)$.} \label{nonsusy0R30}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric 
% charged black holes at the leading order in the range 
% $n, N \in (-30,30)$.


% The global stability properties follows from the behaviour of the
% state-space scalar curvature. In particular, in the range of the
% parameters $n \in (-10,0)$and $N \in (0,10)$, the
% Fig.(\ref{nonsusy0R}) shows that the amplitude of the state-space
% scalar curvature tends to a large positive value. We may notice
% that the underlying black hole configuration is a strongly
% interacting statistical system. Physically, the positive sign of
% the scalar curvature signifies a repulsive of the interactions.
% The Fig.(\ref{nonsusy0R30}) illustrates the nature of the above
% scalar curvature in an equal range of the $n, N \in (-30,30)$. As a
% matter of fact, when the range of $n$and $N$is taken in the
% multiple of $3$, for example (-30, 30), then we see from the
% Fig.(\ref{nonsusy0R30}) that there are four similar disjoint
% regions of the global statistical interactions. In comparison with
% the interactions appearing in the range of $n \in (-10,0)$and $N
% \in (0,10)$, the amplitude of the interactions turns out to be
% much smaller for the range of parameters $n, N \in (-30,30)$. The
% typical value of the amplitude of the scalar curvatures appears to
% be $10^{-10}$. The above mentioned graphical view of the comparison
% of the global statistical interaction follows from the Figs.
% (\ref{nonsusy0R}, \ref{nonsusy0R30}). Qualitatively, in the small
% values of $n,N$, the Figs. (\ref{nonsusy0R}, \ref{nonsusy0R30})
% indicate that the non-supersymmetric black holes are unstable
% statistical configurations.

Les propri\'et\'es globales de la stabilit\'e d\'ecoulent par le comportement 
de la courbure scalaire de l'espace des \'etats. En particulier, dans la gamme des
param\`etres $n \in (-10, 0)$ et $N \in (0, 10) $, la Fig. (\ref{nonsusy0R}) montre 
que l'amplitude de la courbure scalaire de l'espace des \'etats tend vers une tr\`es 
grande valeur positive. On peut remarquer que la configuration sous-jacente des 
trous noirs est un syst\`eme statistique fortement interagissant. Physiquement, 
le signe positif de la courbure scalaire signifie une r\'epulsion de ces interactions.
La Fig. (\ref{nonsusy0R30}) illustre la nature de ce qui pr\'ec\`ede de la courbure 
scalaire dans une range \'egale de $n, N \in (-30, 30) $. En tant que, en effet, 
lorsque la gamme de $n$ et $N$ est prise dans le multiple de $3$, par exemple 
$(-30, 30)$, alors que nous voyons de la Fig. (\ref{nonsusy0R30}) qu'il y a 
quatre r\'egions disjointes similaires de ces interactions statistiques globales. 
En comparaison des interactions apparaissant dans la gamme de $n \in (-10, 0)$
et $N \in (0, 10) $, l'amplitude de ces interactions se r\'ev\`ele \^{e}tre beaucoup 
plus petite dans la gamme des param\`etres $n, N \in (-30,30) $. En ce cas, nous observons 
que le ratio d'une amplitude typique de ces courbures scalaires semble \^{e}tre \`a l'ordre 
de $10^{-10}$. La vue graphique ci-dessus mentionn\'ee de cette comparaison des interactions 
statistiques globales d\'ecoule par les Figs. (\ref{nonsusy0R}, \ref{nonsusy0R30}). 
Qualitativement, dans une petite valeur des $n, N$, les Figs. (\ref{nonsusy0R}, 
\ref{nonsusy0R30}) indiquent que les trous noirs non-supersym\'etriques correspondent 
\`a une configuration statistique interactive qu'elle est globalement instable.


\subsection{Non-susy 1}


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1nn1.ps}\vspace*{-3.0cm}
\caption{La composante $nn$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1nn1}\vspace*{0.5cm}
\end{figure}

% The nn component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1ww5.ps}\vspace*{-3.0cm}
\caption{La composante $ww$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1ww5}\vspace*{0.5cm}
\end{figure}

% The ww component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1NN8.ps}\vspace*{-3.0cm}
\caption{La composante $NN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1NN8}\vspace*{0.5cm}
\end{figure}

% The NN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1WW10.ps}\vspace*{-3.0cm}
\caption{La composante $WW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1WW10}\vspace*{0.5cm}
\end{figure}

% The WW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1nw2.ps}\vspace*{-3.0cm}
\caption{La composante $nw$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1nw2}\vspace*{0.5cm}
\end{figure}

% The nw component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1nN3.ps}\vspace*{-3.0cm}
\caption{La composante $nN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1nN3}\vspace*{0.5cm}
\end{figure}

% The nN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1nW4.ps}\vspace*{-3.0cm}
\caption{La composante $nW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1nW4}\vspace*{0.5cm}
\end{figure}

% The nW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1wN6.ps}\vspace*{-3.0cm}
\caption{La composante $wN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1wN6}\vspace*{0.5cm}
\end{figure}

% The wN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1wW7.ps}\vspace*{-3.0cm}
\caption{La composante $wW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1wW7}\vspace*{0.5cm}
\end{figure}

% The wW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1NW9.ps}\vspace*{-3.0cm}
\caption{La composante $NW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1NW9}\vspace*{0.5cm}
\end{figure}

% The NW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

% In the limit of $n=w$, $N= W$and $\widehat{\alpha}=0.1$, we
% observe for $n \in (-10,0)$and $N \in (0,10)$that the amplitudes
% of the heat capacities $\{g_{nn}, g_{ww}\}$take a maximum value
% of the order $2 \times 10^{+09}$. While, the heat capacities $\{ g_{NN},
% g_{WW}\}$take a typical value between $(-4,14)$. In fact, the
% range of the growth of the first and the second sets of the heat
% capacities happens to be in the opposite limit of the parameters
% $\{n, N\}$. Explicitly, from the Figs.(\ref{nonsusy1nn1},
% \ref{nonsusy1ww5}), we find that that the of growth of the heat
% capacities $\{ g_{nn}, g_{ww}\}$ takes place in the limit of a
% large $N$and small $n$. On the other hand, the
% Figs.(\ref{nonsusy1NN8}, \ref{nonsusy1WW10}) show that the growth
% of the $\{ g_{NN}, g_{WW}\}$ takes place in the limit of a small
% $N$and a large $n$. Similarly, the heat compressibilities
% involving two distinct parameters of the black hole have been
% depicted in the Figs.(\ref{nonsusy1nw2}, \ref{nonsusy1nN3},
% \ref{nonsusy1nW4}, \ref{nonsusy1wN6}, \ref{nonsusy1wW7},
% \ref{nonsusy1NW9}). In this case, we observe that the fluctuations
% involving $\{n, w\}$, as defined by the components of the
% state-space metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W\}$, have
% relatively larger numerical values with respect to those involving
% $\{N, W\}$.

Dans la limite de $n = w$, $N= W$ et $\widehat{\alpha}=0.1$, nous
observons pour $n \in (-10, 0)$ et $N \in (0, 10)$ que l'amplitude
des capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ prend la valeur maximale
\`a l'ordre de $2 \times 10^{+09}$. Alors, les capacit\'es de chaleurs 
$\{g_{NN},g_{WW}\}$ prendent une valeur typique entre $(-4, 14​​)$. En fait, 
la gamme de la croissance de la premi\`ere ensemble et la deuxi\`eme ensemble
des capacit\'es de la chaleure se trouvent \^{e}tre \`a la limite oppos\'ee 
des param\`etres $\{n, N\}$. Explicitement, par les Figs. (\ref{nonsusy1nn1},
\ref{nonsusy1ww5}), nous constatons que la croissance des capacit\'es 
de chaleurs $\{g_{nn}, g_{ww}\}$ a lieu dans la limite d'un grand $N$
et un petit $n$. D'autre part, par les Figs. (\ref{nonsusy1NN8}, \ref{nonsusy1WW10}), 
nous pouvons voir facilement que la croissance de $\{g_{NN}, g_{WW}\}$ 
a lieu dans la limite d'un petit $N$ et un grand $n$. Du fait m\^{e}me, 
les compressibilit\'es de chaleurs en impliquant deux param\`etres distincts 
de la configuration de ces trous noirs sont repr\'esent\'ees dans les Figs. 
(\ref{nonsusy1nw2}, \ref{nonsusy1nN3}, \ref{nonsusy1nW4}, \ref{nonsusy1wN6}, 
\ref{nonsusy1wW7}, \ref{nonsusy1NW9}). Dans ce cas, on observe que les 
fluctuations en impliquant $\{n, w\}$, tel qu'elle sont d\'efinies 
par les composantes de la m\'etrique tenseure de l'espace des \'etats 
$\{g_{ij} \ | \ i, j = n, w\}$, ont relativement des plus grande valeurs 
num\'eriques par rapport \`a celles qui impliquant $\{N, W\}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1detg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1detg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the function of 
% $n, N$, describing the fluctuations in the non-supersymmetric charged 
% black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1minor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1minor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1minor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$.} \label{nonsusy1minor1}\vspace*{0.5cm}
\end{figure}


% The first minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the first order stringy corrections.

% As the function of $n, N$, the ensemble stability condition
% follows from the positivity of the determinant of the metric
% tensor. In this case, we see that the determinant of the metric
% tensor tends to a negative value. For a typical value of $n \in
% (-10,0)$ and $N \in (0,10)$, the Fig.(\ref{nonsusy1detg}) shows
% that the determinant of the metric tensor lies in the interval
% $(-30,-100)$. The stability of the hypersurface defined by a
% constant value of $W$ is shown in the Fig.(\ref{nonsusy1minor3}).
% Hereby, we see that the minor $p_3$ lies in the range of $(-2
% 10^{10}, 0)$. Notice that the negativity of $p_3$ increases as the
% value of $N$is increased from zero to $10$. Moreover, the surface
% defined by the fluctuations of $(n,w)$is unstable because of the
% fact that the corresponding principle minor vanishes, viz.,
% $p_2=0$. When only $n$is allowed to vary, the stability of the
% configuration is given by the positivity of the first principle
% minor $p_1:= g_{nn}$. A rotated view of $p_1$is shown in the 
% Fig.(\ref{nonsusy1minor1}). The above graphical properties of 
% the principle minors and the positivity of the components of the 
% state-space metric tensor provide the qualitative notion of the 
% statistical stability of non-supersymmetric black holes.

Comme une fonction de $\{n, N\}$, la condition de la stabilit\'e d'un ensemble
de ces trous noirs d\'ecoule de la positivit\'e du d\'eterminant de la m\'etrique 
tenseure. Dans ce cas, nous voyons que le d\'eterminant de la m\'etrique tenseure 
tend vers une valeur n\'egative. Pour une valeur typique de $n \in (-10, 0)$
et $N \in (0, 10)$, la Fig. (\ref{nonsusy1detg}) montre que le d\'eterminant 
de la m\'etrique tenseure r\'eside dans l'intervalle $(-30, -100)$. En outre,
la stabilit\'e de l'hypersurface d\'efinie par une valeur constante de $W$ est 
montr\'ee dans la Fig. (\ref{nonsusy1minor3}). Par la pr\'esente, nous voyons que 
le mineur $p_3$ r\'eside dans la gamme de $(-2 \times 10^{+10}, 0)$. Notez bien
que la n\'egativit\'e de $p_3$ augmente \`a mesure que la valeur de $N$ est pass\'ee 
de z\'ero \`a $10$. Par ailleurs, il s'av\`ere que la surface d\'efinies par les fluctuations 
de $\{n, w \}$ est instable en raison du fait m\^eme que le mineur principe correspondant 
dispara\^{i}t, \`a savoir que nous avons $p_2= 0$. Quand le seulement param\`etre $n$ 
est autoris\'e \`a varier, la stabilit\'e de la configuration de ces trous noirs est donn\'ee 
par la positivit\'e du premier mineur principe $p_1:= g_{nn}$. Une vue rotat\'ee de $p_1$
est pr\'esent\'ee dans la Fig. (\ref{nonsusy1minor1}). Les propri\'et\'esgraphiques
ci-dessus des mineurs principaux et la positivit\'e des composants de la m\'etrique 
tenseure de l'espace des \'etats fournent la notion qualitative de la stabilit\'e 
statistique des non-supersym\'etriques trous noirs.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1R.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$ dans la gamme
$n \in (-10,0)$ et $N \in (0,10) $.} \label{nonsusy1R}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the first order stringy corrections in the range 
% $n \in (-10,0)$and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy1R30.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
premier ordre de $\alpha^{\prime}$ dans la gamme
$n, N \in (-30,30)$.} \label{nonsusy1R30}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the first order stringy corrections in the range 
% $n, N \in (-30,30)$.

% Similarly, the global stability properties follows from the
% behaviour of the state-space scalar curvature. In particular, in
% the range of $n \in (-10,0)$and $N \in (0,10)$, the
% Fig.(\ref{nonsusy1R}) shows that the scalar curvature has a large
% positive amplitude. We may note that the underlying black hole
% configuration is a strongly interacting statistical system. The
% positive sign of the scalar curvature signifies a repulsive of the
% interactions. The Fig.(\ref{nonsusy1R30}) illustrates the nature
% of the above scalar curvature in an equal range of the $n, N \in
% (-30,30)$. In fact, when the range of $n$and $N$is taken in the
% multiple of $3$, for example (-30, 30), then we see from the
% Fig.(\ref{nonsusy1R30}) that there are four similar disjoint
% regions of the global statistical interactions. In comparison with
% the interactions appearing in the range of $n \in (-10,0)$and $N
% \in (0,10)$, the amplitude of the interactions turns out to be
% much smaller in the range of $n, N \in (-30,30)$. The typical
% value of the amplitude of the scalar curvatures appears to be
% $10^{-10}$. The graphical view of the above mentioned comparison
% follows from the Figs. (\ref{nonsusy1R}, \ref{nonsusy1R30}).
% Qualitatively, in the small values of the $n,N$, the above
% graphical depictions indicate that the non-supersymmetric
% black holes are unstable statistical configurations at the
% first order stringy corrections.

De plus, les propri\'et\'es de la stabilit\'e globale r\'esultent du
comportement de la courbure scalaire de l'espace des \'etats. En particulier, 
dans la gamme de $n \in (-10, 0)$ et $N \in (0, 10)$, la Fig. (\ref{nonsusy1R}) 
montre que la courbure scalaire a une grande positive amplitude. On peut noter 
que la configuration des trous noirs sous-tendents est un syst\`eme statistique
fortement interagissant. Le signe positif de la courbure scalaire signifie une 
r\'epulsion de ces interactions. La Fig. (\ref{nonsusy1R30}) illustre la nature
de la courbure scalaire ci-dessus dans une range \'egale de $n, N \in
(-30,30)$. En fait, lorsque la gamme de $n$ et $N$ est prise dans le
multiple de $3$, par exemple $(-30, 30)$, alors que nous voyons de la
Fig. (\ref{nonsusy1R30}) qu'il y a quatre r\'egions disjointes similaires 
des interactions statistiques globales. En comparaison des interactions 
apparaissant dans la gamme de $n \in (-10, 0)$ et $N \in (0, 10)$, 
l'amplitude de l'interaction se r\'ev\`ele \^{e}tre beaucoup plus petit 
dans la gamme de $n, N \in (-30, 30) $. Le ratio de la valeur typique de l'amplitude 
de ces courbures scalaires semble \^{e}tre $10^{-10}$. La vue graphique de la 
comparaison ci-dessus d\'ecoule des Figs. (\ref{nonsusy1R}, \ref{nonsusy1R30}).
Qualitativement, dans une petite valeur des $n, N$, les repr\'esentations 
graphiques ci-dessus indiquent que la configuration des trous noirs non-supersym\'etriques
correspond \`a un syst\`eme statistique instable aux corrections de premier 
ordre de $\alpha^{\prime}$.



\subsection{Non-susy 2}



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2nn1.ps}\vspace*{-3.0cm}
\caption{La composante $nn$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2nn1}\vspace*{0.5cm}
\end{figure}

% The nn component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2ww5.ps}\vspace*{-3.0cm}
\caption{La composante $ww$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2ww5}\vspace*{0.5cm}
\end{figure}

% The ww component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2NN8.ps}\vspace*{-3.0cm}
\caption{La composante $NN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2NN8}\vspace*{0.5cm}
\end{figure}

% The NN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2WW10.ps}\vspace*{-3.0cm}
\caption{La composante $WW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2WW10}\vspace*{0.5cm}
\end{figure}

% The WW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2nw2.ps}\vspace*{-3.0cm}
\caption{La composante $nw$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2nw2}\vspace*{0.5cm}
\end{figure}

% The nw component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2nN3.ps}\vspace*{-3.0cm}
\caption{La composante $nN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2nN3}\vspace*{0.5cm}
\end{figure}

% The nN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2nW4.ps}\vspace*{-3.0cm}
\caption{La composante $nW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2nW4}\vspace*{0.5cm}
\end{figure}

% The nW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2wN6.ps}\vspace*{-3.0cm}
\caption{La composante $wN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2wN6}\vspace*{0.5cm}
\end{figure}

% The wN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2wW7.ps}\vspace*{-3.0cm}
\caption{La composante $wW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2wW7}\vspace*{0.5cm}
\end{figure}

% The wW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2NW9.ps}\vspace*{-3.0cm}
\caption{La composante $NW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2NW9}\vspace*{0.5cm}
\end{figure}

% The NW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.


% In the limit of $n=w$, $N= W$and $\widehat{\alpha}=0.1$,
% under the second order of the higher derivative $\alpha^{\prime}$-corrections,
% we observe in the regime of $n \in (-10,0)$and $N \in (0,10)$that the
% amplitudes of the heat capacities $\{g_{nn}, g_{ww}\}$take a maximum value
% of the order $2 \times 10^{+09}$. In this range of the $n,N$, we find that
% the heat capacities $\{ g_{NN}, g_{WW}\}$in the range of $(0,14)$.
% As predicted at the first order $\alpha^{\prime}$-corrections, we see that
% the range of the growth of the first and the second sets of the heat capacities
% remains in the opposite limit of the parameters $\{n, N\}$. Explicitly, the
% Figs.(\ref{nonsusy2nn1}, \ref{nonsusy2ww5}), show that that the growth of the first
% sets of the heat capacities $\{ g_{nn}, g_{ww}\}$takes place in the limit of
% a large $N$and small $n$. Similarly, the Figs.(\ref{nonsusy2NN8}, \ref{nonsusy2WW10})
% show that the growth of the $\{ g_{NN}, g_{WW}\}$takes place in the limit of a small
% $N$and a large $n$. On the other hand, the heat compressibilities involving two
% distinct parameters of the non-supersymmetric black hole are depicted in the
% Figs.(\ref{nonsusy2nw2},\ref{nonsusy2nN3}, \ref{nonsusy2nW4}, \ref{nonsusy2wN6},
% \ref{nonsusy2wW7}, \ref{nonsusy2NW9}). In this case, we observe that the
% fluctuations involving $\{n, w\}$, as defined by the components of the
% state-space metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W\}$, have relatively
% larger numerical values than those involving $\{N, W\}$.

Dans la limite de $n= w$, $N= W$ et $\widehat{\alpha}= 0.1$, sous le second ordre des
corrections de d\'eriv\'ees sup\'erieures de $\alpha^{\prime}$, nous observons dans 
le r\'egime de $n \in (-10, 0)$ et $N \in (0, 10)$ que l'amplitudes des capacit\'es de
chaleurs $\{g_{nn}, g_{ww}\}$ prend la valeur maximale \`a l'ordre de $2 \times 10^{+09}$. 
Dans cette gamme de $\{n, N\}$, nous constatons que les capacit\'es de chaleurs $\{g_{NN}, g_{WW}\}$ 
restent dans la gamme de $(0, 14) $. Comme pr\'evu au premier ordre des corrections de $\alpha^{\prime} $, 
nous voyons que la gamme de la croissance de la premi\`ere ensemble et celle de la la deuxi\`eme ensemble des capacit\'es 
de chaleurs reste dans la limite oppos\'ee des param\`etres $\{n, N\}$ . Explicitement, les Figs. 
(\ref{nonsusy2nn1}, \ref{nonsusy2ww5}), montrent que la croissance de la premi\`ere ensemble des 
capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ a lieu dans la limite d'un grand $N$ et un petit $n$. 
De m\^{e}me, les Fig. (\ref{nonsusy2NN8}, \ref{nonsusy2WW10}) montrent que la croissance de 
$\{g_{NN}, g_{WW}\}$ a lieu dans la limite d'un petit $N$ et d'un grand $n$. D'autre part, 
les compressibilit\'es de chaleurs en impliquant deux param\`etres distincts de la configuration
des trous noirs non-supersym\'etriques sont d\'ecrits dans les Figs.(\ref{nonsusy2nw2},\ref{nonsusy2nN3},
\ref{nonsusy2nW4}, \ref{nonsusy2wN6},\ref{nonsusy2wW7}, \ref{nonsusy2NW9}). Dans ce cas, 
nous observons que les fluctuations en impliquant $\{n, w\}$, qui sont d\'efinies par les composantes 
de la m\'etrique tenseure de l'espace des etats $\{g_{ij} \ | \ i, j = n, w, N, W\}$, ont relativement
une grandes valeurs num\'eriques par rapport \`a celles qui impliquent des param\`etres $\{N, W\}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2detg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2detg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the function of 
% $n, N$, describing the fluctuations in the non-supersymmetric charged 
% black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2minor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2minor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2minor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$.} \label{nonsusy2minor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the second order stringy corrections.

% As the function of $n, N$, the ensemble stability of the ensemble
% follows from the positivity of the determinant of the metric tensor.
% In this case, we notice that the determinant of the metric tensor
% tends to a negative value. For a typical value of $n \in (-10,0)$
% and $N \in (0,10)$, the Fig.(\ref{nonsusy2detg}) shows that the
% determinant of the metric tensor lies in the interval $(-30,-100)$.
% The stability of the hypersurface defined by a constant value of $W$
% is shown in the Fig.(\ref{nonsusy2minor3}). Hereby, we see that the
% minor $p_3$lies in the range of $(-2.5 \times 10^{10}, 0)$. Notice
% that the negativity of $p_3$ increases as the value of $N$is increased
% from zero to $10$. Moreover, the surface defined by the fluctuations of
% $(n,w)$is unstable because of the fact that the corresponding principle
% minor vanishes identically, viz., we have $p_2=0$. When only the parameter
% $n$is allowed to vary, the stability of the black hole configuration
% as given by the positivity of the first principle minor $p_1:= g_{nn}$.
% A rotated view of $p_1$is shown in the Fig.(\ref{nonsusy2minor1}). 
% The above graphical state-space properties and positivity of the 
% concerned principle minors provide the qualitative notion of the 
% statistical stability of non-supersymmetric black holes in string theory.

Comme une fonction de $\{n, N\}$, la stabilit\'e de cet ensemble d\'ecoule de la 
positivit\'e du d\'eterminant de la m\'etrique tenseure. Dans ce cas, nous remarquons 
que le d\'eterminant de la m\'etrique tenseure tend vers une valeur n\'egative. 
Pour une valeur typique de $n \in (-10, 0) $ et $N \in (0, 10)$, la Fig. (\ref{nonsusy2detg}) 
montre que le d\'eterminant de la m\'etrique tenseure r\'eside dans l'intervalle $(-30, -100)$.
De plus, la stabilit\'e de l'hypersurface d\'efinie par une valeur constante de $W$
est montr\'e dans la Fig. (\ref{nonsusy2minor3}). Par la pr\'esente, nous voyons que le
mineur $p_3$ r\'eside dans la gamme de $(-2.5 \times 10^{10}, 0)$. Avis que la 
n\'egativit\'e de $p_3$ augmente \`a mesure que la valeur de $N$ est augment\'e
de z\'ero \`a $10$. Par ailleurs, la surface d\'efinie par les fluctuations de
$\{n, w\}$ est instable en raison du fait que le mineur principe correspondant est 
identiquement nulle, \`a savoir que nous avons $p_2= 0$. Lorsque seul le param\`etre
$n$ est autoris\'e \`a varier, la stabilit\'e de la configuration de ces trous noirs
est donn\'ee par la positivit\'e du premier mineur principe $p_1:= g_{nn}$.
Une vue rotat\'ee de $p_1$ est montr\'e dans la Fig. (\ref{nonsusy2minor1}).
Les vues graphiques ci-dessus de l'espace des \'etats et les propri\'et\'es de la positivit\'e des
mineurs principaux concern\'es fournent la notion qualitative de la stabilit\'e 
statistique des trous noirs non-supersym\'etriques.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2R.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$ dans la gamme
$n \in (-10,0)$ et $N \in (0,10) $.} \label{nonsusy2R}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the second order stringy corrections in the range 
% $n \in (-10,0)$and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy2R30.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
second ordre de $\alpha^{\prime}$ dans la gamme
$n, N \in (-30,30) $.} \label{nonsusy2R30}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the second order stringy corrections in the range 
% $n, N \in (-30,30)$.


% Similarly, the global stability properties follows from the
% behaviour of the state-space scalar curvature. In particular,
% in the range of $n \in (-10,0)$and $N \in (0,10)$, the
% Fig.(\ref{nonsusy2R}) shows that the scalar curvature has a large
% positive amplitude. We may note that the underlying black hole
% configuration is a strongly interacting statistical system. The
% positive sign of the scalar curvature signifies a repulsive nature
% of the statistical interactions. The Fig.(\ref{nonsusy2R30}) illustrates
% the nature of the above scalar curvature in an equal range of the parameters
% $n, N \in (-30,30)$. In fact, when the range of $n$and $N$is taken in
% the multiple of $3$, for example (-30, 30), then we see from the
% Fig.(\ref{nonsusy2R30}) that there exists four similar disjoint
% regions of the global statistical interactions. In comparison with
% the interactions appearing in the range of $n \in (-10,0)$and
% $N \in (0,10)$, the amplitude of the global statistical interactions
% turn out to be much smaller than those appearing in the range of
% $n, N \in (-30,30)$. As mentioned before for the the first order
% $\alpha^{\prime}$-corrections, the typical value of the amplitude
% of the state-space scalar curvatures appears to be $10^{-10}$.
% The graphical view of the above mentioned comparison follows from
% the Figs. (\ref{nonsusy2R}, \ref{nonsusy2R30}). Qualitatively,
% in the small values of the $n,N$, the above graphical depictions
% indicate that the non-supersymmetric black holes are unstable
% statistical configurations at the second order stringy corrections.

De plus, les propri\'et\'es de la stabilit\'e globale r\'esulte du
comportement de la courbure scalaire de l'espace des \'etats. En particulier,
dans la gamme de $n \in (-10, 0)$ et $N \in (0, 10)$, la Fig. (\ref{nonsusy2R}) 
montre que la courbure scalaire a une grande amplitude positive. On peut noter 
bien que la configuration des trous noirs sous-tendents est un syst\`eme statistique
fortement interagissant. Le signe positif de la courbure scalaire signifie la nature 
r\'epulsive des interactions statistiques. La Fig. (\ref{nonsusy2R30}) illustre
la nature de la courbure scalaire ci-dessus dans une range \'egale des param\`etres
$n, N \in (-30, 30)$. En fait, lorsque la gamme de $n$ et $N$ est prise en
le multiple de $3$, par exemple $(-30, 30)$, alors que nous voyons de la
Fig. (\ref{nonsusy2R30}) qu'il existe quatre r\'egions disjoints similaires
de l'interaction statistique globale. En comparaison des interactions apparaissant 
dans la gamme de $n \in (-10, 0)$ et $N \in (0, 10)$, l'amplitude des interactions 
statistiques globales se r\'ev\`elent \^{e}tre beaucoup plus petit ce qui figurant 
dans la gamme de $n, N \in (-30, 30)$. Comme mentionn\'e avant pour le cas de premier 
ordre des corrections de $\alpha^{\prime}$, le ration de la valeur typique de l'amplitude 
de ces courbures scalaires de l'espace des \'etats semble \^{e}tre $10^{-10}$. 
La vue graphique de la comparaison ci-dessus d\'ecoule par les Figs. 
(\ref{nonsusy2R}, \ref{nonsusy2R30}). Qualitativement, dans les petites valeurs 
de $n, N $, les repr\'esentations graphiques ci-dessus indiquent que ces trous noirs 
non-supersym\'etriques de la th\'eorie des cordes correspondent aux configurations 
statistiques instables aux corrections de second ordre de $\alpha^{\prime}$.



\subsection{Non-susy 3}


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3nn1.ps}\vspace*{-3.0cm}
\caption{La composante $nn$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3nn1}\vspace*{0.5cm}
\end{figure}

% The nn component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3ww5.ps}\vspace*{-3.0cm}
\caption{La composante $ww$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3ww5}\vspace*{0.5cm}
\end{figure}

% The ww component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3NN8.ps}\vspace*{-3.0cm}
\caption{La composante $NN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3NN8}\vspace*{0.5cm}
\end{figure}

% The NN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3WW10.ps}\vspace*{-3.0cm}
\caption{La composante $WW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3WW10}\vspace*{0.5cm}
\end{figure}

% The WW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3nw2.ps}\vspace*{-3.0cm}
\caption{La composante $nw$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3nw2}\vspace*{0.5cm}
\end{figure}

% The nw component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3nN3.ps}\vspace*{-3.0cm}
\caption{La composante $nN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3nN3}\vspace*{0.5cm}
\end{figure}

% The nN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3nW4.ps}\vspace*{-3.0cm}
\caption{La composante $nW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3nW4}\vspace*{0.5cm}
\end{figure}

% The nW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3wN6.ps}\vspace*{-3.0cm}
\caption{La composante $wN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3wN6}\vspace*{0.5cm}
\end{figure}

% The wN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3wW7.ps}\vspace*{-3.0cm}
\caption{La composante $wW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3wW7}\vspace*{0.5cm}
\end{figure}

% The wW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3NW9.ps}\vspace*{-3.0cm}
\caption{La composante $NW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3NW9}\vspace*{0.5cm}
\end{figure}

% The NW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

% As mentioned in the forgoing section, we shall continue to offer
% the graphical depictions in the limit of $n=w$, $N= W$and
% $\widehat{\alpha}=0.1$. Under the third order of the higher
% derivative $\alpha^{\prime}$-corrections, we find in the regime of
% $n \in (-10,0)$and $N \in (0,10)$that the amplitudes of the heat
% capacities $\{g_{nn}, g_{ww}\}$take a maximum value of the order
% $2 \times 10^{+09}$. In this range of the $n, N$, we observe that
% the heat capacities $\{ g_{NN}, g_{WW}\}$lies in the range of
% $(0, 70)$. As predicted at the second order
% $\alpha^{\prime}$-corrections, we see that the range of the growth
% of the first and the second sets of the heat capacities remains in
% the opposite limit of the parameters $\{n, N\}$. Explicitly, the
% Figs.(\ref{nonsusy3nn1}, \ref{nonsusy3ww5}), indicate that that
% the growth of the first sets of the heat capacities $\{ g_{nn},
% g_{ww}\}$takes place in the limit of a large $N$ and small $n$.
% This signifies that the higher derivative stringy corrections do
% not significantly change the behaviour of the thermodynamic
% configuration of non-supersymmetric black holes. Similarly, the
% Figs.(\ref{nonsusy3NN8}, \ref{nonsusy3WW10}) show that the growth
% of the $\{ g_{NN}, g_{WW}\}$takes place in the limit of a small
% $N$and a large $n$. On the other hand, the heat compressibilities
% involving two distinct parameters of a given non-supersymmetric
% black hole are depicted in the Figs.(\ref{nonsusy3nw2},
% \ref{nonsusy3nN3}, \ref{nonsusy3nW4}, \ref{nonsusy3wN6},
% \ref{nonsusy3wW7}, \ref{nonsusy3NW9}). At this order of the higher
% derivative stringy corrections, we notice that the fluctuations
% involving $\{n, w\}$, as defined by the components of the
% state-space metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W\}$, have
% relatively larger numerical values than those involving $\{N, W\}$.

Comme mentionn\'e dans la section pr\'ec\`edente, nous allons bien continuer 
\`a offrir les repr\'esentations graphiques dans la limite de $n=w$, $N= W$ et
$\widehat{\alpha}=0.1$. Sous les corrections du troisi\`eme ordre de $\alpha^{\prime}$, 
nous trouvons dans le r\'egime de $n \in (-10, 0)$ et $N \in (0,10)$ que l'amplitude 
des capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ prend la valeur maximale \`a l'ordre 
de $2 \times 10^{+09} $. Dans cette gamme de $\{n, N\}$, nous observons que les capacit\'es 
de chaleurs $\{g_{NN}, g_{WW}\}$ se situent dans la gamme de $(0, 70)$. Comme pr\'evu au 
second ordre des corrections de $\alpha^{\prime}$, nous voyons en ce cas aussi que la gamme 
de la premi\`ere ensemble et celle de la deuxi\`eme ensemble des capacit\'es de chaleurs 
reste dans la limite oppos\'ee des param\`etres $\{n, N\}$ . Explicitement, les Figs. 
(\ref{nonsusy3nn1}, \ref{nonsusy3ww5}) indiquent que la croissance de premier ensemble 
des capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ a lieu dans la limite d'un grand $N$ 
et un petit $n$. Cela signifie que les corrections de d\'eriv\'ees sup\'erieures ne modifient 
pas significativement le comportement thermodynamique de la configuration des trous noirs 
non-supersym\'etriques. De plus, les Figs. (\ref{nonsusy3NN8}, \ref{nonsusy3WW10}) montrent 
que la croissance de $\{g_{NN}, g_{WW}\}$ a lieu dans la limite d'un petit $N$ et d'un grand $n$. 
D'autre part, les compressibilit\'es de chaleurs en impliquant deux param\`etres distincts d'une 
configuration donn\'ee des trous noirs non-supersym\'etriques de la th\'eorie des cordes sont 
repr\'esent\'es dans les Figs. (\ref{nonsusy3nw2}, \ref{nonsusy3nN3}, \ref{nonsusy3nW4}, 
\ref{nonsusy3wN6}, \ref{nonsusy3wW7}, \ref{nonsusy3NW9}). A cet ordre des corrections de 
d\'eriv\'ees sup\'erieures de $\alpha^{\prime}$ aux trous noirs non-supersym\'etriques, 
nous remarquons que les fluctuations, en impliquant $\{n, w\}$, tel qu'elle sont 
d\'efinies par les composantes de la m\'etrique tenseure de l'espace des etats 
$\{g_{ij} \ | \ i, j = n, w, N, W\}$, ont relativement des plus grande valeurs 
num\'eriques en comparision de celles qui impliquant $\{N, W\}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3detg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3detg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the function of 
% $n, N$, describing the fluctuations in the non-supersymmetric charged 
% black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3minor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3minor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3minor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
troisi\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy3minor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the third order stringy corrections.


% As mentioned before, the ensemble stability of the ensemble of the
% system is determined as the function of $n, N$. This follows from
% the positivity of the determinant of the metric tensor. In this
% case, we find that the determinant of the metric tensor tends to a
% negative value. For a typical value of $n \in (-10, 0)$and $N \in
% (0,10)$, the Fig.(\ref{nonsusy3detg}) shows that the determinant
% of the metric tensor lies in the interval $(-80, -120)$. The
% stability of the hypersurface defined by a constant value of $W$
% is shown in the Fig.(\ref{nonsusy3minor3}). Hereby, we observe
% that the minor $p_3$lies in the range of $(-2.5 \times 10^{10},
% 0)$. Notice that the negativity of $p_3$increases as the value of
% $N$is increased from zero to $10$. Also, the surface defined by
% the fluctuations of $(n,w)$is unstable because of the fact that
% the corresponding principle minor vanishes identically, viz., we
% have $p_2=0$. When only the parameter $n$is allowed to vary, the
% stability of the black hole configuration as given by the positivity 
% of the first principle minor $p_1:= g_{nn}$. A rotated view of $p_1$
% is shown in the Fig.(\ref{nonsusy3minor1}). The above graphical 
% state-space properties and positivity of the concerned principle 
% minors provide the qualitative notion of the statistical stability 
% of non-supersymmetric black holes in string theory.

Comme mentionn\'e pr\'ec\'edemment, la stabilit\'e d'un ensemble de syst\`eme de ces 
trous noirs charg\'es non-supersym\'etriques peut \^etre d\'etermin\'ee comme la fonction 
de $\{n, N\}$. Cela d\'ecoule de la positivit\'e du d\'eterminant de la m\'etrique tenseure. 
Dans ce cas, nous constatons que le d\'eterminant de la m\'etrique tenseure tend vers une
valeur n\'egative. Pour une valeur typique de $n \in (-10, 0)$ et $N \in (0, 10) $, 
la Fig. (\ref{nonsusy3detg}) montre que le d\'eterminant de la m\'etrique tenseure r\'eside 
dans l'intervalle $(-80, -120)$. En outre, la stabilit\'e de l'hypersurface d\'efinie par une valeur 
constante de $W$ est montr\'e dans la Fig. (\ref{nonsusy3minor3}). Par la pr\'esente, 
nous observons que les mineurs $p_3$ r\'eside dans la gamme de $(-2.5 \times 10^{10}, 0)$. 
Notez que la n\'egativit\'e de $p_3$ augmente \`a mesure que la valeur de $N$ est pass\'ee 
de z\'ero \`a $10$. En outre, la surface d\'efinie par les fluctuations du $\{n, w\}$ est 
instable en raison du fait que le mineur principe correspondant est identiquement nulle, 
\`a savoir que nous avons $p_2= 0$. Lorsque le seul param\`etre $n$ est autoris\'e \`a varier, 
la stabilit\'e de la configuration des trous noirs charg\'es non-supersym\'etriques est donn\'e 
par la positivit\'e du premier mineur principe $p_1:= g_{nn}$. Une vue rotat\'ee de $p_1$ est 
montr\'ee dans la Fig. (\ref{nonsusy3minor1}). Les propri\'et\'es graphiques ci-dessus 
de l'espace des \'etats et la positivit\'e des mineurs principaux concern\'es fournent 
la notion qualitative de la stabilit\'e statistique des trous noirs non-supersym\'etriques 
corrig\'ees \`a l'ordre de troisi\`eme ordre de $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3R.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $\{n, N\}$, d\'ecrivant 
les fluctuations de la configuration des trous noirs charg\'es non-supersym\'etriques 
aux corrections de troisi\`eme ordre de $\alpha^{\prime}$ dans la gamme de 
$n \in (-10, 0)$ et $N \in (0,10) $.} \label{nonsusy3R}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the third order stringy corrections in the range 
% $n \in (-10,0)$and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy3R30.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $\{n, N\}$, d\'ecrivant 
les fluctuations de la configuration des trous noirs charg\'es non-supersym\'etriques 
aux corrections de troisi\`eme ordre de $\alpha^{\prime}$ dans la gamme de 
$n \in (-10,0)$ et $N \in (0,10) $.} \label{nonsusy3R30}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the third order stringy corrections in the range 
% $n, N \in (-30,30)$.

% The global stability properties follows from the behaviour of the
% state-space scalar curvature. In particular, in the range of $n
% \in (-10,0)$and $N \in (0,10)$, the Fig.(\ref{nonsusy3R}) offers
% that the scalar curvature has a large positive amplitude. We find
% that the underlying black hole configuration is a strongly
% interacting statistical system. The positive sign of the scalar
% curvature signifies a repulsive nature of the statistical
% interactions. The Fig.(\ref{nonsusy3R30}) signifies the nature of
% the above scalar curvature in an equal range of the parameters $n,
% N \in (-30,30)$. In fact, when the range of $n$and $N$is taken
% in the multiple of $3$, for example (-30, 30), then we notice from
% the Fig.(\ref{nonsusy3R30}) that there exists four similar
% disjoint regions of the global statistical interactions. In
% comparison with the interactions appearing in the range of $n \in
% (-10,0)$and $N \in (0,10)$, the amplitude of the global
% statistical interactions appears to be much smaller than those
% appearing in the range of $n, N \in (-30,30)$. As mentioned before
% at the the second order $\alpha^{\prime}$-corrections, we see that
% the typical value of the amplitude of the state-space scalar
% curvatures appears to be $10^{-10}$. In short, he graphical
% conclusion of the above mentioned comparison follows from the
% Figs. (\ref{nonsusy3R}, \ref{nonsusy3R30}). In small values of the
% parameters $n,N$, the aboveindicate that the
% non-supersymmetric black holes are unstable statistical
% configurations at the third order stringy corrections.


Les propri\'et\'es globales de la stabilit\'e statistique d\'ecoule par le comportement 
de la courbure scalaire de l'espace des \'etats. En particulier, dans la gamme de 
$n \in (-10, 0)$ et $N \in (0, 10)$, la Fig. (\ref{nonsusy3R}) offre que la courbure 
scalaire a une grande amplitude positive. Nous trouvons que la configuration sous-jacente 
des trous noirs est un syst\`eme statistique fortement interagissant. Le signe positif de
la courbure scalaire signifie une nature r\'epulsive des interactions statistiques. 
La Fig. (\ref{nonsusy3R30}) signifie la nature de la courbure scalaire ci-dessus dans une 
range \'egale des param\`etres $n, N \in (-30,30)$. En fait, lorsque la gamme de $n$ et $N$
est prise dans les multiples de $3$, par exemple $(-30, 30)$, nous remarquons par la Fig. 
(\ref{nonsusy3R30}) qu'il existe quatre r\'egions similaires disjointes des interactions 
statistiques globales. En comparaison des interactions apparaissant dans la gamme de $n \in
(-10, 0)$ et $N \in (0,10) $, les interactions statistiques globales semble \^{e}tre beaucoup 
plus petits de celles qui apparaissant dans la gamme de $n, N \in (-30, 30)$. Comme mentionn\'e 
pr\'ec\'edemment au second ordre des corrections de $\alpha^{\prime}$, nous voyons que le ration de
la valeur typique de l'amplitude de la courbure scalaire de l'espace des \'etats semble \^{e}tre $10^{-10}$. 
En bref, la conclusion graphique de la comparaison ci-dessus d\'ecoule des Figs. (\ref{nonsusy3R}, 
\ref{nonsusy3R30}). Dans le cas des petite valeur des param\`etres $n, N$, nous voyons que 
les trous noirs non-supersym\'etriques sont int\'eractifs et correspondent \`a une 
configuration statistique instable sous le troisi\`eme ordre de $\alpha^{\prime}$.


\subsection{Non-susy 4}


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4nn1.ps}\vspace*{-3.0cm}
\caption{La composante $nn$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4nn1}\vspace*{0.5cm}
\end{figure}

% The nn component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4ww5.ps}\vspace*{-3.0cm}
\caption{La composante $ww$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4ww5}\vspace*{0.5cm}
\end{figure}

% The ww component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4NN8.ps}\vspace*{-3.0cm}
\caption{La composante $NN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4NN8}\vspace*{0.5cm}
\end{figure}

% The NN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4WW10.ps}\vspace*{-3.0cm}
\caption{La composante $WW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4WW10}\vspace*{0.5cm}
\end{figure}

% The WW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4nw2.ps}\vspace*{-3.0cm}
\caption{La composante $nw$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4nw2}\vspace*{0.5cm}
\end{figure}

% The nw component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4nN3.ps}\vspace*{-3.0cm}
\caption{La composante $nN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4nN3}\vspace*{0.5cm}
\end{figure}

% The nN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4nW4.ps}\vspace*{-3.0cm}
\caption{La composante $nW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4nW4}\vspace*{0.5cm}
\end{figure}

% The nW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4wN6.ps}\vspace*{-3.0cm}
\caption{La composante $wN$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4wN6}\vspace*{0.5cm}
\end{figure}

% The wN component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4wW7.ps}\vspace*{-3.0cm}
\caption{La composante $wW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4wW7}\vspace*{0.5cm}
\end{figure}

% The wW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4NW9.ps}\vspace*{-3.0cm}
\caption{La composante $NW$ de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4NW9}\vspace*{0.5cm}
\end{figure}

% The NW component of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.


% As at the previous order stringy corrections, for the
% case of $n=w$, $N= W$and $\widehat{\alpha}=0.1$,
% we observe for $n \in (-10,0)$and $N \in (0,10)$that the
% amplitudes of the heat capacities $\{g_{nn}, g_{ww}\}$take
% a maximum value of the order $2 e+09$. While, the heat capacities
% $\{ g_{NN}, g_{WW}\}$take a typical value between $(0,90)$.
% This shows that the fourth order $\alpha^{\prime}$-corrected
% non-supersymmetric black holes are locally stable statistical
% configurations. In fact, the range of the growth of the first
% and the second sets of the heat capacities happens to be in the
% opposite limit of the parameters $\{n, N\}$. Explicitly, from the
% Figs.(\ref{nonsusy4nn1}, \ref{nonsusy4ww5}), we find that that the
% of growth of the heat capacities $\{ g_{nn}, g_{ww}\}$takes place
% in the limit of a large $N$ and small $n$. On the other hand, the
% Figs.(\ref{nonsusy4NN8}, \ref{nonsusy4WW10}) show that the growth of
% $\{ g_{NN}, g_{WW}\}$ takes place in the limit of small $N$and large $n$.
% Similarly, the heat compressibilities involving two distinct parameters
% of the black hole have been depicted in the Figs.(\ref{nonsusy4nw2},
% \ref{nonsusy4nN3}, \ref{nonsusy4nW4}, \ref{nonsusy4wN6}, \ref{nonsusy4wW7},
% \ref{nonsusy4NW9}). In this case, we may note that the Fig. \ref{nonsusy4NW9}
% shows an unique feature of $NW$-component of the statistical fluctuations
% for the non-supersymmetric black holes. As defined by the components of
% the state-space metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W\}$, the
% fourth order $\alpha^{\prime}$-corrections indicate that the fluctuations
% involving the parameters $\{n, w\}$ have relatively larger numerical values
% with respect to those involving the parameters $\{N, W\}$.

Comme \`a la correction pr\'ec\'edente des d\'eriv\'ees sup\'erieure de troisi\`eme ordre de 
$\alpha^{\prime}$, pour la cas de $n= w$, $N= W$ et $\widehat{\alpha}= 0.1$, nous observons pour 
$n \in (-10, 0)$ et $N \in (0, 10)$ que l'amplitude des capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ 
se prend la valeur maximale \`a l'ordre de $2 \times 10^+{09}$. Alors, les capacit\'es de chaleurs 
$\{g_{NN}, {g_ WW}\}$ prennent une valeur typique dans l'intervalle $(0, 90)$. Cela montre que 
les trous noirs non-supersym\'etriques corrig\'es par des corrections quatri\`eme ordre de 
$\alpha^{\prime}$ correspondent \`a une configuration statistique localement stable. En fait, 
les gammes de la croissance de la premi\`ere ensemble et celle la deuxi\`eme ensemble des capacit\'es 
de chaleurs se trouvent \^{e}tre dans la limite oppos\'ee des param\`etres $\{n, N\}$. 
Explicitement, par les Figs. (\ref{nonsusy4nn1}, \ref{nonsusy4ww5}), nous constatons que la croissance 
des capacit\'es de chaleurs $\{g_{nn}, g_{ww}\}$ a lieu dans la limite d'un grand $N$ et un petit $n$. 
D'autre part, les Figs. (\ref{nonsusy4NN8}, \ref{nonsusy4WW10}) montrent que la croissance des 
$\{g_{NN}, g_{WW}\}$ a lieu dans la limite d'un petit $N$ et un grand $n$. De m\^eme, les compressibilit\'es 
de chaleurs en comprenant deux param\`etres distincts de ces trous noirs sont repr\'esent\'ees dans les 
Figs. (\ref{nonsusy4nw2}, \ref{nonsusy4nN3}, \ref{nonsusy4nW4}, \ref{nonsusy4wN6}, \ref{nonsusy4wW7},
\ref{nonsusy4NW9}). Dans ce cas, on peut bien noter que la Fig. (\ref{nonsusy4NW9}) montre une 
caract\'eristique unique de la composante $NW$ des fluctuations statistiques des trous noirs
non-supersym\'etriques. Les composantes tel qui sont d\'efinies par les composantes de la m\'etrique 
tenseure de l'espace des \'etats $\{g_{ij} \ | \ i, j = n, w, N, W\}$, le quatri\`eme ordre des corrections 
de $\alpha^{\prime}$ indiquent que les fluctuations, en impliquant les param\`etres $\{n, w\}$, 
prennent relativement des plus grande valeurs num\'eriques par rapport \`a celles qui sont d\'efinies 
ci-dessus en impliquant les param\`etres $\{N, W\}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4g.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4g}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the function of 
% $n, N$, describing the fluctuations in the non-supersymmetric charged 
% black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4minor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4minor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4minor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $\{n, N\}$, d\'ecrivant les fluctuations de la configuration
des trous noirs charg\'es non-supersym\'etriques aux corrections de 
quatri\`eme ordre de $\alpha^{\prime}$.} \label{nonsusy4minor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $n, N$, describing the fluctuations in the non-supersymmetric 
% charged black holes at the fourth order stringy corrections.


% As the function of $n, N$, the ensemble stability condition of the
% fourth order $\alpha^{\prime}$-corrected non-supersymmetric black holes
% follows from the positivity of the determinant of the metric tensor.
% In this case, we see that the determinant of the metric tensor
% generically tends to a negative value. For a typical value of
% $n \in (-10,0)$and $N \in (0,10)$, the Fig.(\ref{nonsusy4g})
% shows that the determinant of the metric tensor lies in the interval
% $(-80,-140)$. Hereby, for $N \in (2,10)$, we see that the determinant
% of the metric tensor has an approximate value of $-97$. In the interval
% $N \in (0,2)$, the determinant of the metric tensor first increases
% to a value of $-80$and sharply reduces to a value of $-140$.
% The corresponding stability of the hypersurface defined by a constant
% value of $W$is shown in the Fig.(\ref{nonsusy4minor3}).
% In this range on $n,N$, we see that the minor $p_3$lies in the range
% of $(-2 \times 10^{10}, 0)$. In the limit of a small $n$, we find that the
% negativity of $p_3$increases as the value of $N$is increased from
% zero to $10$. Moreover, the surface defined by the fluctuations of the
% $(n,w)$is unstable because the corresponding principle minor vanishes
% identically, viz., we have $p_2=0$. When only the parameter $n$is
% allowed to vary, the stability of the configuration is determined
% by the positivity of the first principle minor $p_1:= g_{nn}$. In this case,
% for small $n$and large $N$, we observe from the Fig.(\ref{nonsusy4minor1})
% that $p_1$has a positive amplitude of the order $10^{10}$. In fact, for a small
% value of $n$, thefirst principle minor $p_1$increases as the function of $N$.
% Thus, the above graphical descriptions of the state-space principle minors provide
% qualitative notion of the statistical stability at the fourth order stringy
% $\alpha^{\prime}$-corrections to the non-supersymmetric black holes.

Comme une fonction de $\{n, N\}$, la condition de stabilit\'e d'un ensemble des trous noirs
non-supersym\'etriques corrig\'es au quatri\`eme ordre de $\alpha^{\prime}$ d\'ecoule 
de la positivit\'e du d\'eterminant de la m\'etrique tenseure. Dans ce cas, nous voyons 
que le d\'eterminant de la m\'etrique tenseure tend d'une fa\c{c}on g\'en\'erique \`a une valeur 
n\'egative. Pour une valeur typique de $n \in (-10, 0)$ et $N \in (0, 10) $, la Fig. (\ref{nonsusy4g})
montre que le d\'eterminant de la m\'etrique tenseure r\'eside dans l'intervalle $(-80, -140)$. 
Par la pr\'esente, pour $N \in (2, 10) $, nous voyons que le d\'eterminant de la m\'etrique tenseure 
a une valeur approximative de $-97$. Dans l'intervalle $N \in (0, 2) $, le d\'eterminant de la 
m\'etrique tenseure \`a tout d'abord augmente \`a une valeur de $-80$ et puis il r\'eduit fortement 
\`a une valeur de $-140$. La stabilit\'e correspondante de l'hypersurface d\'efinie par une valeur 
constante de $W$ est montr\'e dans la Fig. (\ref{nonsusy4minor3}). Dans cette gamme de $\{n, N\}$, 
nous voyons que le mineur $p_3$ r\'eside dans la gamme de $(-2 \times 10^{ +10}, 0)$. 
Dans la limite d'un petit $n$, nous constatons que la n\'egativit\'e de $p_3$ augmente 
\`a mesure que la valeur de $N$ est pass\'ee de z\'ero \`a $10$. Par ailleurs, la surface 
d\'efinie par les fluctuations de $\{n, w\}$ est instable par-ce que les mineurs principe 
correspondant dispara\^{i}t identiquement, \`a savoir que nous avons $p_2= 0$. Lorsque le seul 
param\`etre $n$ est autoris\'e \`a varier, la stabilit\'e de la configuration est d\'etermin\'ee
par la positivit\'e du premier mineur principe $p_1:= g_{nn}$. Dans ce cas, pour un petit $n$ et
un grand $N$, on peut observer par la Fig. (\ref{nonsusy4minor1}) que $p_1$ a une amplitude 
positive \`a l'ordre de $10^{+10}$. En fait, pour une petite valeur de $n$, le premier mineur
principe $p_1$ augmente \`a mesure que la fonction de $N$. Ainsi, les descriptions graphiques 
ci-dessus des mineurs principaux de l'espace des \'etats fournent la notion qualitative de la 
stabilit\'e statistique des trous noirs non-supersym\'etriques sous les quatri\`eme ordre 
des corrections de $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4R.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $\{n, N\}$, d\'ecrivant 
les fluctuations de la configuration des trous noirs charg\'es non-supersym\'etriques 
aux corrections de quatri\`eme ordre de $\alpha^{\prime}$ dans la gamme 
$n \in (-10, 0)$ et $N \in (0,10) $.} \label{nonsusy4R}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the fourth order stringy corrections in the range 
% $n \in (-10,0)$and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonsusy4R30.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $\{n, N\}$, d\'ecrivant 
les fluctuations de la configuration des trous noirs charg\'es non-supersym\'etriques 
aux corrections de quatri\`eme ordre de $\alpha^{\prime}$ dans la gamme 
$n, N \in (-30,30)$.} \label{nonsusy4R30}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $n, N$, 
% describing the fluctuations in the non-supersymmetric charged 
% black holes at the fourth order stringy corrections in the range 
% $n, N \in (-30,30)$.

% Under the higher derivative $\alpha^{\prime}$-correction of order four,
% the global stability properties of the non-supersymmetric black holes
% are shown in the Figs. (\ref{nonsusy4R}, \ref{nonsusy4R30}). In the
% range of $n \in (-10,0)$and $N \in (0,10)$, it follows from the
% Figs. (\ref{nonsusy4R}) that the state-space scalar curvature acquires
% a peak of order $10^{08}$ in the limit of small $n, N$. In fact,
% in the limit of a small $n$, the Figs. (\ref{nonsusy4R}) shows that
% the scalar curvature decreases as the function of $N$. In particular,
% ii the small value of both the $n,N$, the Fig.(\ref{nonsusy4R}) shows
% that the scalar curvature has a large positive amplitude of the order
% $10^{08}$. Thus, we may note that the underlying black hole configuration
% is a strongly interacting statistical system in this limit of the charges.
% As mentioned in the previous cases, the fourth order higher derivative
% $\alpha^{\prime}$-corrections yield the positive sign of the scalar
% curvature. This signifies that the black hole is repulsive interactions.
% The Fig.(\ref{nonsusy4R30}) illustrates the nature of the above scalar
% curvature in an equal range of the $n, N \in (-30,30)$. Namely,
% when the range of $n$and $N$is taken in the multiple of $3$,
% for example (-30, 30), then we see from the Fig.(\ref{nonsusy4R30})
% that there are four similar disjoint regions of the global statistical
% interactions. In comparison with the interactions appearing in the
% range of $n \in (-10,0)$and $N \in (0,10)$, the amplitude of the
% interactions remains much smaller for the range of $n, N \in (-30,30)$.
% The typical value of the ratio of the amplitude of the scalar curvatures
% appears to be a factor of $10^{-10}$. The graphical view of this comparison
% is shown the Figs. (\ref{nonsusy4R}, \ref{nonsusy1R30}). Qualitatively,
% in the small values of the $n,N$, the above graphical depictions of the
% scalar curvatures indicate that the non-supersymmetric black holes are
% unstable statistical configurations at the fourth order
% $\alpha^{\prime}$-corrections.

\`A quatri\`eme ordre des corrections de d\'eriv\'ee sup\'erieures de $\alpha^{\prime}$,
les propri\'et\'es de la stabilit\'e globale des trous noirs non-supersym\'etriques sont 
pr\'esent\'es dans les . Fig. (\ref{nonsusy4R}, \ref{nonsusy4R30}). Dans la gamme de 
$n \in (-10, 0)$ et $N \in (0, 10)$, il r\'esulte de la Fig. (\ref{nonsusy4R}) que la 
courbure scalaire de l'espace des \'etats acquiert un pic \`a l'ordre de $10^{+08}$ dans la 
limite d'une petite valeur de $n, N$. En fait, dans la limite d'un petit $n$, la Fig. (\ref{nonsusy4R}) 
montre que la courbure scalaire diminue \`a mesure que la fonction de $N$. En particulier,
dans la cas de petite valeur de $\{n, N\}$, la Fig. (\ref{nonsusy4R}) montre que la courbure 
scalaire a une grande amplitude positive \`a l'ordre de $10^{+08}$. Ainsi, on peut noter que 
la configuration des trous noirs sous-tendents est un syst\`eme statistique fortement interagissant
dans cette limite des charges. Comme mentionn\'e dans les cas pr\'ec\'edents, le quatri\`eme ordre 
des corrections de d\'eriv\'es sup\'erieures de $\alpha^{\prime}$ rend le signe positif \`a la 
courbure scalaire. Cela signifie que la configuration statistique de ces trous noirs a des 
interactions r\'epulsives. La Fig. (\ref{nonsusy4R30}) illustre la nature de la courbure 
scalaire ci-dessus dans une range \'egale de $n, N \in (-30,30)$. \`A savoir, quand $n$ et 
$N$ prennent des valeurs en multiple de $3$, par exemple $(-30, 30)$, alors que nous voyons 
de la Fig. (\ref{nonsusy4R30}) qu'il y a quatre r\'egions disjointes similaire des interactions
statistiques globales. En comparaison des interactions apparaissant dans la gamme de 
$n \in (-10,0)$ et $N \in (0, 10) $, l'amplitude des interactions demeure \`a une beaucoup plus petite 
valeur dans la gamme de $n, N \in (-30,30)$. Le ration de la valeur typique de l'amplitude de ces courbures scalaires
semble \^{e}tre \`a l'ordre de $10^{-10}$. La vue graphique de cette comparaison est montr\'e dans
les Figs. (\ref{nonsusy4R}, \ref{nonsusy4R30}). Qualitativement, dans le cas des petites valeurs 
de $\{n, N\}$, les repr\'esentations graphiques ci-dessus de la courbure scalaire indiquent que les 
trous noirs non-supersym\'etriques sont globalement une configuration statistique instable 
bien qu'on aie ajout\'e le quatri\`eme ordre des corrections de $\alpha^{\prime}$.



% DONE TILL HERE




\section{Les solutions non-extr\'emalaux de branes noirs}


\subsection{Nonextremal $D_1 D_5$}

\subsubsection{\`A l'ordre dominant}

% At leading order 

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextN1N1.ps}\vspace*{-3.0cm}
\caption{La composante $N_1N_1$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextN1N1}\vspace*{0.5cm}
\end{figure}

% The $N_1 N_1$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextN5N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextN5N5}\vspace*{0.5cm}
\end{figure}

% The $N_5 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextNRNR.ps}\vspace*{-3.0cm}
\caption{La composante $N_RN_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextNRNR}\vspace*{0.5cm}
\end{figure}

% The $N_RN_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextN1N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_1N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextN1N5}\vspace*{0.5cm}
\end{figure}

% The $N_1N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextN1NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_1N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextN1NR}\vspace*{0.5cm}
\end{figure}

% The $N_1N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextN5NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextN5NR}\vspace*{0.5cm}
\end{figure}

% The $N_5N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.


% Since there are three number of independent variables, thus in
% order to offer three dimensional , we shall work in the
% limit of $N_1=N$, $N_5=N$and $N_R= W$. For a given $D_1 D_5$
% nonextremal black hole, the fluctuations properties can be
% expressed by the following . Namely, in the regime of $N
% \in (0, 10)$and $W \in (0,10)$, we observe that the amplitudes of
% the heat capacities $\{g_{N_1 N_1}, g_{N_5 N_5}\}$take a value
% of the order $25$. In this range of $N, W$, the heat capacities
% $\{ g_{N_R N_R}\}$lies in the range of $(0, 120)$. As per the
% prediction of the state-space geometry, we find that the range of
% the growth of the first and the second sets of the heat capacities
% remains in the opposite limit of the parameters $\{N, W\}$.
% Specifically, for a given small value of $N$, the first set of
% heat capacities increase for the increasing value of $W$. However,
% for a given small value of $W$, the component $g_{N_R N_R} $
% increases for the increasing value of $N$. In this concern, the
% Figs.(\ref{nonextN1N1}, \ref{nonextN5N5}), show that that the
% growth of the first sets of heat capacities $\{ g_{N_1 N_1},
% g_{N_5 N_5}\}$takes place in the limit of a large $W$ and small
% $N$. Similarly, the Fig.(\ref{nonextNRNR}) shows that the growth
% of the $\{ g_{N_R N_R}\}$takes place in the limit of a small $W$
% and a large $N$. Similarly, the heat compressibilities involving
% two distinct parameters of the black hole are depicted in the
% Figs.(\ref{nonextN1N5},\ref{nonextN1NR}, \ref{nonextN5NR}). In
% fact, we find that the amplitude of (i) $g_{N_1 N_5}$ is of the
% order $-25$, (ii) $g_{N_1 N_R}$ is of the order $-5$and (iii)
% $g_{N_5 N_R}$is also of the order $-5$. Hereby, the state-space
% metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W\}$as depicted in
% the Figs.(\ref{nonextN1N1}, \ref{nonextN5N5}, \ref{nonextNRNR})
% show that the leading order nonextremal $D_1 D_5$black holes
% correspond a locally stable statistical configuration with a set
% of positive heat capacities.

Puisqu'il y a trois variables ind\'ependantes, c'est \`a dire que nous avons
les nombres $\{N_1, N_5, N_R \}$, et donc en afin d'offrir les vues graphiques 
de trois dimensions, nous allons consid\'erer dans la limite de $N_1= N$, $N_5 = N$ 
et $N_R = W$. Pour une configuration donn\'ee des trous noirs $D_1 D_5$ nonextremaux, 
les propri\'et\'es des fluctuations peuvent \^{e}tre exprim\'ees par les charact\'erisation 
suivantes. Notamment, dans le r\'egime de $N \in (0, 10)$ et $W \in (0, 10)$, on observe que 
l'amplitudes des les capacit\'es de chaleurs $\{g_{N_1 N_1}, g_{N_5 N_5}\}$ prennent une valeur 
\`a l'ordre de $25$. Dans cette gamme de $N, W$, la capacit\'e de chaleur $\{g_{N_R N_R}\}$ 
se situe dans la gamme de $(0, 120)$. Conform\'ement \`a la pr\'ediction de la g\'eom\'etrie 
de l'espace des \'etats, nous constatons que les gammes de croissance de la premi\`ere ensemble 
et celle de la deuxi\`eme ensemble des capacit\'es de chaleurs restent dans la limite oppos\'ee 
des param\`etres $\{N, W\}$. Plus pr\'ecis\'ement, pour une petite valeur donn\'ee de $N$, 
la premi\`ere s\'erie des capacit\'es de chaleurs augmente quand on augmente la valeur de $W$. 
Cependant, pour une petite valeur donn\'ee de $W$, la composante $g_{N_R N_R}$ augmente 
quand on augmente la valeur de $N$. Dans cette pr\'eoccupation, les Figs. (\ref{nonextN1N1}, 
\ref{nonextN5N5}) montrent que la croissance de premier ensemble des capacit\'es de chaleurs 
$\{g_{N_1 N_1}, g_{N_5 N_5}\}$ est li\'ee dans la limite d'un grand $W$ et un petit $N$. 
Du fait m\^{e}me, la Fig. (\ref{nonextNRNR}) montre que la croissance de $\{g_{N_R N_R}\}$
se situe dans la limite d'un petit $W$ et un grand $N$. De plus, les compressibilit\'es
de chaleurs en impliquant deux param\`etres distincts de la configuration des trous noirs
sous-jacents sont repr\'esent\'es dans les Figs. (\ref{nonextN1N5},\ref{nonextN1NR}, \ref{nonextN5NR}). 
En fait, nous constatons que l'amplitude de (i) $g_{N_1 N_5}$ est \`a l'ordre de $-25$, 
(ii) $g_{N_1 N_R}$ est \`a l'ordre de $-5$ et (iii) $g_{N_5 N_R}$ est aussi \`a l'ordre de $-5$. 
Par la pr\'esente, la m\'etrique tenseure de l'espace des \'etats $\{g_{ij} \ | \ i, j = N_1, N_5, N_R\}$ 
tel qu'elle est d\'ecrite dans les Figs. (\ref{nonextN1N1}, \ref{nonextN5N5}, \ref{nonextNRNR}) ce qui
est montr\'ee \`a l'ordre dominant de la configuration des trous noirs $D_1 D_5 $ nonextremaux, 
correspond \`a un ensemble statistique localement stable avec une positive valeur des 
capacit\'es de chaleurs. 

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextdetg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextdetg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre dominant.} \label{nonextminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the leading order.


% Under the fluctuations of the parameters $\{N_1, N_5, N_R\}$, the
% ensemble stability of the nonextremal $D_1 D_5$black holes
% follows from the positivity of the determinant of the metric
% tensor. For the choice of $N_1=N$, $N_5=N$and $N_R= W$, we find
% that the determinant of the metric tensor $g$ceases to a large
% negative value as we decrease the parameters $\{N, W\}$. In this
% case, we find that $g \in (-500, 0)$. For a typical value of $N
% \in (0, 10)$and $W \in (0,10)$, the Fig.(\ref{nonextdetg}) offers
% the graphical nature of the determinant of the metric tensor $g$.
% Furthermore, the surface defined by the fluctuations of $\{N_1,
% N_5\}$is unstable because the corresponding principle minor
% vanishes identically, viz., we have $p_2=0$. Finally, when only
% the parameter $N_1$is allowed to vary, the stability of the black
% hole is given by the positivity of the first principle minor
% $p_1:= g_{N_1 N_1}$. A rotated view of $p_1$is shown in the
% Fig.(\ref{nonextminor1}). The above state-space properties and
% positivity of the concerned principle minors describes qualitative
% behaviour of the statistical stability of the nonextremal $D_1
% D_5$ black holes.

Sous les fluctuations des param\`etres $\{N_1, N_5, N_R\}$, la stabilit\'e 
d'un ensemble de la configuration des trous noirs $D_1 D_5$ nonextremaux
d\'ecoule de la positivit\'e du d\'eterminant de la m\'etrique tenseure. 
Pour le choix de $N_1= N$, $N_5= N$ et $W= N_R$, nous trouvons que le 
d\'eterminant de la m\'etrique tenseure $g$ prend une grande valeur n\'egative 
quand nous diminuons les param\`etres $\{N, W\}$. Dans ce cas, nous constatons que 
$g \in (-500, 0)$. Pour une valeur typique de $N \in (0, 10)$ et $W \in (0,10)$, 
la Fig. (\ref{nonextdetg}) offre la nature graphique du d\'eterminant de la m\'etrique 
tenseure $g$. En outre, la surface d\'efinie par les fluctuations de $\{N_1, N_5\}$ 
est instable par-ce que le mineur principe correspondant est identiquement nulle, \`a savoir que
nous avons $p_2= 0$. Enfin d'alors que le seulement le param\`etre $N_1$ est autoris\'e \`a varier, 
la stabilit\'e de la configuration des trous noirs $D_1 D_5$ nonextremaux est donn\'ee par la 
positivit\'e du premier principe mineur $p_1:= g_{N_1 N_1}$. Une vue rotat\'ee de $p_1$ est 
pr\'esent\'ee dans la Fig. (\ref{nonextminor1}). Les propri\'et\'es ci-dessus de l'espace 
des \'etats et la positivit\'e des mineurs principaux concern\'es d\'ecritent le comportement 
qualitative de la stabilit\'e statistique d'un ensemble des trous noirs $D_1D_5 $ nonextremaux
ce qui sont d\'efinis par la th\'eorie des cordes.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextR.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs charg\'es 
nonextremaux $D_1 D_5 $ \`a l'ordre dominant dans la gamme des charges
$N, W \in (0, 10)$.} \label{nonextR}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_1 D_5$charged 
% black holes at the leading order in the range of the charges
% $N, W \in (0, 10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextR10.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs charg\'es 
nonextremaux $D_1 D_5 $ \`a l'ordre dominant dans la gamme des charges
$N, W \in (-10, 10)$.} \label{nonextR10}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_1 D_5$charged 
% black holes at the leading order in the range of the charges
% $N, W \in (-10, 10)$.


% As mentioned in the previous chapter, the state-space scalar
% curvature offers the global statistical properties under the
% fluctuation of the $\{N_1, N_5, N_R\}$. In the range of $N \in (0,
% 10)$and $W \in (0, 10)$, the Fig.(\ref{nonextR}) shows that the
% scalar curvature has a small positive amplitude of the order
% $0.5$. In this range of the parameters, we observe that the
% underlying black hole configuration is a weakly interacting
% statistical system. Physically, the positive sign of the scalar
% curvature signifies that the statistical interactions are
% repulsive in their nature. The Fig.(\ref{nonextR10}) illustrates
% the behaviour of the above scalar curvature for range of the
% parameters $N, W \in (-10, 10)$. In fact, we see that the
% interactions are largely present near about the line $N=0$and the
% state-space scalar curvature acquires a large peak of order $4
% \times 10^{+07}$at the origin $(N,W)= (0, 10)$. In the small the
% range of $N$and $W$we notice from the Fig.(\ref{nonextR10}) that
% the global statistical interactions are symmetric about the line
% $N=0$. In comparison with the interactions appearing in the range
% of $N, W \in (0,10)$, the amplitude of the global statistical
% interactions turn out to be much larger in the range of $n, N \in
% (-10, 10)$. Precisely, we find that the ratio of typical values of
% the amplitude of the state-space scalar curvatures is of the order
% $10^{-08}$. The graphical view of the above mentioned comparison is
% apparent from the plots Figs.(\ref{nonextR}, \ref{nonextR10}).
% Qualitatively, from the state-space depictions, we observe that the
% nonextremal $D_1 D_5$ black holes are globally unstable interacting
% statistical configurations at the leading order two derivative 
% gravity theory.

Comme mentionn\'e dans le chapitre pr\'ec\'edent, la courbure scalaire 
de l'espace des \'etats offre les propri\'et\'es statistiques globales 
sous la fluctuation d'une configuration des trous noirs charg\'es 
$D_1 D_5 $ nonextremaux en terme de $\{N_1, N_5, N_R\}$. Dans la gamme de 
$N \in (0, 10)$ et $W \in (0, 10)$, la Fig. (\ref{nonextR}) montre que 
la courbure scalaire a une petite amplitude positive de l'ordre de $0.5$. 
Dans cette gamme de param\`etres, nous observons que la configuration 
sous-jacente de ces trous noirs $D_1 D_5$ nonextremaux est un syst\`eme 
statistique faiblement interactive. Physiquement, le signe positif de la 
courbure scalaire signifie que les interactions statistiques sont r\'epulsives 
dans la leur nature. La Fig. (\ref{nonextR10}) illustre le comportement de la 
courbure scalaire ci-dessus pour la range des param\`etres $N, W \in (-10, 10)$. 
En fait, nous voyons que les interactions sont largement pr\'esents pr\`es de la 
ligne $N= 0$ et la courbure scalaire de l'espace des \'etats acquiert un grand 
pic \`a l'ordre de $4 \times 10^{+07}$ pr\`es de l'origine $(N, W) = (0, 0)$. 
Dans la gamme d'un petit $W$ et un petit $N$, nous remarquons de la Fig. (\ref{nonextR10}) 
que les interactions statistiques globales sont sym\'etriques autour de la ligne $N= 0$. 
En comparaison des interactions apparaissant dans la gamme de $N, W \in (0, 10)$, 
l'amplitude des interactions statistiques globales se r\'ev\`elent d'\^{e}tre beaucoup 
plus grande dans la gamme de $N, W \in (-10, 10) $. Pr\'ecis\'ement, nous constatons que 
le ratio des valeurs typiques de l'amplitude de ces courbures scalaires de l'espace des \'etats 
est \`a l'ordre de $10^{-08}$. La vue graphique de cette comparaison ci-dessus mentionn\'ee 
est apparente par les Figs. (\ref{nonextR}, \ref{nonextR10}). Qualitativement, par les 
repr\'esentations de l'espace des \'etats, nous observons que la configuration des trous 
noirs $D_1D_5$ nonextremaux sont interactives au niveau globale, et elles correspond \`a 
un syst\`eme statistique instable dans des deux d\'eriv\'es de la gravit\'e.


\subsubsection{\`A l'ordre de $\alpha^{\prime}$}

% At the order of $\alpha^{\prime}$



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaN1N1.ps}\vspace*{-3.0cm}
\caption{La composante $N_1N_1$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaN1N1}\vspace*{0.5cm}
\end{figure}

% The $N_1 N_1$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaN5N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaN5N5}\vspace*{0.5cm}
\end{figure}

% The $N_5 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaNRNR.ps}\vspace*{-3.0cm}
\caption{La composante $N_RN_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaNRNR}\vspace*{0.5cm}
\end{figure}

% The $N_RN_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the order of $\alpha^{\prime}$.



\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaN1N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_1N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaN1N5}\vspace*{0.5cm}
\end{figure}

% The $N_1N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaN1NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_1N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaN1NR}\vspace*{0.5cm}
\end{figure}

% The $N_1N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaN5NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaN5NR}\vspace*{0.5cm}
\end{figure}

% The $N_5N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_1 D_5$
% charged black holes at the order of $\alpha^{\prime}$.

% Following the convention of the graphs of the previous section, we
% shall continue to work with $N_1=N$, $N_5=N$and $N_R= W$. This
% offers the three dimensional depiction of the fluctuations
% properties of $\alpha^{\prime}$corrected $D_1 D_5$nonextremal
% black holes. In the regime of $N \in (0, 10)$and $W \in (0, 10)$,
% we find that the amplitudes of the heat capacities $\{g_{N_1 N_1},
% g_{N_5 N_5}\}$take a value of the order $30$. In this range of
% $N, W$, the heat capacities $\{ g_{N_R N_R}\}$lies in the range
% of $(0, 120)$. As per the prediction of the $\alpha^{\prime}$
% corrected state-space geometry, we observe that the range of the
% growth of the first and the second sets of the heat capacities
% remains in the opposite limit of the parameters $\{N, W\}$.
% Specifically, we find that the $\alpha^{\prime}$corrections do
% not alter graphical nature of heat capacities. In fact, for a
% given small value of $N$, we may notice that the first set of heat
% capacities $\{g_{N_1 N_1}, g_{N_5 N_5}\}$increase when we
% increase the value of $W$. Similarly, for a given small value of
% $W$, we observe that the heat capacity $g_{N_R N_R} $increases
% when we increase the value of $N$. In this case, the
% Figs.(\ref{nonextalphaN1N1}, \ref{nonextalphaN5N5}), show that
% that the growth of the first sets of heat capacities $\{ g_{N_1
% N_1}, g_{N_5 N_5}\}$takes place in the limit of a large $W$and
% small $N$. Similarly, the Fig.(\ref{nonextalphaNRNR}) shows that
% the growth of the $\{ g_{N_R N_R}\}$takes place in the limit of a
% small $W$and a large $N$. It is worth mentioning that the heat
% capacities find a set of positive numerical values. On the other
% hand, the Figs.(\ref{nonextalphaN1N5}, \ref{nonextalphaN1NR},
% \ref{nonextalphaN5NR}) depict the heat compressibilities involving
% two distinct parameters of the $\alpha^{\prime}$corrected
% nonextremal $D_1 D_5$black holes. Hereby, we notice that the
% amplitude of (i) $g_{N_1 N_5}$is of the order $-22$, (ii) $g_{N_1
% N_R}$is of the order $-5$and (iii) $g_{N_5 N_R}$is also of the
% order $-5$. As shown in the Figs.(\ref{nonextalphaN1N1},
% \ref{nonextalphaN5N5}, \ref{nonextalphaNRNR}), the state-space
% metric tensor $\{g_{ij}\ |\ i, j= N_1, N_5, N_R\}$ illustrate that
% the $\alpha^{\prime}$corrected nonextremal $D_1 D_5$black holes
% correspond a locally stable statistical configuration.

En suivant la convention des graphiques de la section pr\'ec\'edente, 
nous allons continuer \`a la consid\'eration de $N_1= N$, $N_5= N$ et $N_R= W$. 
\c{C}a offre une repr\'esentation des propri\'et\'es de la fluctuation en trois 
dimensions de la configuration des trous noirs $D_1 D_5$ nonextremaux sous les
corrections de $\alpha^{\prime}$. Dans le r\'egime de $N \in (0, 10)$ et $W \in (0, 10)$,
nous trouvons que l'amplitudes des capacit\'es de chaleurs $\{g_{N_1 N_1},
g_{N_5 N_5}\}$ prend une valeur \`a l'ordre de $30$. Dans cette gamme de
$N, W$, les capacit\'es de chaleurs $\{g_{N_R N_R}\}$ est dans l'intervalle $(0, 120)$. 
En conformant \`a la pr\'ediction de lag\'eom\'etrie de l'espace des \'etats
sous lec corrections de $\alpha^{\prime}$, on observe que l'augmentation de l'amplitude
de la premi\`ere ensemble et celle de la deuxi\`eme ensemble des capacit\'es de chaleurs
reste dans la limite oppos\'ee des param\`etres $\{N, W\}$. Plus pr\'ecis\'ement, 
nous constatons que les corrections de $\alpha^{\prime}$ ne modifie pas la nature graphique 
des capacit\'es de chaleurs. En fait, pour une petite valeur donn\'ee de $N$, nous pouvons noter 
que la premi\`ere s\'erie des capacit\'es de chaleurs $\{g_{N_1 N_1}, g_{N_5 N_5}\}$ augmente,
quand nous augmentons la valeur de $W$. Du fait m\^{e}me, pour une valeur donn\'ee petite de $W$, 
on observe que la capacit\'e thermique $g_{N_R N_R}$ augmente lorsque nous augmentons la valeur de $N$. 
Dans ce cas, les Figs. (\ref{nonextalphaN1N1}, \ref{nonextalphaN5N5}) montrent que
la croissance de premier ensemble des capacit\'es de chaleurs $\{g_{N_1N_1}, g_{N_5 N_5}\}$ 
a lieu dans la limite d'un grand $W$ et un petite $N$. De plus, la Fig. (\ref{nonextalphaNRNR}) 
montre que l'amplitude de $\{g_{N_R N_R}\}$ a lieu dans la limite d'un petit $W$ et un grand $N$. 
Il est \`a noter que les capacit\'es de chaleurs de cet ensemble trouvent des positives num\'eriques
valeurs. D'autre part, les Figs. (\ref{nonextalphaN1N5}, \ref{nonextalphaN1NR},
\ref{nonextalphaN5NR}) r\'epresentent les compressibilit\'es de chaleurs en impliquant
deux param\`etres distincts de la configuration des trous noirs $D_1 D_5$ nonextremaux sous
les corrections de $\alpha^{\prime}$. Par la pr\'esente, nous remarquons que l'amplitude de (i) 
$g_{N_1 N_5} $ est \`a l'ordre de $-22$, (ii) $g_{N_1N_R}$ est \`a l'ordre de $-5$ et (iii) 
$g_{N_5 N_R}$ est aussi \`a l'ordre de $-5$. Comme nous avons montr\'e dans les Figs. 
(\ref{nonextalphaN1N1}, \ref{nonextalphaN5N5}, \ref{nonextalphaNRNR}), la m\'etrique 
tenseure de l'espace des \'etats $\{g_{ij} \ | \ i, j = N_1, N_5, N_R\}$ illustre le fait 
que les corrcetions de $\alpha^{\prime}$ \`a la configuration des trous noirs $D_1 D_5$ 
nonextremaux correspondent \`a un syst\`eme statistique localement stable.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphadetg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphadetg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_1 D_5$charged black holes 
% at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaminor2.ps}\vspace*{-3.0cm}
\caption{Le mineur de surface de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaminor2}\vspace*{0.5cm}
\end{figure}

% The surface minor of the metric tensor plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_1 D_5$charged black holes 
% at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_1 D_5 $ 
\`a l'ordre de $\alpha^{\prime}$.} \label{nonextalphaminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_1 D_5$charged black holes 
% at the order of $\alpha^{\prime}$.


% Under the fluctuations of the parameters $\{N_1, N_5, N_R\}$, the
% ensemble stability of the nonextremal $D_1 D_5$ black holes can be
% described from the positivity of the determinant of the metric
% tensor $g$. For the $\alpha^{\prime}$corrected nonextremal $D_1
% D_5$black holes with $N_1=N$, $N_5=N$and $N_R= W$, we find that
% the determinant of the metric tensor $g$ceases to a large
% negative value, as we decrease the parameters $\{N, W\}$. This
% shows that the higher derivative stringy corrections do not yield
% statistical stability. In this case, we may observe also that $g
% \in (-500, 0)$. For a typical value of $N \in (0, 10)$and $W \in
% (0, 10)$, the Fig.(\ref{nonextalphadetg}) describes the graphical view
% of the determinant of the metric tensor $g$. Interestingly, the
% surface defined by the fluctuations of $\{N_1, N_5\}$ becomes
% stable under the $\alpha^{\prime}$corrections. This follows from
% the positivity of the corresponding principle minor vanishes
% $p_2$. The graphical view of the minor $p_2$ is shown in the
% Fig.(\ref{nonextalphaminor2}). In this case, we find that $p_2$
% lies in the range of $(0, 330)$. For a given small value of $N$,
% notice that the positivity of $p_2$increases as the value of $W$
% from zero to $10$. Finally, when only the parameter $N_1$ is
% allowed to vary, the stability of the black hole is given by the
% positivity of the first principle minor $p_1:= g_{N_1 N_1}$. With
% a different orientation, the graphical view of the minor $p_1$ is
% shown in the Fig.(\ref{nonextalphaminor1}). The above state-space
% properties and positivity of the principle minors describes
% qualitative behaviour of the statistical fluctuation of the
% $\alpha^{\prime}$ corrected nonextremal $D_1 D_5$black holes.

Sous les fluctuations des param\`etres $\{N_1, N_5, N_R\}$, la stabilit\'e d'un
ensemble de la configuration des trous noirs $D_1 D_5$ nonextremaux peut \^{e}tre
d\'ecrite de la positivit\'e du d\'eterminant de la m\'etrique tenseure $g$. 
Sous les corrections de $\alpha^{\prime}$ \`a la configuration des trous noirs
$D_1D_5$ nonextremaux avec $N_1= N$, $N_5= N$ et $W= N_R$, nous constatons que
le d\'eterminant de la m\'etrique tenseure $g$ prend une grande valeur n\'egative, 
quand nous diminuons les param\`etres $\{N, W\}$. \c{C}a montre que les corrections 
des d\'eriv\'es sup\'erieures de la th\'eorie des cordes ne donnent pas la stabilit\'e 
statistique aux trous noirs $D_1D_5$ nonextremaux. Dans ce cas, on peut aussi constater
que $g \in (-500, 0)$. Pour une valeur typique de $N \in (0, 10)$ et $W \in (0, 10)$, 
la Fig. (\ref{nonextalphadetg}) d\'ecrit la vue graphique du d\'eterminant de la m\'etrique 
tenseure $g$. Fait int\'eressant, la surface d\'efinie par les fluctuations de $\{N_1, N_5\}$ 
devient stable sous les corrections de $\alpha^{\prime}$. Cela d\'ecoule de la positivit\'e 
de mineur principe correspondant $p_2 $. La vue graphique de $p_2$ est montr\'e dans la
Fig. (\ref{nonextalphaminor2}). Dans ce cas, nous constatons que $p_2 $ r\'eside dans la 
gamme de $(0, 330)$. Pour une petite valeur donn\'ee de $N$, notez bien que la positivit\'e 
de $p_2$ augmente \`a mesure que nous augmentons la valeur de $W$ de z\'ero \`a $10$. 
Enfin, lorsque le seul param\`etre $N_1$ est autoris\'e \`a varier, la stabilit\'e de la
configuration des trous noirs est donn\'ee par la positivit\'e du premier mineur principe 
$p_1:= g_{N_1 N_1}$. Avec une orientation diff\'erente, la vue graphique du mineur $p_1$
est montr\'e dans la Fig. (\ref{nonextalphaminor1}). Les propri\'et\'es ci-dessus de l'espace 
des \'etats et la positivit\'e des mineurs principaux d\'ecritent le comportement qualitatif 
des fluctuations statistiques de la configuration des trous noirs $D_1 D_5$ nonextremaux
sous les corrections de $\alpha^{\prime}$. 

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaR.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
charg\'es nonextremaux $D_1 D_5 $ \`a l'ordre de $\alpha^{\prime}$ dans la gamme des charges
$N, W \in (0, 10)$.} \label{nonextalphaR}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_1 D_5$charged black holes 
% at the order of $\alpha^{\prime}$in the range of the charges
% $N, W \in (0, 10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{nonextalphaR10.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
charg\'es nonextremaux $D_1 D_5 $ \`a l'ordre de $\alpha^{\prime}$ dans la gamme des charges
$N, W \in (-10, 10)$.} \label{nonextalphaR10}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_1 D_5$charged black holes 
% at the order of $\alpha^{\prime}$in the range of the charges
% $N, W \in (-10, 10)$.

% As mentioned in the previous chapter, the state-space description
% remains valid under the higher derivative stringy corrections.
% Namely, the scalar curvature offers the global properties of the
% statistical fluctuation. In the range $N \in (0, 10)$and $W \in
% (0, 10)$, we observe from the Fig.(\ref{nonextalphaR}) that the
% the scalar curvature has a small positive amplitude of the order
% $0.4$. In this range of the parameters $\{N_1, N_5, N_R\}$, we
% find that the $\alpha^{\prime}$corrected nonextremal $D_1 D_5$
% black holes correspond to a weakly interacting statistical
% configuration. As mentioned before, the positive sign of the
% state-space scalar curvature signifies that the statistical
% interactions are repulsive in their character. Furthermore, the
% Fig.(\ref{nonextalphaR10}) illustrates the behaviour of the above
% scalar curvature for the range of the parameters $N, W \in (-10,
% 10)$. Precisely, we see that the interactions are largely present
% near about the line $N=0$and the state-space scalar curvature
% acquires a small peak of order $0.15$at the origin $(N,W)= (0,
% 0)$. In the small the range of $N$and $W$, we observe from the
% Fig.(\ref{nonextalphaR10}) that the global statistical
% interactions are symmetric about the line $N=0$. In comparison
% with the interactions appearing in the range of $N, W \in (0,10)$,
% the amplitude of the global scalar curvature turn out to be
% smaller in the range of $N, W \in (-10, 10)$. Also, from the
% Figs.(\ref{nonextalphaR}, \ref{nonextalphaR10}), we find that the
% state-space scalar curvatures in both the above intervals remains
% almost of the same order. Qualitatively, the state-space
% depictions indicate that the $\alpha^{\prime}$corrected
% nonextremal $D_1 D_5$ black holes are globally unstable weakly
% interacting statistical configurations. In short, the leading
% order higher derivative $\alpha^{\prime}$ correction improve the
% stability of fluctuating nonextremal $D_1 D_5$ configurations by
% (i) offering a positive surface minor $p_2$ and (ii) reducing the
% peak of scalar curvature.

Comme mentionn\'e dans le chapitre pr\'ec\'edent, la description de la
g\'eom\'etrie de l'espace des \'etats reste valable en vertu des corrections 
d\'eriv\'eesup\'erieures de $\alpha^{\prime}$. A savoir, la courbure scalaire 
offre les propri\'et\'es globales des fluctuations statistiques. Dans la gamme de 
$N \in (0, 10)$ et $W \in (0, 10)$, on observe de la Fig. (\ref{nonextalphaR}) que 
la courbure scalaire a une petite positive amplitude \`a l'ordre de $0.4$. 
Dans cette gamme des param\`etres $\{N_1, N_5, N_R\}$, nous constatons que les
trous noirs $D_1 D_5$ nonextremaux corrig\'es par les termes de $\alpha^{\prime}$ 
correspondent \`a une configuration statistique faiblement interactive. 
Comme mentionn\'e pr\'ec\'edemment, le signe positif de la courbure scalaire 
de l'espace des \'etats signifie que les interactions statistiques sont r\'epulsives 
dans la leur caract\`ere. En outre, la Fig. (\ref{nonextalphaR10}) illustre le 
comportement de ce qui pr\'ec\`ede, voil\`a, la courbure scalaire dans la gamme 
des param\`etres $N, W \in (-10, 10) $. Justement, nous voyons que les interactions 
sont largement pr\'esentes pr\`es de la ligne $N= 0$, et la courbure scalaire sous-jacente 
de l'espace des \'etats acquiert un petit pic \`a l'ordre de $0.15$ pr\`es de 
l'origine $(N, W)= (0,0)$. Dans une petite gamme de $N$ et $W$, on observe de 
la Fig. (\ref{nonextalphaR10}) que les interactions statistiques globales sont 
sym\'etriques autour de la ligne $N= 0$. En comparaison des interactions 
apparaissant dans la gamme de $N, W \in (0, 10)$, l'amplitude de la courbure scalaire 
globale se r\'ev\'ele plus petits dans la gamme de $n, N \in (-10, 10) $. 
Aussi, \`a partir des Figs. (\ref{nonextalphaR}, \ref{nonextalphaR10}), nous constatons que 
la courbure scalaire de l'espace des \'etats dans ces deux intervalles ci-dessus reste
pr\`es du m\^{e}me ordre. Qualitativement, les repr\'esentations de l'espace des \'etats
indiquent que la configuration des trous noirs $D_1D_5$ nonextremaux corrig\'ee par
les termes de $\alpha^{\prime}$  correspond \`a un syst\`eme statistique faiblement 
interagissant et globalement instable. En bref, les corrections de d\'eriv\'ees sup\'erieures
de $\alpha^{\prime}$ am\'eliorent la stabilit\'e de la configuration des trous noirs
$D_1 D_5$ nonextremaux. C'est \`a dire, sous les fluctuation de $\{N_1, N_5, N_R\}$, 
les corrections de $\alpha^{\prime}$ viennet (i) en offrant une surface de l'espace 
des \'etats avec une positive valeur de mineur $p_2$ et (ii) en r\'eduissant le sommet 
sous-jacent de la courbure scalaire.

\subsection{Nonextremal $D_2 D_6 NS_5$}

% Non-extremal= Non-extr\'emaux

\subsubsection{A l'ordre dominant}
% At the leading order

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N2N2.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_2$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N2N2}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_2$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N6N6.ps}\vspace*{-3.0cm}
\caption{La composante $N_6N_6$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N6N6}\vspace*{0.5cm}
\end{figure}

% The $N_6 N_6$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N5N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N5N5}\vspace*{0.5cm}
\end{figure}

% The $N_5 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5NRNR.ps}\vspace*{-3.0cm}
\caption{La composante $N_RN_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5NRNR}\vspace*{0.5cm}
\end{figure}

% The $N_R N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N2N6.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_6$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N2N6}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_6$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N2N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N2N5}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N2NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N2NR}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N6N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_6N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N6N5}\vspace*{0.5cm}
\end{figure}

% The $N_6 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N6NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_6N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N6NR}\vspace*{0.5cm}
\end{figure}

% The $N_6 N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5N5NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5N5NR}\vspace*{0.5cm}
\end{figure}

% The $N_5 N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

% In this case, since there are four number of independent variables, 
% thus in order to offer three dimensional view of the statistical properties, 
% we consider the setting $N_2=N$, $N_6=N$, $N_5= W$and $N_R= W$. 
% For a given $D_2 D_6 NS_5$nonextremal black hole, the fluctuations 
% properties can be expressed by the following set of . Namely, 
% in the regime of $N \in (0, -10)$and $W \in (0, 10)$, we see that the 
% amplitudes of the heat capacities $\{g_{N_2 N_2}, g_{N_6 N_6}\}$take 
% the values of the order $4 \times 10^{+09}$. In this range of $N, W$, 
% the heat capacities $\{g_{N_5 N_5}, g_{N_R N_R}\}$lies in the range 
% $(0, 80)$. As per the prediction of the state-space geometry, we observe 
% that the range of the growth of the first set of the and the second sets 
% of the heat capacities remains in the opposite limit of the parameters 
% $\{N, W\}$. Specifically, for a given small value of $N$, the first set
% of heat capacities increase when $W$increases. However, for a given 
% small value of $W$, the other set of components increase when the value
% of $N$increases. In this concern, the Figs.(\ref{d2d6ns5N2N2}, \ref{d2d6ns5N6N6}),
% show that that the growth of the first sets of heat capacities $\{ g_{N_2 N_2},
% g_{N_6 N_6}\}$takes place in the limit of a large $W$and small $|N|$. 
% Similarly, the Figs.(\ref{d2d6ns5N5N5}, \ref{d2d6ns5NRNR}) show that the growth
% of the $\{ g_{N_5 N_5}, g_{N_R N_R}\}$takes place in the limit of the 
% small $W$and large $|N|$. Similarly, the heat compressibilities involving
% two distinct parameters of the black hole are depicted in the
% Figs.(\ref{d2d6ns5N2N6},\ref{d2d6ns5N2N5}, \ref{d2d6ns5N2NR}, 
% \ref{d2d6ns5N6N5}, \ref{d2d6ns5N6NR}, \ref{d2d6ns5N5NR}). In
% this case, we find that (i) the amplitude of $g_{N_2 N_6}$is of the
% order $-4 \times 10^{+09}$, (ii) $g_{N_2 N_5}$, $g_{N_6 N_5}$,
% $g_{N_6 N_R}$and $g_{N_2N_R}$remain in the interval $(-3, 3)$
% and (iii) $g_{N_5 N_R}$leis in the interval $(0, -80)$. 
% Thus, the graphical depiction of the state-space metric tensor 
% $\{g_{ij}\ |\ i, j= N_2, N_6, N_5, N_R\}$shows that the leading 
% order nonextremal $D_2 D_6 NS_5$black holes possess a set of 
% positive heat capacities, and thus they correspond a locally 
% stable statistical configuration.

Dans ce cas, puisqu'il y a quatre variables ind\'ependantes, c'est \`a dire
que nous avous les nombre $\{N_2, N_6, N_5, N_R\}$, et ainsi, dans le but d'offrir 
une vue tridimensionnelle des propri\'et\'es statistiques, nous consid\'erons la 
mise de $N_2= N$, $N_6= N$, $N_5= W$ et $N_R= W$. Pour une configuration donn\'ee 
des trous noirs $D_2 D_6 NS_5$ nonextremaux, la propri\'et\'e des fluctuations peut 
\^{e}tre exprim\'ee par l'ensemble suivant. \`A savoir, dans le r\'egime de 
$N \in (0, -10)$ et $W \in (0, 10)$, nous voyons que l'amplitude des capacit\'es 
de chaleurs $\{g_{N_2 N_2}, g_{N_6 N_6}\}$ prend les valeurs \`a l'ordre de 
$4 \times 10^{+09}$. Dans cette gamme de $N, W$, les capacit\'es de chaleurs 
$\{g_{N_5 N_5}, g_{N_R N_R}\}$ restent dans l'intervalle $(0, 80) $. Conform\'ement, 
\`a la pr\'ediction de la g\'eom\'etrie de l'espace des '\'etats, nous observons que 
les gammes de la premi\`ere s\'erie et celle de la seconde s\'erie des capacit\'es de 
chaleurs restent dans la limite opposite des param\`etres $\{N, W\}$. Plus pr\'ecis\'ement, 
pour une petite valeur donn\'ee de $N$, la premi\`ere s\'erie des capacit\'es de chaleurs 
augmente lorsqu'on augmente le param\'etre $W$. Cependant, pour une petite valeur donn\'ee
de $W$, l'autre s\'erie des composantes augmentent lorsqu'on augmente la valeur $N$. 
Dans ce cas, les Figs. (\ref{d2d6ns5N2N2}, \ref{d2d6ns5N6N6}) montrent que la croissance 
de premier ensemble des capacit\'es de chaleurs $\{g_{} N_2 N_2, g_{N_6 N_6}\}$ a lieu dans 
la limite d'un grand $W$ et un petit $|N|$. Du fait m\^{e}me, les Figs. (\ref{d2d6ns5N5N5}, 
\ref{d2d6ns5NRNR}) montrent que la croissance de $\{g_{N_5 N_5}, g_{N_R N_R}\}$ a lieu dans 
la limite d'un petit $W$ et un grand $|N|$. De plus, les compressibilit\'es de chaleurs en
impliquant deux param\`etres distincts de la configuration des trous noirs sous-jacents 
sont repr\'esent\'es dans les Figs. (\ref{d2d6ns5N2N6},\ref{d2d6ns5N2N5}, \ref{d2d6ns5N2NR}, 
\ref{d2d6ns5N6N5}, \ref{d2d6ns5N6NR}, \ref{d2d6ns5N5NR}). Dans ce cas, nous constatons que 
l'amplitude de (i) $g_{N_2 N_6} $ reste environt de $-4 \times 10^{09}$, 
(ii) $g_{N_2 N_5} $, $g_{N_6 N_5} $, $g_{N_6 N_R}$ et $g_{N_2N_R}$ reste 
dans l'intervalle $(-3, 3)$ et (iii) $g_{N_5 N_R} $ reste dans l'intervalle $(0, -80)$.
Ainsi, la repr\'esentation graphique de la m\'etrique tenseure de l'espace des \'etats
$\{g_{ij} \ | \ i, j = N_2, N_6, N_5, N_R\}$ montre que la configuration des trous noirs 
$D_2 D_6 NS_5$ nonextremaux, \`a l'ordre dominant de $\alpha^{\prime}$ de la th\'eorie de cordes, 
poss\`ede un ensemble des capacit\'es de chaleurs positives, et donc elle correspond \`a un 
syst\`eme statistique stables au niveau local.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5minor3.ps}\vspace*{-3.0cm}
\caption{La mineur d'hypersurface de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5minor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5minor1.ps}\vspace*{-3.0cm}
\caption{La premier mineur de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre dominant.} \label{d2d6ns5minor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order.

% Under the fluctuations of the parameters $\{N_2, N_6, N_5, N_R\}$, 
% the ensemble stability of the nonextremal $D_2 D_6 NS_5$black holes
% follows from the positivity of the determinant of the metric tensor. 
% For the choice of $N_2=N$, $N_5=N$and $N_R= W$, we find that the 
% determinant of the metric tensor $g$remains to constant negative value. 
% In this case, it turns out that the numerical value of $g$is $-16\pi^4$. 
% Furthermore, the stability of the hypersurface defined by a constant value 
% of $N_R$is shown in the Fig.(\ref{d2d6ns5minor3}). Hereby, we see that the 
% minor $p_3$lies in the range of $(-1.6 \times 10^{11}, 0)$. For a given small
% value of $N$, we notice that the negativity of $p_3$decreased as the value 
% of the parameter $N$is increased from zero to $10$. Similarly, the surface 
% defined by the fluctuations of $\{N_2, N_6\}$is unstable because of the fact
% that the corresponding principle minor vanishes identically, viz., $p_2=0$. 
% Finally, when only the parameter $N_1$is allowed to vary, we find that 
% the stability of the black hole is given by the positivity of the first 
% principle minor $p_1:= g_{N_2 N_2}$. A rotated view of $p_1$is shown 
% in the Fig.(\ref{d2d6ns5minor1}). The above state-space properties and 
% positivity of the principle minors offer qualitative behaviour of the 
% statistical stability of the nonextremal $D_2D_6 NS_5$ black holes.

Sous les fluctuations des param\`etres $\{N_2, N_6, N_5, N_R\}$,
la stabilit\'e d'un ensemble des trous noirs $D_2 D_6 NS_5$ nonextremaux 
d\'ecoule de la positivit\'e du d\'eterminant de la m\'etrique tenseure.
Pour le choix des param\`etres $N_2= N$, $N_5= N$ et $W= N_R$, nous constatons 
que le d\'eterminant de la m\'etrique tenseure $g$ reste \`a une constante valeur 
n\'egative. Dans ce cas, il s'av\`ere que la valeur num\'erique de $g$ est $-16 \pi^4$.
Par ailleurs, la stabilit\'e de l'hypersurface d\'efinie par une valeur constante de 
$N_R$ est montr\'e dans la Fig. (\ref{d2d6ns5minor3}). Par la pr\'esente, nous voyons 
que le mineur $p_3$ r\'eside dans la gamme de $(-1.6 \times 10^{+11}, 0)$. 
Pour une petite valeur donn\'ee de $N$, on remarque que la n\'egativit\'e de $p_3$
diminu\'e quand la valeur du param\`etre $N$ est pass\'ee de z\'ero \`a $10$. 
Du plus, la surface d\'efinies par les fluctuations de $\{N_2, N_6\}$ est instable 
en raison du fait que le mineur principe correspondant est identiquement nulle, \`a savoir que
nous avons $p_2= 0$. Enfin, lorsque le seul param\`etre $N_1$ est autoris\'e \`a varier, 
nous constatons que la stabilit\'e de la configuration des trous noirs sous-jacents est donn\'ee 
par la positivit\'e de premier mineur principe $p_1:= g_{N_2 N_2}$. Une vue rotat\'ee de $p_1$
est donn'ee dans la Fig. (\ref{d2d6ns5minor1}). Ci-dessus, les propri\'et\'es de l'espace des 
\'etats et la positivit\'e des mineurs principaux offrent le comportement qualitatif de la
stabilit\'e statistique de la configuration des trous noirs $D_2D_6 NS_5$ nonextremaux.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5R.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
charg\'es nonextremaux $D_2 D_6 NS_5$ \`a l'ordre dominant dans la gamme
$n \in (-10,0)$ et $N \in (0,10)$.} \label{d2d6ns5R}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order in the range 
% $n \in (-10,0)$ and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5R10.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
charg\'es nonextremaux $D_2 D_6 NS_5$ \`a l'ordre dominant dans la
gamme $n, N \in (-10, 10)$.} \label{d2d6ns5R10}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the leading order in the range 
% $n, N \in (-10, 10)$.

% As mentioned in the previous case, the state-space scalar curvature 
% offers the global statistical properties under the fluctuation of the 
% parameter $\{N_2, N_6, N_5, N_R\}$. In the range of $N \in (0, -10)$
% and $W \in (0, 10)$, the Fig.(\ref{d2d6ns5R}) shows that the scalar 
% curvature has a large positive amplitude of the order $8 \times 10^{+07}$. 
% In this range of the parameters, we observe that the underlying black hole 
% configuration is a strongly interacting statistical system. Physically, 
% the positive sign of the scalar curvature signifies that the statistical 
% interactions are repulsive in their nature. The Fig.(\ref{d2d6ns5R10}) 
% illustrates the behaviour of the above scalar curvature for range of the
% parameters $N, W \in (-10, 10)$. In the range of $N \in (0, -10)$
% and $W \in (0, 10)$, we see that the interactions are largely present 
% near about the line $N=0$. In the range of $N, W \in (-10, 10)$,
% the state-space scalar curvature acquires a large peak of order 
% $4 \times 10^{+30}$at the origin $(N,W)= (0, 0)$. In the small the 
% range of $N$and $W$, we notice from the Fig.(\ref{d2d6ns5R10}) that
% the global statistical interactions are only present at the origin.
% In comparison with the interactions appearing in the range of the
% parameters $N, W \in (0,10)$, we see that the amplitude of the 
% global statistical interactions turn out to be much larger in 
% the range of $n, N \in (-10, 10)$. Precisely, it follows that 
% the ratio of typical values of the amplitude of the state-space 
% scalar curvatures is of the order $10^{-23}$. The graphical view 
% of the above mentioned comparison is apparent from the plots 
% Figs.(\ref{d2d6ns5R}, \ref{d2d6ns5R10}). Qualitatively, the 
% state-space depictions indicate that the nonextremal 
% $D_2D_6 NS_5$black holes are globally unstable strongly
% interacting statistical configurations.

Comme mentionn\'e dans le cas pr\'ec\'edent, la courbure scalaire d'espace 
d'\'etats offre les propri\'et\'es statistiques globales sous la fluctuation 
des param\`etres $\{N_2, N_6, N_5, N_R\}$. Dans la gamme de $N \in (0, -10)$
et $W \in (0, 10) $, la Fig. (\ref{d2d6ns5R}) montre que la scalaire courbure 
sous-jacente a une grande amplitude positive \`a l'ordre de $8 \times 10^{+07}$. 
Dans cette gamme des param\`etres, nous observons que la configuration sous-jacente
des trous noirs est un syst\`eme statistique fortement interagissant. Physiquement,
le signe positif de la courbure scalaire signifie que les interactions statistiques
sont r\'epulsives dans la leur nature. La Fig. (\ref{d2d6ns5R10}) illustre le comportement 
de la courbure scalaire ci-dessus pour la range des param\`etres $N, W \in (-10, 10)$. 
Dans la gamme de $N \in (0, -10) $ et $W \in (0, 10) $, nous voyons que les interactions 
sont largement pr\'esents pr\`es de la ligne $N = 0 $. Dans la gamme de $N, W \in (-10, 10)$,
la courbure scalaire de l'espace des \'etats acquiert un grand pic \`a l'ordre de $4 \times 10^{30}$
pr\`es de l'origine $(N, W) = (0, 0)$. Dans la gamme de petit $N$ et un petit $W$, on constate 
de la Fig. (\ref{d2d6ns5R10}) que les interactions statistiques globales ne sont pr\'esents pr\`es de 
l'origine. En comparaison des interactions apparaissant dans la gamme des param\`etres $N, W \in (0,10)$, 
nous voyons que l'amplitude des interactions statistiques globales se r\'ev\`ele \^{e}tre beaucoup 
plus grande dans la gamme de $N, W \in (-10, 10) $. Pr\'ecis\'ement, il s'ensuit que le ratio des 
valeurs typiques de l'amplitude de ces courbures scalaires de l'espace des \'etats est \`a l'ordre 
de $10^{-23}$. La vue graphique de la comparaison mentionn\'e ci-dessus est montr\'ee par les Figs. 
(\ref{d2d6ns5R}, \ref{d2d6ns5R10}). Qualitativement, les repr\'esentations de l'espace des \'etats
indiquent que la configuration des trous noirs $D_2D_6NS_5$ nonextremaux de la th\'eorire des cordes 
correspond \`a un syst\`eme statistique globalement instable et fortement interactive. 


\subsubsection{\`A l'ordre de $\alpha^{\prime}$}

% At the order $\alpha^{\prime}$

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN2N2.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_2$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN2N2}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_2$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN6N6.ps}\vspace*{-3.0cm}
\caption{La composante $N_6N_6$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN6N6}\vspace*{0.5cm}
\end{figure}

% The $N_6 N_6$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN5N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN5N5}\vspace*{0.5cm}
\end{figure}

% The $N_5 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaNRNR.ps}\vspace*{-3.0cm}
\caption{La composante $N_RN_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaNRNR}\vspace*{0.5cm}
\end{figure}

% The $N_R N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN2N6.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_6$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN2N6}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_6$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN2N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN2N5}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN2NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_2N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN2NR}\vspace*{0.5cm}
\end{figure}

% The $N_2 N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN6N5.ps}\vspace*{-3.0cm}
\caption{La composante $N_6N_5$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN6N5}\vspace*{0.5cm}
\end{figure}

% The $N_6 N_5$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN6NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_6N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN6NR}\vspace*{0.5cm}
\end{figure}

% The $N_6 N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaN5NR.ps}\vspace*{-3.0cm}
\caption{La composante $N_5N_R$ de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaN5NR}\vspace*{0.5cm}
\end{figure}

% The $N_5 N_R$component of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

% As mentioned before, we shall continue with the setting $N_2=N$, 
% $N_6=N$, $N_5= W$and $N_R= W$. In order to offer three dimensional 
% graphical depictions of the fluctuations properties of $\alpha^{\prime}$
% corrected $D_2D_6 NS_5$nonextremal black holes, we chose the higher
% derivative correction parameter $b_1= 0.001644670833$. In the regime 
% of $N \in (-10, 0)$and $W \in (0, 10)$, we find that the amplitudes 
% of the heat capacities $\{g_{N_2 N_2}, g_{N_6 N_6}\}$ take the value 
% in the range $(0, 10^{+32}$. In this range of $N, W$, the heat capacity 
% $\{ g_{N_5 N_5}\}$lies in the range $(0, 1.2 \times 10^{+17})$. 
% However, the heat capacity $\{ g_{N_R N_R}\}$changes it nature 
% and lies in the range $(-3.5 \times 10{+15}, 0)$. The negative sign 
% of $\{ g_{N_R N_R}\}$shows a local instability of the black hole 
% statistical system. From the above $\alpha^{\prime}$corrected 
% state-space geometry prediction, we observe that the range of the 
% growth of all the heat capacities $\{g_{N_2 N_2}, g_{N_6 N_6}, g_{N_5 N_5},
% g_{N_R N_R}\}$appears in the small limit of the parameters $\{N, W\}$.
% However, the first two of the components have peaks of the order 
% $10^{+32}$, $g_{N_5 N_5}$ has the peak of order $10^{+17}$and the
% component $\{ g_{N_R N_R}\}$the peak of the order $10{+15}$.
% In fact, under the $\alpha^{\prime}$corrections, we find that 
% the graphical nature of heat capacities is altered. Specifically, 
% , we observe that the heat capacities have a large peak for the 
% small values of $\{N, W\}$. In this case, the Figs.(\ref{d2d6ns5alphaN2N2}, 
% \ref{d2d6ns5alphaN6N6}), show that that the growth of the heat capacities 
% $\{ g_{N_2N_2}, g_{N_6 N_6}\}$takes place in the small limit of $W$and
% $|N|$. Similarly, the Figs.(\ref{d2d6ns5alphaN5N5}, \ref{d2d6ns5alphaNRNR}) 
% show that the growth of the $\{ g_{N_5N_5}, g_{N_R N_R}\}$takes place 
% in the small limit of $W$and $|N|$. It is worth mentioning that the first
% three of the heat capacities find a set of positive numerical values, while
% the fourth does not. On the other hand, the Figs.(\ref{d2d6ns5alphaN2N6},
% \ref{d2d6ns5alphaN2N5}, \ref{d2d6ns5alphaN2NR}, \ref{d2d6ns5alphaN6N5},
% \ref{d2d6ns5alphaN6NR}, \ref{d2d6ns5alphaN5NR}) depict the mix heat 
% compressibilities involving two distinct parameters of leading order 
% $\alpha^{\prime}$corrected nonextremal $D_2 D_6 NS_5$black holes. 
% Hereby, we notice that the amplitude of 
% (i) $g_{N_2 N_6}$ is of the order $10{+31}$, 
% (ii) $g_{N_2 N_5}$ is of the order $10{+24}$, 
% (iii) $g_{N_2 N_R}$ is of the order $-10{+23}$, 
% (iv) $g_{N_6 N_5}$ is of the order $10{+24}$, 
% (v) $g_{N_6N_R}$ is of the order $-10{+23}$, 
% and (vi) $g_{N_5 N_R}$ is of the$-10{+16}$. 
% As shown in the above graphical depictions, the state-space
% metric tensor $\{g_{ij}\ |\ i, j= n, w, N, W\}$ illustrate that
% the $\alpha^{\prime}$corrected nonextremal $D_1 D_5$black holes
% correspond a locally stable statistical configuration.

Comme mentionn\'e pr\'ec\'edemment, nous allons continuer avec la mise de 
$N_2= N$, $N_6= N$, $N_5= W$ et $N_R= W$. Afin d'offrir les repr\'esentations 
graphiques de trois dimensions des fluctuations de la configuration des trous noirs 
$D_2D_6 NS_5$ nonextremaux corrig\'es par le dominant terme de $\alpha^{\prime}$, 
nous pouvons choisir la valeur du param\`etre des corrections d\'eriv\'ees sup\'erieures 
de la th\'eorie des cordes comme $b_1= 0.001644670833$. Dans le r\'egime de 
$N \in (-10, 0)$ et $W \in (0, 10)$, nous constatons que l'amplitude des capacit\'es de chaleurs 
$\{g_{N_2 N_2}, g_{N_6 N_6}\}$ prend une valeur dans l'intervalle $(0, 10^{+32}$. 
Dans cette gamme de $N, W$, la capacit\'e thermique $\{g_{N_5 N_5}\}$ est compris\'ee 
entre $(0, 1.2 \times 10^{+17})$. Cependant, la capacit\'e thermique $\{g_{N_R N_R}\}$ 
change sa nature et elle se situe dans la gamme de $(-3,5 \times 10^{15}, 0) $. 
Le signe n\'egatif de $\{g_{N_R N_R}\}$ montre une instabilit\'e locale du syst\`eme 
statistique de ces trous noirs. De ce qui pr\'ec\`ede de la pr\'evision des corrections 
de $\alpha^{\prime}$ \`a la g\'eom\'etrie de l'espace des \'etat, nous observons que 
la range de toutes les capacit\'es de chaleurs $\{g_{N_2 N_2}, g_{N_6 N_6}, g_{N_5 N_5},
g_{N_R N_R}\}$ appara\^{i}t dans la limite d'une petite valeur des param\`etres $\{N, W\}$.
Notez bien que les deux premi\`eres composantes ont des pics \`a l'ordre de $10^{+32} $, la
composante $g_{N_5 N_5} $ a le pic \`a l'ordre de $10^{+17}$ et la composante $\{g_{N_R N_R}\}$ 
a le pic \`a l'ordre $10^{+15}$. En fait, sous les corrections de $\alpha^{\prime}$, 
nous constatons que la nature graphique des capacit\'es de chaleurs est alt\'er\'e. 
Plus pr\'ecis\'ement, nous observons que les capacit\'es de chaleurs ont un grand pic 
pour certaines petites valeurs de $\{N, W\}$. Dans ce cas, les Figs. (\ref{d2d6ns5alphaN2N2},
\ref{d2d6ns5alphaN6N6}) montrent que la croissance des capacit\'es de chaleurs $\{g_{N_2N_2}, 
g_{N_6 N_6}\}$ a lieu dans la limite d'un petit $W$ et un petit $|N|$. De plus, les Figs. 
(\ref{d2d6ns5alphaN5N5}, \ref{d2d6ns5alphaNRNR}) montrent que la croissance de 
$\{g_{N_5N_5}, g_{N_R N_R}\}$ a lieu dans la limite des petits $W$ et $|N|$. 
Il est \`a noter que le premier trois des capacit\'es de chaleurs trouvent un ensemble 
des valeurs num\'eriques positives, tandis que la quatri\`eme n'a pas. D'autre part, 
les Figs. (\ref{d2d6ns5alphaN2N6}, \ref{d2d6ns5alphaN2N5}, \ref{d2d6ns5alphaN2NR}, 
\ref{d2d6ns5alphaN6N5}, \ref{d2d6ns5alphaN6NR}, \ref{d2d6ns5alphaN5NR}) d\'epeignent 
les compressibilit\'es de chaleurs m\'elang\'es, en impliquant deux param\`etres distincts 
des trous noirs $D_2D_6NS_5$ nonextremaux sous les corrections de $\alpha^{\prime}$.
Par la pr\'esente, nous remarquons que l'amplitude des 
(i) $g_{N_2 N_6}$ est \`a l'ordre de $10{+31}$, 
(ii) $g_{N_2 N_5}$ est \`a l'ordre de $10{+24}$, 
(iii) $g_{N_2 N_R}$ est \`a l'ordre de $-10{+23}$, 
(iv) $g_{N_6 N_5}$ est \`a l'ordre de $10{+24}$, 
(v) $g_{N_6N_R}$ est \`a l'ordre de $-10{+23}$, 
et (vi) $g_{N_5 N_R}$ est \`a l'ordre de $-10{+16}$. 
Comme montr\'e ci-dessus par la repr\'esentation graphique, 
les composantes de la m\'etrique tenseure de l'espace des \'etats 
$\{g_{ij} \ | \ i, j = N_2, N_6, N_5, N_R\}$ illustrent le fait que
les trous noirs $D_2D_6NS_5$ nonextremaux corrig\'ees par les
$\alpha^{\prime}$ correspondent \`a une configuration statistique
localement stable.


\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphadetg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphadetg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the function of 
% $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaminor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaminor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaminor2.ps}\vspace*{-3.0cm}
\caption{Le mineur de surface de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaminor2}\vspace*{0.5cm}
\end{figure}

% The surface minor of the metric tensor plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_2 D_6 NS_5$charged black holes 
% at the order of $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee 
comme la fonction de $N, W$, en d\'ecrivant les fluctuations dans 
la configuration des trous noirs charg\'es nonextremaux $D_2 D_6 NS_5$
\`a l'ordre de $\alpha^{\prime}$.} \label{d2d6ns5alphaminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $N, W$, describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$.

% In this case, under the fluctuations of $\{N_2, N_6, N_5, N_R\}$, 
% the ensemble stability of the nonextremal $D_2 D_6 NS_5$black holes 
% can be described from the positivity of the determinant of the metric
% tensor $g$. For the $\alpha^{\prime}$corrected nonextremal $D_2
% D_6 NS_5$black holes with $N_2=N$, $N_6=N$, $N_5= W$ and $N_R= W$, 
% we find that the determinant of the metric tensor $g$ ceases to a 
% large negative value, as we decrease the parameters $\{|N|, W\}$. 
% This shows that the leading order higher derivative string theory 
% corrections do not yield statistical stability. In fact, we observe 
% that $g \in (-4 \times 10^{11}, 0)$. For a typical value of $N \in (-10, 1)$
% and $W \in (0, 10)$, the Fig.(\ref{d2d6ns5alphadetg}) describes the 
% graphical view of the determinant of the metric tensor $g$. Interestingly, 
% the stability of the hypersurface defined by a constant value of $N_R$
% is shown in the Fig.(\ref{d2d6ns5alphaminor3}). Namely, we see that the 
% hypersurface minor $p_3$lies in the range of $(0, 8 \times 10^{9})$. 
% For a given small value of $|N|, W$, we notice that the peak of $p_3$
% increases as we approach to the origin. On the other hand, the surface 
% defined by the fluctuations of $\{N_2, N_6\}$acquires positive signature
% under the $\alpha^{\prime}$corrections. This positivity of the principle 
% minors $\{ p_2, p_3\}$shows internal stability of the black hole system. 
% For $N \in (-10, 1)$and $W \in (0, 10)$, the graphical view of the minor 
% $p_2$is shown in the Fig.(\ref{d2d6ns5alphaminor2}). In this case, we see
% that $p_2$lies in the range of $(0, 2 \times 10^{+07}))$. Also, we notice
% that the minor $p_2$has a large positive peak at the origin. Finally, 
% when only the parameter $N_2$is allowed to vary, the stability of the 
% black hole system is given by the positivity of the first principle minor 
% $p_1:= g_{N_2 N_2}$. With a different orientation, the graphical view of 
% $p_1$ is shown in the Fig.(\ref{d2d6ns5alphaminor1}). The above qualitative 
% behaviour of the state-space metric tensor and the positivity of the 
% principle minors describe statistical fluctuation properties of the
% $\alpha^{\prime}$corrected nonextremal $D_2 D_6 NS_5$ black holes.

Dans ce cas, sous les fluctuations de $\{N_2, N_6, N_5, N_R\}$,
la stabilit\'e d'un ensemble des trous noirs $D_2 D_6 NS_5 $ nonextremaux 
peut \^{e}tre d\'ecrite de la positivit\'e du d\'eterminant de la m\'etrique
tenseure $g$. Pour les trous noirs $D_2D_6 NS_5$ nonextremaux corrig\'ees par 
les termes de $\alpha^{\prime}$ avec $N_2= N$, $N_6= N$, $N_5= W$ et $N_R=W$,
nous constatons que le d\'eterminant de la m\'etrique tenseure $g$ prend une 
grande valeur n\'egative, quant \`a nous diminuons les param\`etres $\{|N|, W\}$.
Cela montre que les corrections d\'eriv\'ees sup\'erieures de la th\'eorie des cordes
\`a l'ordre dominant ne donnent pas de stabilit\'e statistique. En fait, nous observons
que $g \in (-4 \times 10^{+11}, 0)$. Pour une valeur typique de $N \in (-10, 1)$ et 
$W \in (0, 10)$, la Fig. (\ref{d2d6ns5alphadetg}) d\'ecrit la vue graphique du 
d\'eterminant de la m\'etrique tenseure $g$. Fait int\'eressant, la stabilit\'e 
de l'hypersurface d\'efinie par une valeur constante de $N_R$ est montr\'e dans 
la Fig. (\ref{d2d6ns5alphaminor3}). Notamment, nous voyons que le mineur de l'hypersurface 
$p_3$ r\'eside dans la gamme de $(0, 8 \times 10^{+09})$. Pour une petite valeur donn\'ee des 
param\`etres $|N|, W$, on constate que le pic de $p_3$ augmente \`a mesure que nous 
approchons \`a l'origine. D'autre part, la surface d\'efinies par les fluctuations de 
$\{N_2, N_6\}$ acquiert la signature positive sous les corrections de $\alpha^{\prime}$. 
Cette positivit\'e des mineurs principaux $\{p_2, p_3\}$ montre la stabilit\'e interne 
du syst\`eme de ces trous noirs. Pour $N \in (-10, 1)$ et $W \in (0, 10)$, la vue graphique 
du mineur $p_2$ est montr\'e dans la Fig. (\ref{d2d6ns5alphaminor2}). Dans ce cas, nous voyons
que $p_2$ r\'eside dans la gamme de $(0, 2 \times 10^{+07})$. En outre, nous remarquons par la 
Fig. (\ref{d2d6ns5alphaminor2}) que le mineur $p_2$ a un grand pic positif pr\`es de l'origine. 
Enfin, lorsque le seul param\`etre $N_2$ est autoris\'e \`a varier, la stabilit\'e du syst\`eme 
de ces trous noirs est donn\'ee par la positivit\'e de premier mineur principe $p_1:= g_{N_2 N_2}$.
Avec une orientation diff\'erente, la vue graphique de premier mineur principe $p_1$ est montr\'e 
dans la Fig. (\ref{d2d6ns5alphaminor1}). Le comportement qualitatif ci-dessus de la m\'etrique 
tenseure de l'espace des \'etats et la positivit\'e des mineurs principaux d\'ecrirent les 
propri\'et\'es statistiques des fluctuations de trous noirs $D_2 D_6 NS_5$ nonextremaux 
corrig\'es de $\alpha^{\prime}$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaR.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
charg\'es nonextremaux $D_2 D_6 NS_5$ \`a l'ordre de $\alpha^{\prime}$ 
dans la gamme $n \in (-10,0)$ et $N \in (0,10)$.} \label{d2d6ns5alphaR}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$in the range 
% $n \in (-10,0)$and $N \in (0,10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{d2d6ns5alphaR10.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $N, W$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs
charg\'es nonextremaux $D_2 D_6 NS_5$ \`a l'ordre de $\alpha^{\prime}$ 
dans la gamme $n, N \in (-10, 10)$.} \label{d2d6ns5alphaR10}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing the fluctuations in the nonextremal $D_2 D_6 NS_5$
% charged black holes at the order of $\alpha^{\prime}$ in the range 
% $n, N \in (-10, 10)$.

% As mentioned in the previous section, the state-space description
% continues to the higher derivative corrected $D_2 D_6 NS_5$black holes.
% In particular, the scalar curvature offers the global properties of 
% underlying statistical fluctuations. In the range $N \in (-10, 0)$
% and $W \in (0, 10)$, we observe from the Fig.(\ref{d2d6ns5alphaR}) 
% that the the scalar curvature has a positive peak of the order
% unity. In this range of the parameters $\{N_2, N_6, N_5, N_R\}$, 
% the $\alpha^{\prime}$corrected nonextremal $D_1 D_6 NS_5$black 
% holes correspond to an interacting statistical configuration. 
% As mentioned before, the positive sign of the state-space scalar 
% curvature signifies that the statistical interactions are repulsive 
% in their nature. Furthermore, the Fig.(\ref{d2d6ns5alphaR10}) 
% illustrates the behaviour of the state-space scalar curvature for 
% the range of the parameters $N, W \in (-10, 10)$. Precisely, we see 
% that there are found band of interactions. The interaction increases
% as we approach to the origin. We find that the corresponding scalar 
% curvature has a small peak of order $0.35$ at the origin $(N,W)= (0,
% 0)$. In the range of $N,W \in (-10, 10)$, we observe from the
% Fig.(\ref{d2d6ns5alphaR10}) that the global statistical interactions 
% are symmetric in each quadrant of the $NW$-plane. In contrast to the 
% peak of the scalar curvature appearing in the range $N, W \in (0,10)$,
% the peak of the scalar curvature turn out to be smaller in the range 
% $N, W \in (-10, 10)$. From the Figs.(\ref{d2d6ns5alphaR}, \ref{d2d6ns5alphaR10}), 
% we observe that the state-space scalar curvatures remains positive
% in both the above intervals. Qualitatively, the state-space depictions 
% indicate that the $\alpha^{\prime}$corrected nonextremal $D_2 D_6 NS_5$
% black holes are globally unstable weakly interacting statistical configurations. 
% In short, the leading order higher derivative $\alpha^{\prime}$ correction 
% improve the stability of fluctuating nonextremal $D_1 D_5$ configurations 
% by offering (i) positive principle minors and (ii) small peak to the 
% state-space scalar curvature.

Comme mentionn\'e dans la section pr\'ec\'edente, la description de l'espace
des \'etats continue \`a la configuration des trous noirs $D_2 D_6 NS_5$ nonextremaux 
corrig\'es par les d\'eriv\'es sup\'erieures de $\alpha^{\prime}$. 
En particulier, la courbure scalaire sous-jacente de l'espace des \'etats offre les 
propri\'et\'es globales des fluctuations statistiques. Dans la gamme de $N \in (-10, 0)$
et $W \in (0, 10)$, on observe de la Fig. (\ref{d2d6ns5alphaR}) que la courbure scalaire 
a un pic positif \`a l'ordre d'unit\'e. Dans cette gamme de param\`etres $\{N_2, N_6, N_5, N_R\}$,
les trous noirs $D_1 D_6 NS_5$ nonextremaux corrig\'ees par les termes de $\alpha^{\prime}$
correspondent \`a une configuration statistique avec certaines interactions non-nulles.
Comme mentionn\'e pr\'ec\'edemment, le signe positif de la courbure scalaire de l'espace 
des \'etats signifie que les interactions statistiques sont r\'epulsives dans la leur nature. 
En outre, la Fig. (\ref{d2d6ns5alphaR10}) illustre le comportement de la courbure scalaire 
de l'espace des \'etats dans la gamme des param\`etres $N, W \in (-10, 10)$. Justement, 
nous voyons qu'il y a d\'ecouvert de la bande des interactions. L'interaction augmente alors 
que nous approchons de l'origine. Nous constatons que la courbure scalaire correspondante
a un petit pic \`a l'ordre de $0.35$ pr\`es de l'origine $(N, W)= (0,0)$. Dans la gamme de 
$N, W \in (-10, 10) $, on observe de la Fig. (\ref{d2d6ns5alphaR10}) que les interactions 
statistiques globales sont sym\'etriques, dans chaqu'un de quadrant de plan $NW$. 
En contraire du sommet de la courbure scalaire apparaissant dans la gamme de 
$N, W \in (0, 10)$, le pic de la courbure scalaire s'av\'ere plus petit dans la gamme
$N, W \in (-10, 10) $. Par les Figs. (\ref{d2d6ns5alphaR}, \ref{d2d6ns5alphaR10}),
nous observons que la courbure scalaire de l'espace des \'etats reste positif dans 
les deux intervalles ci-dessus. Qualitativement, les repr\'esentations de l'espace
des \'etats indiquent que les trous noirs $D_2 D_6 NS_5 $ nonextremaux corrig\'es
par les termes de $\alpha^{\prime}$ sont globalement instables et correspondent 
\`a une configuration statistique faiblement interactive. En bref, les corrections 
des d\'eriv\'ees sup\'erieures de $\alpha^{\prime}$ \`a l'ordre dominant am\'eliorent 
la stabilit\'e des fluctuations dans la configuration des trous noirs $D_2D_6NS_5$
nonextremaux en offrant (i) des valeurs positives aux mineurs principaux et (ii) un petit 
pic \`a la courbure scalaire sous-jacente de l'espace des \'etats.


\section{Les trous noirs en rotation}
% Rotating Black Holes


\subsection{Les trous noirs de Kerr Newman}

% Kerr-Neumann black holes

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KNqq.ps}\vspace*{-3.0cm}
\caption{La composante $qq$ de la m\'etrique tenseure trac\'ee comme la
fonction de $q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kerr-Neumann.} \label{KNqq}\vspace*{0.5cm}
\end{figure}

% The qq component of the metric tensor plotted as the
% function of $q, J$, describing the fluctuations in the Kerr-Neumann
% rotating black configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KNJJ.ps}\vspace*{-3.0cm}
\caption{La composante $JJ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kerr-Neumann.} \label{KNJJ}\vspace*{0.5cm}
\end{figure}

% The JJ component of the metric tensor plotted as the
% function of $q, J$, describing the fluctuations in the Kerr-Neumann 
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KNqJ.ps}\vspace*{-3.0cm}
\caption{La composante $qJ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kerr-Neumann.} \label{KNqJ}\vspace*{0.5cm}
\end{figure}

% The qJ component of the metric tensor plotted as the
% function of $q, J$, describing the fluctuations in the Kerr-Neumann 
% rotating black hole configuration.


% Under the fluctuation of the parameters $\{q, J\}$, 
% the Figs.(\ref{KNqq}, \ref{KNJJ}) depict the nature of the components 
% $\{g_{qq}, g_{JJ}\}$of the thermodynamic metric tensor. In the regime 
% of $q \in (-10,2)$and $J\in (-2,10)$, we find that the amplitude of heat
% capacity $\{g_{qq}\}$takes value in the interval $(-0.003, 0)$. 
% In this range of $\{q, J\}$, we observe that the component $\{ g_{JJ}\}$
% lies in the range of $(0, -50)$. In this case, we see that the range of 
% the growth of the amplitudes of both the components $\{g_{qq}\}$and 
% $\{g_{JJ}\}$remains mostly about the line $J=0$. Explicitly, the 
% Figs.(\ref{KNqq}, \ref{KNJJ}) indicate that the growth of the $\{g_{qq}\}$
% takes place in the limit of a small $q$. The negative sign of $\{g_{qq}\}$
% signifies that the Kerr-Neumann black holes are thermodynamically unstable 
% in the limit of small electric charge. Similarly, the Fig.(\ref{KNqJ}) shows 
% that the nature of $\{ g_{qJ}\}$component of the thermodynamic metric tensor. 
% We find that the mix component $\{ g_{qJ}\}$lies in the interval $(-0.03, +0.03)$
% In this limit of $q$and $J$, the heat compressibilities as depicted in the 
% Figs.(\ref{KNqq},\ref{KNJJ}, \ref{KNqJ}) illustrate the parametric 
% fluctuation properties of the Kerr-Neumann black holes. Hereby, 
% we notice that the self pair fluctuations involving $\{q, J\}$, 
% as defined by the metric tensor $\{g_{ij}\ |\ i, j= S, Q\}$, 
% have only negative values, while the mix component $\{ g_{qJ}\}$
% has the both. At this juncture, we find that the Kerr-Neumann 
% black holes have negative heat capacities and thus a signature 
% of the local statistical instability.

Sous la fluctuation des param\`etres $\{q, J\}$, les Figs. (\ref{KNqq}, \ref{KNJJ}) 
d\'epeignent la nature des composantes $\{g_{qq}, g_{JJ}\}$ de la m\'etrique tenseure 
thermodynamique. Dans le r\'egime de $q \in (-10, 2)$ et $J \in (-2, 10) $, 
nous constatons que l'amplitude des capacit\'es de chaleurs $\{g_{qq}\}$ prend 
une valeur dans l'intervalle $(-0.003, 0)$. Dans cette gamme des param\`etres $\{q, J\}$, 
on peur observer que la composante $\{g_{JJ}\}$ r\'eside dans la gamme de $(-50, 0)$. 
Dans ce cas, nous voyons que l'amplitudes des deux composantes $\{g_{qq}\}$ et $\{g_{JJ}\}$ 
reste la plupart du temps sur la ligne $J= 0$. Explicitement, les Figs. (\ref{KNqq}, 
\ref{KNJJ}) indiquent que la croissance de la composante $\{g_{qq}\}$ prend un place dans 
la limite d'une petite charge $q$. Le signe n\'egatif de $\{g_{qq}\}$ signifie 
que les trous noirs de Kerr-Neumann sont thermodynamiquement instables dans la limite d'une 
petite charge \'electrique. Du fait m\^{e}me, la Fig. (\ref{KNqJ}) montre que la nature de la 
composante $\{g_{qJ}\}$ de la m\'etrique tenseure thermodynamique. Nous constatons que la composante 
mixe $\{g_{qJ}\}$ reste dans l'intervalle $(-0.03, +0.03)$. Dans cette limite de $\{q, J\}$, 
les compressibilit\'es de chaleurs, qui sont pr\'es\'ent\'ees dans les Figs. (\ref{KNqq}, \ref{KNJJ}, \ref{KNqJ}) 
illustrent les propri\'et\'es param\'etriques au dessus des fluctuations de la configuration 
des trous noirs de Kerr-Neumann. Par la pr\'esente, nous pouvons voir que les fluctuations d'auto-paires, 
en impliquant $\{q, J\}$ tel qu'elles sont d\'efinies par les composantes de la m\'etrique tenseure 
$\{g_{ij} \ | \ i, j= q, J\}$, n'ont que des valeurs n\'egatives, tandis que la composante mixe 
$\{g_{qJ}\}$ \`a la fois a les deux signe. \`A ce stade, nous constatons que les trous noirs 
de Kerr-Neumann ont des capacit\'es de chaleurs n\'egatives, et donc on a une signature 
des instabilit\'es statistiques locales.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KNminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kerr-Neumann.} \label{KNminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $q, J$, describing the fluctuations in the Kerr-Neumann
% rotating black hole configuration.

% The stability of the black hole ensemble can be determined in terms 
% of the parameters $q, J$. This follows from the behaviour of the
% determinant of thermodynamic metric tensor. In this case, since
% the determinant of the metric tensor vanishes identically for all
% $(q, J)$. Thus, the fluctuations of $(q, J)$introduces instability 
% in the ensemble. When only the parameter $q$is allowed to vary, 
% thestability of the Kerr-Neumann black hole is determined by the
% positivity of the first principle minor $p_1:= g_{qq}$. A rotated
% view of the $p_1$is shown in the Fig.(\ref{KNminor1}). The
% above graphical depictions of the thermodynamic geometry provide 
% the qualitative statistical properties of the two parameter 
% Kerr-Neumann black holes.

% Notice that the global stability of the Kerr-Neumann black holes 
% follows from the behaviour of the thermodynamic scalar curvature.
% In this case, for all values of the parameters $(q, J)$, we find 
% that the scalar curvature is ill-defined. This shows that the 
% Kerr-Neumann black hole configuration corresponds to ill-behaved 
% statistical basis at the two derivative level. In short, the 
% thermodynamic geometry indicate that the Kerr-Neumann black holes 
% are unstable statistical configurations under the fluctuation
% of the parameters $\{q, J\}$.

La stabilit\'e d'un ensemble des trous noirs de Kerr-Neumann peut \^{e}tre 
d\'etermin\'e en termes des param\`etres $\{q, J\}$. Cela d\'ecoule du comportement 
de la d\'eterminant de la m\'etrique tenseure thermodynamique. Dans ce cas, puisque
le d\'eterminant de la m\'etrique tenseure est identiquement nulle pour toute valeur 
des $\{q, J\}$. Ainsi, les fluctuations de $\{q, J\}$ introduissent une instabilit\'e
dans l'ensemble sous-jacent. Lorsque le seul param\`etre $q$ est autoris\'e \`a varier,
la stabilit\'e de la configuration des trous noirs de Kerr-Neumann est d\'etermin\'ee 
par la positivit\'e du premier mineur principe $p_1:= g_{qq}$. Une vue rotat\'ee de 
$p_1$ est montr\'ee dans la Fig. (\ref{KNminor1}). Les repr\'esentations graphiques 
ci-dessus de la g\'eom\'etrie thermodynamiques fournissent la propri\'et\'e qualitative
des fluctuations de la configuration statistique des trous noirs de Kerr-Neumann 
de deux param\`etres.

Notez bien que la stabilit\'e globale des trous noirs de Kerr-Neumann
d\'ecoule du comportement de la courbure scalaire thermodynamique.
Dans ce cas, pour toute valeur des param\`etres $\{q, J\}$, on trouve que 
la courbure scalaire est partout mal d\'efinie. Cela montre que la configuration 
des trous noirs de Kerr-Neumann correspond \`a mal comportement de base statistique
au niveau de la th\'eorie de gravit\'e des deux d\'eriv\'es. En bref, la 
g\'eom\'etrie thermodynamique indiquent que les trous noirs de Kerr-Neumann
correspondent \`a une configuration statistique instable en vertu de la 
fluctuation des param\`etres $\{q, J\}$.


\subsection{Les trous noirs de Kaluza-Klein}

% Kaluza-Klein black holes

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKPP.ps}\vspace*{-3.0cm}
\caption{La composante $PP$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKPP}\vspace*{0.5cm}
\end{figure}

% The $PP$component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKQQ.ps}\vspace*{-3.0cm}
\caption{La composante $QQ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKQQ}\vspace*{0.5cm}
\end{figure}

% The $QQ$component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKJJ.ps}\vspace*{-3.0cm}
\caption{La composante $JJ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKJJ}\vspace*{0.5cm}
\end{figure}

% The $JJ$component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKPQ.ps}\vspace*{-3.0cm}
\caption{La composante $PQ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKPQ}\vspace*{0.5cm}
\end{figure}

% The $PQ$component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKPJ.ps}\vspace*{-3.0cm}
\caption{La composante $PJ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKPJ}\vspace*{0.5cm}
\end{figure}

% The $PJ$component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKQJ.ps}\vspace*{-3.0cm}
\caption{La composante $QJ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKQJ}\vspace*{0.5cm}
\end{figure}

% The $QJ$component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

% In this case, since there are three independent variables $\{P, Q, J\}$, 
% thus we are required to fix one of the variable in order to offer the 
% three dimensional graphical views of the fluctuation. We do so by choosing
% $P= Q$. For a given Kaluza-Klein extremal black holes, the fluctuations 
% properties are expressed in the following . In the regime of $Q
% \in (-10, 10)$and $J \in (-10,10)$, we observe that the amplitudes of
% the heat capacities $\{g_{QQ}, g_{PP}\}$ take a value of the order $120$. 
% In this range of $Q, J$, the heat capacities $\{ g_{JJ}\}$lies in the 
% range $(0, 30)$. As per the prediction of the state-space geometry, 
% we find that the range of the growth of the first and the second sets 
% of the heat capacities shifts away from the origin, as we increase 
% the values of the parameters $\{Q, J\}$. Specifically, for $Q \simeq 5 $, 
% the peak of the heat capacities $\{g_{QQ}, g_{PP}\}$ increase randomly,
% as we increase the value of $J$. However, for $Q \simeq 5$, the peak of
% the component $g_{JJ}$ decreases, as we increase the value of $J$. 
% In this concern, the Figs.(\ref{KKPP}, \ref{KKQQ}), show that that the
% growth of the heat capacities $\{ g_{PP}, g_{QQ}\}$ takes place in 
% a set of random amplitude $QJ$ surfaces. Similarly, the Fig.(\ref{KKJJ}) 
% shows that the growth of the component $\{ g_{JJ}\}$ takes place in 
% a set of increasing amplitude $QJ$surfaces. Similarly, the heat 
% compressibilities involving two distinct parameters of Kaluza-Klein
% black hole are depicted in the Figs.(\ref{KKPQ}, \ref{KKPJ},\ref{KKQJ}). 
% Herewith, we find that the amplitude of (i) $g_{PQ}$ lies in the interval 
% $(0, 100)$, (ii) $g_{PJ}$ lies in the range $(-50, 50)$ and (iii) 
% $g_{QJ}$ also lies in the interval $(-50, 50)$. Hereby, the components
% of the state-space metric tensor $\{g_{ij}\ |\ i, j= P, Q, J\}$, 
% as depicted in the Figs.(\ref{KKPP}, \ref{KKQQ}, \ref{KKJJ}) show 
% that the Kaluza-Klein black holes correspond to a locally stable 
% statistical system with a set of positive heat capacities.

Dans ce cas, puisqu'il y a trois variables ind\'ependantes $\{P, Q, J\}$,
donc nous sommes tenus \`a fixer l'une des variables afin d'offrir la vue graphique
de trois dimensions des fluctuations sous-jacentes. Nous le faisons en choisissant $P= Q$. 
Pour une configuration donn\'ee des trous noirs extr\'emalaux de Kaluza-Klein, 
les propri\'et\'es des fluctuations sont exprim\'ees comme les suivantes. 
Dans le r\'egime de $Q \in (-10, 10)$ et $J \in (-10,10)$, on observe que l'amplitude 
des capacit\'es de chaleurs $\{g_{QQ}, g_{PP}\}$ prend une valeur \`a l'ordre de $120$.
Dans cette gamme de $\{Q, J\}$, la capacit\'e de la chaleur $\{g_{JJ}\}$ r\'eside dans la
gamme de $(0, 30)$. En conformant \`a la pr\'ediction de la g\'eom\'etrie de l'espace des \'etats,
nous constatons que les gammes de la premi\`ere ensemble et la deuxi\`eme ensemble des capacit\'es 
de chaleurs s'\'eloignent de l'origine, quand nous augmentons les valeurs de param\`etres $\{Q, J\}$. 
Plus pr\'ecis\'ement, pour $Q \simeq 5$, le pic des capacit\'es de chaleurs $\{g_{QQ}, g_{PP}\}$ 
augmente au hasard, \`a mesure que nous augmentons la valeur de $J$. De plus, pour $Q \simeq 5$, 
le pic de l'\'el\'ement $g_{JJ}$ diminue, quand nous augmentons la valeur de $J$. Dans ce cas, 
les Figs. (\ref{KKPP}, \ref{KKQQ}) montrent que la croissance des capacit\'es de chaleurs 
$\{g_{PP}, g_{QQ}\}$ a lieu dans un ensemble des amplitudes al\'eatoires sur la surface $QJ$. 
En outre, la Fig. (\ref{KKJJ}) montre que la croissance de la composante $\{g_{JJ}\}$ a lieu 
dans un ensemble des croissantes amplitudes sur la surface $QJ$. De m\^{e}me, les compressibilit\'es
de chaleurs en impliquant deux param\`etres distincts de la configuration des trous noirs de 
Kaluza-Klein sont repr\'esent\'es dans les Figs. (\ref{KKPQ}, \ref{KKPJ}, \ref{KKQJ}).
Par la pr\'esente, nous constatons que l'amplitude de (i) $g_{PQ}$ reste dans l'intervalle
$(0, 100)$, (ii) $g_{PJ}$ se situe dans la gamme de $(-50, 50)$ et (iii) $g_{QJ}$ r\'eside 
aussi dans l'intervalle $(-50, 50)$. De toute fa\c{c}on, les composantes de la m\'etrique 
tenseure de l'espace des \'etats $\{g_{ij} \ | \ i, j = P, Q, J\}$, comme illustr\'e dans les
Figs. (\ref{KKPP}, \ref{KKQQ}, \ref{KKJJ}) montrent que la configuration des trous noirs de 
Kaluza-Klein correspond \`a un syst\`eme statistique localement stable avec un ensemble des 
capacit\'es thermiques positives par rapport \`a la g\'eom\'etrie de l'espace des \'etats.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKdetg.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKdetg}\vspace*{0.5cm}
\end{figure}

% The determinant of the metric tensor plotted as the 
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKminor2.ps}\vspace*{-3.0cm}
\caption{Le mineur de surface de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKminor2}\vspace*{0.5cm}
\end{figure}

% The surface minor of the metric tensor plotted as the 
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de Kaluza-Klein.} \label{KKminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the 
% function of $Q, J$, describing fluctuations in the Kaluza-Klein
% rotating black hole configuration.

% Under the fluctuations of the parameters $\{P, Q, J\}$, the ensemble 
% stability of the Kaluza-Klein black holes follows from the positivity 
% of the determinant of the metric tensor. For the choice of $P= Q$, 
% we find that the determinant of the metric tensor $g$ceases to a large 
% negative value, as we allow to fluctuate the parameters $\{P, Q, J\}$. 
% In this case, we see that $g \in (-7000, 0)$. For a typical value of 
% $Q \in (-10, 10)$and $J \in (-10,10)$, the Fig.(\ref{KKdetg}) offers 
% the graphical nature of the determinant of the metric tensor $g$. 
% Furthermore, the fluctuations of $\{P, Q\}$corresponds to a stable surface. 
% From the Fig.(\ref{KKminor2}), this follows because the corresponding principle 
% minor $p_2 \in (0, 5000)$. Finally, when only the parameter $P$is allowed to vary, 
% the stability of the Kaluza-Klein black hole is determined by the positivity of 
% the first principle minor $p_1:= g_{PP}$. A rotated view of $p_1$is shown in 
% the Fig.(\ref{KKminor1}). The above qualitative properties of the principle 
% minors describes state-space behaviour of the statistical fluctuations of 
% the Kaluza-Klein black holes.

Sous les fluctuations des param\`etres $\{P, Q, J\}$, la stabilit\'e 
d'un ensemble des trous noirs de Kaluza-Klein d\'ecoule de la positivit\'e
du d\'eterminant de la m\'etrique tenseure. Pour le choix du $P= Q$, 
nous constatons que le d\'eterminant de la m\'etrique tenseure $g$ prend une grande
valeur n\'egative, quand nous permetons \`a fluctuer les param\`etres $\{P, Q, J\}$.
Dans ce cas, nous voyons que $g \in (-7000, 0)$. Pour une valeur typique de
$Q \in (-10, 10)$ et $J \in (-10, 10)$, la Fig. (\ref{KKdetg}) offre la nature graphique 
de d\'eterminant de la m\'etrique tenseure $g$. Par la suite, les fluctuations de 
$\{P, Q\}$ correspond \`a une surface stable. De la Fig. (\ref{KKminor2}), 
ce qui suit par-ce que le mineur principe correspondant $p_2 \in (0, 5000)$. Enfin, 
lorsque le seul param\`etre $P$ est autoris\'e \`a varier, la stabilit\'e de la
configuration des trous noirs de Kaluza-Klein est d\'etermin\'ee par la positivit\'e 
du premier mineur principe $p_1:= g_{PP}$. Une vue rotat\'ee de $p_1$ est montr\'e 
dans la Fig. (\ref{KKminor1}). Les propri\'et\'es qualitative ci-dessus des mineurs
principaux d\'ecritent le comportement des fluctuations statistiques de l'espace des 
\'etats des trous noirs de Kaluza-Klein.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKR.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction 
de $Q, J$, en d\'ecrivant les fluctuations dans la 
configuration des trous noirs de Kaluza-Klein dans la 
gamme de $Q, J \in (-10, 10)$.} \label{KKR}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing fluctuations in the Kaluza-Klein rotating black hole 
% configuration in the range of $Q, J \in (-10, 10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{KKRhalf.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction 
de $Q, J$, en d\'ecrivant les fluctuations dans la configuration 
des trous noirs de Kaluza-Klein dans la gamme de $Q \in (-10, 0)$
et $J \in (0, 10)$.} \label{KKRhalf}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $N, W$, 
% describing fluctuations in the Kaluza-Klein rotating black 
% hole configuration in the range of $Q \in (-10, 0)$and 
% $J \in (0, 10)$.


% As mentioned in the previous section, the state-space scalar
% curvature describes the global statistical ensemble properties of
% the fluctuating black holes. Under the fluctuation of $\{P, Q, J\}$,
% the global stability structure of the Kaluza-Klein black holes 
% can be described as follows. In the range of $Q, J \in (-10, 10)$, 
% the Fig.(\ref{KKR}) shows that the scalar curvature has a small 
% negative amplitude of the order $-0.30$. In this range of the parameters, 
% we observe that the Kaluza-Klein configuration is a weakly interacting 
% statistical system. Physically, the negative sign of the scalar curvature 
% signifies that the statistical interactions are attractive in their nature. 
% The Fig.(\ref{KKRhalf}) illustrates the behaviour of the above scalar 
% curvature for range of the parameters $Q \in (-10, 0)$and $J \in (0, 10)$. 
% In fact, we see that the interactions are largely present near the origin.
% The Fig.(\ref{KKRhalf}) shows that the state-space scalar curvature acquires 
% a large peak of order $-3 \times 10^{+15}$at the origin $(Q, J)= (0, 0)$. 
% Moreover, we notice from the Fig.(\ref{KKRhalf}) that the global statistical 
% interactions fill the full line $J=0$in the limit of $Q=0$. In comparison 
% with the interactions appearing in the range of $Q, J \in (-10,10)$, 
% the amplitude of the global statistical interactions turn out to be much larger 
% in the range $Q \in (-10, 0)$and $J \in (0, 10)$. Precisely, we find that 
% the ratio of typical values of the amplitude of the scalar curvatures is 
% of the order $10^{+16}$. The graphical view of the above mentioned comparison 
% follows from the Figs.(\ref{KKR}, \ref{KKRhalf}). Qualitatively, from the above
% mentioned state-space depictions, we observe that the Kaluza-Klein black holes 
% are globally unstable interacting statistical configurations when they are 
% considered in the two derivative gravity theory.

Comme mentionn\'e dans la section pr\'ec\'edente, la courbure scalaire de
l'espace des \'etats d\'ecrit les propri\'et\'es globales d'un ensemble statistique
de ces trous noirs en fluctuant $\{P, Q, J\}$. Sous la fluctuation de $\{P, Q, J\}$,
la structure de la stabilit\'e globale des trous noirs de Kaluza-Klein
peut \^{e}tre d\'ecrit comme la suit. Dans la gamme de $Q, J \in (-10, 10)$,
la Fig. (\ref{KKR}) montre que la courbure scalaire prend une petite amplitude 
n\'egative \`a l'ordre de $-0.30$. Dans cette gamme de param\`etres, 
nous observons que la configuration de Kaluza-Klein est un syst\`eme statistique
faiblement interactif. Physiquement, le signe n\'egatif de la courbure scalaire
signifie que les interactions statistiques sont attrayantes dans la leur nature.
La Fig. (\ref{KKRhalf}) illustre le comportement de la courbure scalaire ci-dessus
pour la gamme des param\`etres $Q \in (-10, 0)$ et $J \in (0, 10)$. En fait, 
nous voyons que les interactions sont largement pr\'esentes pr\`es de l'origine.
La Fig. (\ref{KKRhalf}) montre que la courbure scalaire de l'espace des \'etats 
acquiert un grand pic \`a l'ordre de $-3 \times 10^{+15}$ pr\`es de l'origine 
$(Q, J)= (0, 0)$. Par ailleurs, nous remarquons de la Fig. (\ref{KKRhalf}) que 
les interactions statistiques globales remplissent la gamme compl\`ete $J= 0$,
dans la limite de $Q= 0$. En comparaison des interactions apparaissent dans la gamme 
de $Q, J \in (-10,10)$, l'amplitude des interactions statistiques globales 
se r\'ev\`ele d'\^{e}tre beaucoup plus grande dans la gamme de $Q \in (-10, 0)$
et $J \in (0, 10)$. Pr\'ecis\'ement, nous constatons que le ratio des valeurs typiques 
de l'amplitude des courbures scalaire est \`a l'ordre de $10^{16}$. La vue graphique 
de cette comparaison ci-dessus d\'ecoule par les Figs. (\ref{KKR}, \ref{KKRhalf}). 
Qualitativement, de ce qui pr\'ec\`ede est mentionn\'es vers la repr\'esentation de
l'espace des \'etats, nous observons que la configuration des trous noirs de Kaluza-Klein 
est globalement instable et correspond \`a un syst\`eme statistique int\'eractif, quand elle
est pris en compte dans la th\'eorie de la gravit\'e des deux d\'eriv\'es.


\subsection{Les trous noirs h\'et\'erotiques}

% Heterotic black holes

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP1P1.ps}\vspace*{-3.0cm}
\caption{La composante $P_1P_1$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP1P1}\vspace*{0.5cm}
\end{figure}

% The $P_1P_1$component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetQ2Q2.ps}\vspace*{-3.0cm}
\caption{La composante $Q_2Q_2$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetQ2Q2}\vspace*{0.5cm}
\end{figure}

% The $Q_2Q_2$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration. 

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP3P3.ps}\vspace*{-3.0cm}
\caption{La composante $P_3P_3$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP3P3}\vspace*{0.5cm}
\end{figure}

% The $P_3P_3$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetQ4Q4.ps}\vspace*{-3.0cm}
\caption{La composante $Q_4Q_4$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetQ4Q4}\vspace*{0.5cm}
\end{figure}

% The $Q_4Q_4$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetJJ.ps}\vspace*{-3.0cm}
\caption{La composante $JJ$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetJJ}\vspace*{0.5cm}
\end{figure}

% The $JJ$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP1Q2.ps}\vspace*{-3.0cm}
\caption{La composante $P_1Q_2$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP1Q2}\vspace*{0.5cm}
\end{figure}

% The $P_1Q_2$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP1P3.ps}\vspace*{-3.0cm}
\caption{La composante $P_1P_3$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP1P3}\vspace*{0.5cm}
\end{figure}

% The $P_1P_3$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP1Q4.ps}\vspace*{-3.0cm}
\caption{La composante $P_1Q_4$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP1Q4}\vspace*{0.5cm}
\end{figure}

% The $P_1Q_4$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP1J.ps}\vspace*{-3.0cm}
\caption{La composante $P_1J$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP1J}\vspace*{0.5cm}
\end{figure}

% The $P_1J$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetQ2P3.ps}\vspace*{-3.0cm}
\caption{La composante $Q_2P_3$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetQ2P3}\vspace*{0.5cm}
\end{figure}

% The $Q_2P_3$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetQ2Q4.ps}\vspace*{-3.0cm}
\caption{La composante $Q_2Q_4$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetQ2Q4}\vspace*{0.5cm}
\end{figure}

% The $Q_2Q_4$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetQ2J.ps}\vspace*{-3.0cm}
\caption{La composante $Q_2J$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetQ2J}\vspace*{0.5cm}
\end{figure}

% The $Q_2J$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP3Q4.ps}\vspace*{-3.0cm}
\caption{La composante $P_3Q_4$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP3Q4}\vspace*{0.5cm}
\end{figure}

% The $P_3Q_4$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetP3J.ps}\vspace*{-3.0cm}
\caption{La composante $P_3J$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetP3J}\vspace*{0.5cm}
\end{figure}

% The $P_3J$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetQ4J.ps}\vspace*{-3.0cm}
\caption{La composante $Q_4J$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetQ4J}\vspace*{0.5cm}
\end{figure}

% The $Q_4J$ component of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black hole configuration.



% In this case, notice that there are five independent variables 
% $\{ P_1, Q_2, P_3, Q_4, J\}$of fluctuations. Thus, in order to 
% offer three dimensional view of the statistical fluctuations, 
% we need to fix three of variables. We do so by considering 
% $P_1= Q$, $Q_2= Q$, $P_3= Q$and $Q_4= Q$. For a given heterotic
% black holes, the fluctuations properties can be described by the 
% following set of three dimensional . Namely, in the regime 
% of $Q, J \in (-10, 10)$, we see that the amplitude of the heat 
% capacities $\{g_{P_1 P_1}, g_{Q_2 Q_2}, g_{P_3 P_3}, g_{Q_4 Q_4}\}$
% lies in the interval $(0, 1.6)$. In this range of $Q, J$, the heat 
% capacity $\{g_{JJ}\}$ lies in the range $(-10, 0)$. As per the 
% prediction of the state-space geometry, we observe that the range 
% of the growth of the first set and the second set of the heat capacities 
% remains opposite in the nature. Specifically, for a given small value of $Q$, 
% the first set of heat capacities increase when $Q$increases. However, 
% for a given small value of $Q$, the component $\{g_{JJ}\}$decreases,
% when the value of $Q$increases. In this concern, the Figs.(\ref{hetP1P1}, 
% \ref{hetQ2Q2}, \ref{hetP3P3}, \ref{hetQ4Q4} ) show that that the growth 
% of the heat capacities $\{ g_{P_1 P_1}, g_{Q_2 Q_2}, g_{P_3 P_3}, g_{Q_4 Q_4}\}$
% takes place away from the origin and it becomes flat at about the value of $|Q|=5$. 
% Similarly, the Fig.(\ref{hetJJ}) shows that the growth of the component 
% $\{ g_{JJ},\}$takes place in the small limit of $|Q|$. Interestingly,
% we find from thesethat all the diagonal components of the state-space
% metric tensor is symmetric about the line $Q=0$. On the other hand, 
% the heat compressibilities involving two distinct parameters of the 
% heterotic black hole are depicted in the Figs.(\ref{hetP1Q2},\ref{hetP1P3}, 
% \ref{hetP1Q4}, \ref{hetP1J},\ref{hetQ2P3}, \ref{hetQ2Q4}, \ref{hetQ2J}, 
% \ref{hetP3Q4},\ref{hetP3J}, \ref{hetQ4J}). In this case, we find that 
% the heat capacities involving the electric and magnetic charges 
% $\{ g_{P_1 Q_2}, g_{P_1 P_3}, g_{P_1 Q_4}, g_{Q_2 P_3}, g_{Q_2 Q_4}, g_{P_3 Q_4}\}$
% belong to the interval $(-1.7, 0)$and the heat capacities involving angular momentum 
% and one of the charges $\{ g_{P_1J}, g_{Q_2 J}, g_{P_3J}, g_{Q_4 J}\}$
% belong to the interval $(-1.2, 1.2)$. From the graphical depiction of the 
% state-space metric tensor $\{g_{ij}\ |\ i, j= P_1, Q_2, P_3, Q_4, J\}$, 
% we see that the heterotic black holes possess positive heat capacities
% only with respect to the electric magnetic charges. However, the angular momentum 
% component $\{ g_{JJ},\}$has negative signature. Thus, the fluctuating heterotic 
% black holes correspond a locally unstable statistical configuration.

Dans ce cas, \`a l'avis qu'il y a cinq variables ind\'ependantes
$\{P_1, Q_2, P_3, Q_4, J\}$ des fluctuation, et ainsi, afin d'offrir
d'une vue tridimensionnelle des fluctuations statistiques, nous avons besoin de 
fixer les trois variables. Nous le faisons en consid\'erant $P_1= Q$, $Q_2 = Q$,
$P_3= Q$ et $Q_4 = Q $. Pour une configuration donn\'ee des trous noirs h\'et\'erotiques, 
les propri\'et\'es des fluctuations peuvent \^{e}tre d\'ecrites par un ensemble des 
graphiques suivantes de trois dimensions. Notamment, dans le r\'egime de $Q, J \in (-10, 10)$, 
nous voyons que l'amplitude des capacit\'es de chaleurs $\{g_{P_1 P_1}, g_{Q_2 Q_2},
g_{P_3 P_3}, g_{Q_4 Q_4}\}$ r\'eside dans l'intervalle $(0, 1.6)$. Dans cette gamme de 
$Q, J$, la capacit\'e de chaleur $\{g_{JJ}\}$ est comprise entre $(-10, 0)$. En conformant 
\`a la pr\'ediction de la g\'eom\'etrie de l'espace des \'etats, nous observons que la gamme
de la croissance de la premi\`ere s\'erie et celle de la deuxi\`eme s\'erie des capacit\'es de 
chaleurs reste oppos\'ee \`a la sa nature-m\^eme. Plus pr\'ecis\'ement, pour une petite valeur 
donn\'ee de la charge $Q$, le premier ensemble des capacit\'es de chaleurs augment lorsque $Q$ augmente. 
Cependant, pour une petite valeur donn\'ee de la charge $Q$, la composante $\{g_{JJ}\}$ diminue,
lorsque la valeur de $Q$ est augment\'ee. Dans ce cas, les Figs. (\ref{hetP1P1}, 
\ref{hetQ2Q2}, \ref{hetP3P3}, \ref{hetQ4Q4} ) montrent que la croissance des capacit\'es de chaleurs 
$\{ g_{P_1 P_1}, g_{Q_2 Q_2}, g_{P_3 P_3}, g_{Q_4 Q_4}\}$ a lieu loin de l'origine et elles devient plat 
au sujet de la valeur de $|Q|= 5$. De plus, la Fig. (\ref{hetJJ}) montre que la croissance de la composante
$\{g_{JJ}\}$ a lieu dans la limite des petits $|Q|$. Fait int\'eressant, on trouve \`a rapporte de ces chiffres 
que l'ensemble des composantes diagonales de la m\'etrique tenseures de l'espace des \'etats est sym\'etrique 
par rapport \`a la ligne $Q= 0$. D'autre part, les compressibilit\'es de chaleurs en comprenant des deux param\`etres 
distincts des trous noirs de la th\'eorie des cordes h\'et\'erotiques sont repr\'esent\'es dans les Figs. 
(\ref{hetP1Q2},\ref{hetP1P3}, \ref{hetP1Q4}, \ref{hetP1J},\ref{hetQ2P3}, \ref{hetQ2Q4}, \ref{hetQ2J}, 
\ref{hetP3Q4},\ref{hetP3J}, \ref{hetQ4J}). Dans ce cas, nous constatons que les capacit\'es de chaleurs,
en impliquant des charges \'electriques et magn\'etiques $\{ g_{P_1 Q_2}, g_{P_1 P_3}, g_{P_1 Q_4}, 
g_{Q_2 P_3}, g_{Q_2 Q_4}, g_{P_3 Q_4}\}$ appartiennent \`a l'intervalle $(-1.7, 0)$ et les capacit\'es 
de chaleurs, en impliquant le moment angulaire et l'une des charges \'electriques et magn\'etiques 
$\{ g_{P_1J}, g_{Q_2 J}, g_{P_3J}, g_{Q_4 J}\}$ appartiennent \`a l'intervalle $(-1.2, 1.2) $. 
De la repr\'esentation graphique de lam\'etrique tenseure de l'espace des \'etats
$\{g_{ij}\ |\ i, j= P_1, Q_2, P_3, Q_4, J\}$, nous voyons que les trous noirs h\'et\'erotiques 
poss\`edent les capacit\'es de chaleurs positifs seulement \`a l'\'egard des charges \'electriques 
magn\'etiques. Notez bien que la composante en impliquant le moment angulaire $\{g_{JJ},\}$ a une 
valeur n\'egative. Ainsi, les fluctuations des trous noirs h\'et\'erotiques correspondent 
une configuration statistique localement instable.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetdet.ps}\vspace*{-3.0cm}
\caption{Le d\'eterminant de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.
The determinant of the metric tensor plotted as the 
function of $Q, J$, describing fluctuations in the heterotic
rotating black holes configuration.} \label{hetdet}\vspace*{0.5cm}
\end{figure}

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetminor4.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface $p_4$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetminor4}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor $p_4$of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black holes configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetminor3.ps}\vspace*{-3.0cm}
\caption{Le mineur d'hypersurface $p_3$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetminor3}\vspace*{0.5cm}
\end{figure}

% The hypersurface minor $p_3$of the metric tensor plotted as 
% the function of $Q, J$, describing fluctuations in the heterotic
% rotating black holes configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetminor2.ps}\vspace*{-3.0cm}
\caption{Le mineur de surface $p_2$ de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetminor2}\vspace*{0.5cm}
\end{figure}

% The surface minor of the metric tensor plotted as 
% the function of $Q, J$, describing fluctuations in the heterotic
% rotating black holes configuration.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetminor1.ps}\vspace*{-3.0cm}
\caption{Le premier mineur de la m\'etrique tenseure trac\'ee comme la
fonction de $Q, J$, en d\'ecrivant les fluctuations dans la configuration
des trous noirs de la th\'eorie des cordes h\'et\'erotiques.} \label{hetminor1}\vspace*{0.5cm}
\end{figure}

% The first minor of the metric tensor plotted as the
% function of $Q, J$, describing fluctuations in the heterotic
% rotating black holes configuration.



% Under the fluctuations of the parameters $\{P_1, Q_2, P_3, Q_4, J\}$, 
% the ensemble stability of the rotating black holes in heterotic string
% theory follows from the positivity of the determinant of the metric tensor. 
% For the choice of $Q_i=Q$and $P_i= Q$, we find that the determinant of 
% the metric tensor $g$has positive sign. In fact, Fig.(\ref{hetdet}) shows 
% that the numerical value of $g$lies in the interval $(0, 900)$. Furthermore, 
% the stability of the hypersurface defined by a constant value of $J$is shown 
% in the Fig.(\ref{hetminor4}). Hereby, we see that the minor $p_4$lies in the 
% range $(-100, 0)$. For a given $J$, we notice that the minor $p_4$form a gate 
% shaped symmetric region as the parameter $Q$is increased from zero to $5$. 
% Similarly, the stability of the hypersurface defined by a constant value of 
% $J$and $P_4$is shown in the Fig.(\ref{hetminor3}). In this case, we see 
% that the minor $p_3$ lies in the range $(-20, 0)$. The minor $p_3$also
% form a gate shaped symmetric region, but the hypersurface is less smooth.
% On the same line of observation, the surface defined by the fluctuations of 
% $\{P_1, Q_2\}$ is shown in the Fig.(\ref{hetminor2}). In this case, we see 
% that the minor $p_2$ lies in the range $(-2.5, 0)$. The minor $p_2$also
% form a gate shaped symmetric region with a more rough hypersurface of
% fluctuations. Finally, when only the parameter $P_1$ is allowed to vary, 
% the stability of the black hole is given by the positivity of the first 
% principle minor $p_1:= g_{P_1 P_1}$. A rotated view of $p_1$ is shown 
% in the Fig.(\ref{hetminor1}). The above state-space qualitative behaviour
% offer properties of the statistical fluctuations. Since the minors 
% $\{p_i\ |\ i= 2, 3, 4\}$ are less that zero. Thus, the requirement
% that all the principle minors must be positive under the fluctuations 
% of the parameters $\{P_1, Q_2, P_3, Q_4, J\}$shows that the rotating 
% black holes in heterotic string theory correspond to a globally 
% unstable statistical ensemble.

Sous les fluctuations des param\`etres $\{P_1, Q_2, P_3, Q_4, J\}$,
la stabilit\'e d'un ensemble des trous noirs en rotation dans la th\'eorie des cordes 
h\'et\'erotiques d\'ecoule de la positivit\'e du d\'eterminant de la m\'etrique tenseure.
Pour le choix de $Q_i= Q$ et $P_i = Q$, nous constatons que le d\'eterminant de
la m\'etrique tenseure $g$ a le signe positif. En fait, la Fig. (\ref{hetdet}) montre
que la valeur num\'erique de $g$ est dans l'intervalle $(0, 900)$. Par ailleurs,
la stabilit\'e de l'hypersurface d\'efinie par une valeur constante de $J$ est indiqu\'ee
dans la Fig. (\ref{hetminor4}). Par la pr\'esente, nous voyons que le mineur $p_4$ r\'eside 
dans la gamme de $(-100, 0)$. Pour une valeur donn\'ee de $J$, nous remarquons que le mineur $p_4$ 
forme une sous porte ce qui est fa\c{c}onn\'e de la r\'egion sym\'etriques, comme le 
param\`etre $Q$ est pass\'ee de z\'ero \`a $5$. De plus, la stabilit\'e de l'hypersurface 
d\'efinie par une valeur constante de $J$ et $P_4$ est montr\'e dans la Fig. (\ref{hetminor3}). 
Dans ce cas, nous voyons que le mineur $p_3$ r\'eside dans la gamme de $(-20, 0)$. Le mineur $p_3$
aussi forme une sous porte en forme de la r\'egion sym\'etrique, mais l'hypersurface est moins lisse.
Sur la m\^{e}me ligne d'observation, la surface d\'efinie par les fluctuations de $\{P_1, Q_2\}$ 
est montr\'e dans la Fig. (\ref{hetminor2}). Dans ce cas, nous voyons que les mineurs $p_2$ r\'eside 
dans la gamme de $(-2.5, 0)$. Le mineur $p_2 $ est \'egalement forme une sous porte, mais la forme 
de la r\'egion sym\'etrique avec une hypersurface plus riugueuse des fluctuations. Enfin, lorsque 
le seul param\`etre $P_1$ est autoris\'e \`a varier, la stabilit\'e de la configuration de ces trous noirs 
est donn\'ee par la positivit\'e du premier mineur principe $p_1:= g_{P_1 P_1}$. Une vue rotat\'ee de 
$p_1$ est montr\'ee dans la Fig. (\ref{hetminor1}). Le comportement qualitatif ci-dessus de l'espace 
des \'etats offrent des propri\'et\'es des fluctuations statistiques. Depuis les mineurs principaux
$\{p_i \ | \ i = 2, 3, 4\}$ sont moins que z\'ero pour certain $i$. Ainsi, l'exigence que tous les 
mineurs principaux doit \^{e}tre positif des fluctuations, en invoquant des param\`etres 
$\{P_1, Q_2, P_3, Q_4, J\}$, montre que la configuration des trous noirs en rotation 
de la th\'eorie des cordes h\'et\'erotiques correspondent \`a un ensemble statistique 
instables au niveau globale.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetR.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $Q, J$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
de la th\'eorie des cordes h\'et\'erotiques dans la gamme de 
$Q, J \in (-5, 10) $.} \label{hetR}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, J$, 
% describing fluctuations in the Kaluza-Klein rotating black hole 
% configuration in the range of $Q, J \in (-5, 10)$.

\begin{figure}
\hspace*{1.0cm}\vspace*{-6.0cm}
\includegraphics[width=12.0cm,angle=-0]{hetRhalf.ps}\vspace*{-3.0cm}
\caption{La courbure scalaire trac\'ee comme la fonction de $Q, J$, 
en d\'ecrivant les fluctuations dans la configuration des trous noirs 
de la th\'eorie des cordes h\'et\'erotiques dans la gamme de 
$Q \in (-10, 0.01)$ et $J \in (0, 10)$.} \label{hetRhalf}\vspace*{0.5cm}
\end{figure}

% The scalar curvature plotted as the function of $Q, J$, 
% describing fluctuations in the Kaluza-Klein rotating black 
% hole configuration in the range of $Q \in (-10, 0.01)$and 
% $J \in (0, 10)$.


% As mentioned in the case of Kerr-Neumann black holes and Kaluza-Klein black holes, 
% the state-space scalar curvature signifies global statistical interactions 
% under the fluctuation of the charges and angular momentum. Thus, for the given
% set of parameters $\{P_1, Q_2, P_3, Q_4, J\}$, the global stability structure 
% of the rotating black holes in heterotic string theory can be described as follows. 
% In the range of $Q, J \in (-5, 10)$, the Fig.(\ref{hetR}) shows that the scalar 
% curvature has a positive peak of the order $100$. In this range of the parameters, 
% we observe that the underlying black hole configuration corresponds to an interacting 
% statistical system. Physically, the positive sign of the scalar curvature signifies 
% that the statistical interactions are attractive in their nature. The Fig.(\ref{hetRhalf}) 
% illustrates the behaviour of the above scalar curvature for range of the parameters 
% $Q \in (-10, 0.01)$and $J \in (0, 10)$. In the range of $Q, J \in (-5, 10)$, 
% we see that the interactions are symmetrically present near about the lines 
% $Q=0$and $J=0$. In the range of $Q \in (-10, 0.01)$and $J \in (0, 10)$,
% the state-space scalar curvature acquires a large peak of order 
% $1.4 \times 10^{+09}$at the value $J= 10$. In the small the range 
% of $Q$, we notice from the Fig.(\ref{hetRhalf}) that the global 
% statistical interactions increase, as we increase the value of $J$
% from zero to $10$. In comparison with the interactions appearing 
% in the range of the parameters $Q, J \in (-5, 10)$, we see that 
% the amplitude of the global statistical interactions turn out to be
% much larger in the range $Q \in (-10, 0.01)$and $J \in (0, 10)$. 
% Precisely, it follows that the ratio of typical values of the peak 
% of the state-space scalar curvatures is of the order $10^{+07}$. 
% The graphical view of the above comparison follows from the mentioned
% Figs.(\ref{hetR}, \ref{hetRhalf}). Qualitatively, the state-space 
% depictions indicate that the rotating black holes in heterotic 
% string theory correspond to a strongly interacting unstable 
% statistical configuration.

Comme mentionn\'e dans le cas des trous noirs de Kerr-Neumann et des trous noirs de Kaluza-Klein,
la courbure scalaire de l'espace des \'etats signifie des interactions statistiques globales
de la fluctuation des charges et le moment angulaire. Ainsi, pour un ensemble donn\'e des 
param\`etres $\{P_1, Q_2, P_3, Q_4, J\}$, la structure de la stabilit\'e globale des trous noirs 
en rotation de la th\'eorie des cordes h\'et\'erotiques peut \^{e}tre d\'ecrite comme la suite.
Dans la gamme de $Q, J \in (-5, 10)$, la Fig. (\ref{hetR}) montre que la courbure scalaire a un 
pic positif \`a l'ordre de $100$. Dans cette gamme de param\`etres, on observe que la configuration 
sous-jacente de ces trous noirs correspondant \`a un syst\`eme statistique avec des interactions non-nulles. 
Physiquement, le signe positif de la courbure scalaire signifie que les interactions statistiques 
sont r\'epulsives dans la leur nature. La Fig. (\ref{hetRhalf}) illustre le comportement de la courbure 
scalaire ci-dessus pour la gamme des param\`etres $Q \in (-10, 0.01)$ et $J \in (0, 10) $. Dans la gamme 
de $Q, J \in (-5, 10)$, nous voyons que les interactions sont pr\'esentes pr\`esque sym\'etriquement 
sur les lignes $Q= 0$ et $J= 0$. Dans la gamme de $Q \in (-10, 0.01)$ et $J \in (0, 10)$, la courbure 
scalaire de l'espace des \'etats acquiert un grand pic \`a l'ordre de $1.4 \times 10^{09}$ pr\`es 
de la valeur de $J= 10$. Dans une gamme petite de $Q$, nous constatons de la Fig. (\ref{hetRhalf}) 
que les interactions statistiques globales augmentent quand on augmente la valeur de $J$ de z\'ero \`a $10$. 
En comparaison des interactions apparaissant dans la gamme des param\`etres $Q, J \in (-5, 10)$, 
nous voyons que l'amplitude des interactions statistiques globales se r\'ev\`ele d'\^{e}tre beaucoup 
plus grande dans la gamme de $Q \in (-10, 0.01)$ et $J \in (0, 10)$. Pr\'ecis\'ement, il s'ensuit que 
le ratio des valeurs typiques de l'amplitude des courbures scalaires de l'espace des \'etats 
est \`a l'ordre de $10^{+07}$. La vue graphique de cette comparaison mentionn\'ee ci-dessus
d\'ecoule des Figs. (\ref{hetR}, \ref{hetRhalf}). Qualitativement, les repr\'esentations de 
l'espace des \'etats indiquent que les trous noirs en rotation de la th\'eorie des cordes 
h\'et\'erotiques correspondent \`a une configuration statistique instable et fortement interactive.



==> chap14.tex <==

\chapter{chapter14}
% From the perspective of the above examination,
% the entropy of nonsupersymmetric black holes may in general be expressed as

\`A la perspective de cet examen, ce que nous l'avons expliqu\'ee ci-dessus, 
il s'av\`ere que l'entropie des trous noirs nonsupersymmetrics peut \^etre 
en g\'en\'eral exprim\'ee comme 

\begin{eqnarray}
\mathrm{S}(n, \,w, \,N, \,\mathrm{W})&=& \pi \,\sqrt{n\,w\,N\,
\mathrm{W}}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) 
\end{eqnarray}


% The components of the metric tensor are

Les composantes de la m\'etrique tenseure sont


\begin{eqnarray}
{g_{\mathit{nn}}}&=&{\displaystyle \frac {1}{4}} \,{\displaystyle 
\frac {\pi \,w\,N\,\mathrm{W}\, \left(  \! {\displaystyle \sum _{
k=0}^{r}} \,{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )
^{k} \!  \right) }{n\,\sqrt{n\,w\,N\,\mathrm{W}}}} , \nonumber \\
%
{g_{\mathit{nw}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \, \left(  \! {\displaystyle \sum _{k=0
}^{r}} \,{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}
 \!  \right) \,N\,\mathrm{W}}{\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\
%
{g_{\mathit{nN}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \,w\,\mathrm{W}\, \left(  \!  \left( 
 \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\
%
{g_{\mathit{nW}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \,w\,N\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\
%
{g_{\mathit{ww}}}&=& {\displaystyle \frac {1}{4}} \,{\displaystyle 
\frac {\pi \,n\,N\,\mathrm{W}\, \left(  \! {\displaystyle \sum _{
k=0}^{r}} \,{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )
^{k} \!  \right) }{w\,\sqrt{n\,w\,N\,\mathrm{W}}}}, %\nonumber  \\
\end{eqnarray}
\begin{eqnarray}
{g_{\mathit{wN}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \,n\,\mathrm{W}\, \left(  \!  \left( 
 \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\
%
{g_{\mathit{wW}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \,n\,N\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\
%
{g_{\mathit{NN}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \,n\,w\,\mathrm{W}\, \left(  \!  - 
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \! 
 \right)  \!  \right) }{\sqrt{n\,w\,N\,\mathrm{W}}\,N}},\nonumber \\
%
{g_{\mathit{NW}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \,n\,w\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \!  \right)  \!  \right) 
}{\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\
%
{g_{\mathit{WW}}}&=& - {\displaystyle \frac {1}{4}} \,
{\displaystyle \frac {\pi \,n\,w\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \!  \right)  \! 
 \right) }{\sqrt{n\,w\,N\,\mathrm{W}}\,\mathrm{W}}}.
\end{eqnarray}

% The determinant of the metric tensor is given by

Le d\'eterminant de la m\'etrique tenseure est donn\'e par

\begin{eqnarray}
g&=&{\displaystyle \frac {1}{16}} \pi ^{4}\, g_1 g_3
\end{eqnarray}

o\`u la fonction $g_1$ est la somme 

\begin{eqnarray}
g_1&=& 
%\left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} %\!  \right)  \! 
%\! \left. {\vrule height1.44em width0em depth1.44em} \right).
\end{eqnarray}

et la fonction $g_3$ est la produit des trois sommes 

\begin{eqnarray}
g_3&=& 
%\left( {\vrule height1.44em width0em depth1.44em} \right. \!  \!  
-  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{3} + 4\, \left( 
 \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)   \nonumber \\ &&
\mbox{} + 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{
2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right) 
 \nonumber \\ && \mbox{} 
- 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right) 
  \nonumber \\ &&
\mbox{} + 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right)   \nonumber \\ &&
\mbox{} + 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
 \right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c
_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {
c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
 \right)   \nonumber \\ &&  
- 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) ^{2
} \mbox{} - 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{
2}\, \nonumber \\ && \times \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right) \mbox{} % \nonumber \\ &&
\mbox{} - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
 \right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{
k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
% \right)  \! \! \left. {\vrule height1.44em width0em depth1.44em} 
 \right) 
\end{eqnarray}


% \left(  \! 
% {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
% \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  \left( {\vrule 
% height1.44em width0em depth1.44em} \right. \!  \!  -  \left(  \! 
% {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
% \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{3} \nonumber \\ &&
% \mbox{} + 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{
% 2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) 
%  \nonumber \\ &&
% \mbox{} + 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{
% 2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right) 
%  \nonumber \\ &&
% \mbox{} - 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) ^{2
% } \nonumber \\ &&
% \mbox{} - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right) 
%  \nonumber \\ &&
% \mbox{} - 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{
% 2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
%  \right)  \nonumber \\ &&
% \mbox{} + 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
%  \right)  \nonumber \\ &&
% \mbox{} + 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
%  \right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c
% _{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {
% c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
%  \right)  \nonumber \\ &&
% \mbox{} - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
%  \right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{
% k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
%  \right)  \! \! \left. {\vrule height1.44em width0em depth1.44em}
%  \right) 


% The other minors are given by the expressions

Il n'est pas difficile de voir que les autres mineurs sont 
donn\'es par les expressions 


\begin{eqnarray}
\mathit{p_3} &=&  - {\displaystyle \frac {1}{16}} \pi ^{3}\,
\mathrm{W}^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c
_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \! 
 \right)  \left( {\vrule height1.44em width0em depth1.44em}
 \right. \!  \!  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c
_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \! 
 \right) ^{2}  \nonumber \\ &&
\mbox{} - 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) 
\nonumber \\ && + 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) ^{2
} \! \! \left. {\vrule height1.44em width0em depth1.44em}
\right)  \left/ {\vrule height0.41em width0em depth0.41em}
\right. \!  \! \sqrt{n\,w\,N\,\mathrm{W}},  \nonumber \\ 
%
\mathit{p2} &=& 0, \nonumber \\ 
%
\mathit{p_1} &=& {\displaystyle \frac {1}{4}} \,{\displaystyle 
\frac {\pi \,w\,N\,\mathrm{W}\, \left(  \! {\displaystyle \sum _{
k=0}^{r}} \,{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )
^{k} \!  \right) }{n\,\sqrt{n\,w\,N\,\mathrm{W}}}} 
\end{eqnarray}


% The scalar curvature takes the following form

\`A la fin, la courbure scalaire prend la forme suivante

\begin{eqnarray}
R&=& - \frac{3}{\pi\,\sqrt{n\,w\,N\,\mathrm{W}}} \frac{r_1- r_2}{g_1 g_3}
\end{eqnarray}

o\`u les facteures $\{ r_1, r_2 \}$ sont donn\'ees par

% \begin{eqnarray}
% r_1&=& 
% %\left( {\vrule height1.44em width0em depth1.44em} \right. \!  \!  
%
% - 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \! \right) \, 
% \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
%  \right) ^{2}  \nonumber \\ && \mbox{} 
%
% - 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
% \right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c
% _{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {
% c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
% \right)   \nonumber \\ && \mbox{} 
% %
% + 6\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right) 
% \nonumber \\ && \mbox{} 
% %
% +  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}
% \, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right) \mbox{} 
% %
% +  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}
% \nonumber \\ && \times \, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
%  \right) %  \nonumber \\ &&
% \mbox{} 
% %
% + 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
%  \right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{
% k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
%  \right) \nonumber \\ && \mbox{} 
% %
% - 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{
% 2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  
% %
% + 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) 
% \nonumber \\ && \times \,
% \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + 3\,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + 2\,{c
% _{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
% \right)   \nonumber \\ && \mbox{} 
% %
% - 6\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
% \right)  \nonumber \\ &&
% %
% -2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + {c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}) \! 
% \right)   \nonumber \\ && \mbox{} 
% %
% +  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{3}
% %
% + 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
%  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
% \right) ^{2}  \nonumber \\ &&
% \mbox{} 
% %
% -  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}
% \, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + 3\,{c_{k}
% }\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + 2\,{c
% _{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
% \right)   \nonumber \\ && \mbox{} 
% %
% + \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}
% \, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
% {\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + {c_{k}}\,
% ({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}) 
% \!  \right) 
% %\! \! \left. {\vrule height1.44em width0em depth1.44em}\right) 
% %\left/ {\vrule height1.44em width0em depth1.44em}
% % \right. \!  \!  \left( {\vrule height1.44em width0em depth1.44em
% %} \right. \!  \!  
% \end{eqnarray}

\begin{eqnarray}
r_1&=& 
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{3}
%
+  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}\, 
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right)   \nonumber \\ &&
%
+ \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}
\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + {c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}) 
\!  \right)  \nonumber \\ &&
%
+  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}
\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right)  \nonumber \\ &&
%
+ 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
\right) ^{2} 
\mbox{} 
%
+ 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \,
 \nonumber \\ && \times
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + 3\,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + 2\,{c
_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
\right)   \nonumber \\ && 
%
+ 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
 \right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{
k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right) 
%
+ 6\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
\nonumber \\ && \times 
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \!  \right).
\end{eqnarray}

\begin{eqnarray}
r_2&=& 
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{2}
\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + 3\,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + 2\,{c
_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
\right)   \nonumber \\ && \mbox{} 
%
+ 2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \! \right) \, 
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
 \right) ^{2}  \nonumber \\ && \mbox{} 
%
+2\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{3} + {c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}) \! 
\right)   \nonumber \\ && 
%
+ 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,
({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
\right) ^{2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,({c
_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} + {
c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k) \! 
\right)   \nonumber \\ && 
%
+ 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) ^{
2}\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)   \nonumber \\ &&
%
+ 6\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) \,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
\right).
\end{eqnarray}

% With the symmetric in the first two indices, 
% the Christoffel symbol of the first kind are given by

Avec la sym\'etrie dans les deux premiers indices,
le symbole de Christoffel du premier type sont donn\'es par


\begin{eqnarray}
{\Gamma _{\mathit{nnn}}}&=&  - {\displaystyle \frac {3}{16}} \,
{\displaystyle \frac {\pi \,w\,N\,\mathrm{W}\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) }{n^{2}\,\sqrt{n\,w\,
N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nnw}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,N\,\mathrm{W}\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) }{n\,\sqrt{n\,w\,N\,
\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nnN}}}&=&  - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,\mathrm{W}\, \left(  \!  - 
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) 
 \!  \right) }{n\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nnW}}}&=&  - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{n\,
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nwn}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,N\,\mathrm{W}\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) }{n\,\sqrt{n\,w\,N\,
\mathrm{W}}}}, %\nonumber  \\ 
\end{eqnarray}
\begin{eqnarray}
{\Gamma _{\mathit{nww}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,N\,\mathrm{W}\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) }{w\,\sqrt{n\,w\,N\,
\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nwN}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,\mathrm{W}\, \left(  \!  -  \left( 
 \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nwW}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nNn}}}&=&  - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,\mathrm{W}\, \left(  \!  - 
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\,
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) 
\!  \right) }{n\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nNw}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,\mathrm{W}\, \left(  \!  -  \left( 
 \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, %\nonumber  \\ 
\end{eqnarray}
\begin{eqnarray}
{\Gamma _{\mathit{nNN}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,\mathrm{W}\, \left(  \!  - 
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\,
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \! 
\right)  \!  \right) }{N\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nNW}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \!  \right)  \!  \right) 
}{\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nWn}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{n\,
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nWw}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{nWN}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \!  \right)  \!  \right) 
}{\sqrt{n\,w\,N\,\mathrm{W}}}}, %\nonumber  \\ 
\end{eqnarray}
\begin{eqnarray}
{\Gamma _{\mathit{nWW}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \!  \right)  \! 
\right) }{\mathrm{W}\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wwn}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,N\,\mathrm{W}\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) }{w\,\sqrt{n\,w\,N\,
\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{www}}}&=& - {\displaystyle \frac {3}{16}} \,
{\displaystyle \frac {\pi \,n\,N\,\mathrm{W}\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right) }{w^{2}\,\sqrt{n\,w\,
N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wwN}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,\mathrm{W}\, \left(  \!  - 
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) 
 \!  \right) }{w\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wwW}}}&=&  - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{w\,
\sqrt{n\,w\,N\,\mathrm{W}}}}, %\nonumber  \\ 
\end{eqnarray}
\begin{eqnarray}
{\Gamma _{\mathit{wNn}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,\mathrm{W}\, \left(  \!  -  \left( 
 \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wNw}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,\mathrm{W}\, \left(  \!  - 
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right) 
 \!  \right) }{w\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wNN}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,\mathrm{W}\, \left(  \!  - 
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \! 
 \right)  \!  \right) }{N\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wNW}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \!  \right)  \!  \right) 
}{\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wWn}}}&=& {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{
\sqrt{n\,w\,N\,\mathrm{W}}}}, %\nonumber  \\ 
\end{eqnarray}
\begin{eqnarray}
{\Gamma _{\mathit{wWw}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  + 2\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  \!  \right) }{w\,
\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wWN}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \!  \right)  \!  \right) 
}{\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{wWW}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \!  \right)  \! 
\right) }{\mathrm{W}\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{NNn}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,\mathrm{W}\, \left(  \!  - 
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\,
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \! 
\right)  \!  \right) }{N\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{NNw}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,\mathrm{W}\, \left(  \!  - 
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\,
\left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \! 
\right)  \!  \right) }{N\,\sqrt{n\,w\,N\,\mathrm{W}}}}, %\nonumber  \\ 
\end{eqnarray}
\begin{eqnarray}
{\Gamma _{\mathit{NNN}}}&=& - {\displaystyle \frac {1}{16}} \pi \,n
\,w\,\mathrm{W} \left( {\vrule height1.36em width0em depth1.36em}
 \right. \!  \! 3\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \! 
 \right)  + 6\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{
k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
 \right)   \nonumber \\ &&
\mbox{} + 12\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k
}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1)
 \!  \right)  - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k^{
2} + 3\,k + 2) \!  \right)  \! \! \left. {\vrule 
height1.36em width0em depth1.36em} \right)  \left/ {\vrule 
height0.41em width0em depth0.41em} \right. \!  \! (N^{2}  \nonumber \\ &&
\sqrt{n\,w\,N\,\mathrm{W}}), \nonumber  \\
%
{\Gamma _{\mathit{NNW}}}&=& - {\displaystyle \frac {1}{16}} \pi \,n
\,w \left( {\vrule height1.36em width0em depth1.36em} \right. \! 
 \!  -  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right)   \nonumber \\ &&
\mbox{} + 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1)
 \!  \right)  - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}\,
(k + 1) \!  \right)  \! \! \left. {\vrule 
height1.36em width0em depth1.36em} \right)  \left/ {\vrule 
height0.41em width0em depth0.41em} \right. \!  \! (N\,\sqrt{n\,w
\,N\,\mathrm{W}}) ,\nonumber \\
%
{\Gamma _{\mathit{NWn}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \!  \right)  \!  \right) 
}{\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{NWw}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\, \left(  \!  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \!  \right)  \!  \right) 
}{\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{NWN}}}&=& - {\displaystyle \frac {1}{16}} \pi \,n
\,w \left( {\vrule height1.36em width0em depth1.36em} \right. \! 
 \!  -  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right)   \nonumber \\ &&
\mbox{} + 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1)
 \!  \right)  - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}\,
(k + 1) \!  \right)  \! \! \left. {\vrule 
height1.36em width0em depth1.36em} \right)  \left/ {\vrule 
height0.41em width0em depth0.41em} \right. \!  \! (N\,\sqrt{n\,w
\,N\,\mathrm{W}}), %\nonumber  \\ 
\end{eqnarray}
\begin{eqnarray}
{\Gamma _{\mathit{NWW}}}&=& - {\displaystyle \frac {1}{16}} \pi \,n
\,w \left( {\vrule height1.36em width0em depth1.36em} \right. \! 
 \!  -  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right)   \nonumber \\ &&
\mbox{} + 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1)
 \!  \right)  - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}\,
(k + 1) \!  \right)  \! \! \left. {\vrule 
height1.36em width0em depth1.36em} \right)  \left/ {\vrule 
height0.41em width0em depth0.41em} \right. \!  \! (\mathrm{W}  \nonumber \\ &&
\sqrt{n\,w\,N\,\mathrm{W}}), \nonumber  \\
%
{\Gamma _{\mathit{WWn}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,w\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \!  \right)  \! 
\right) }{\mathrm{W}\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{WWw}}}&=& - {\displaystyle \frac {1}{16}} \,
{\displaystyle \frac {\pi \,n\,N\, \left(  \!  -  \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 4\, \left(  \! 
{\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,({\displaystyle 
\frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1) \!  \right)  \! 
\right) }{\mathrm{W}\,\sqrt{n\,w\,N\,\mathrm{W}}}}, \nonumber  \\ 
%
{\Gamma _{\mathit{WWN}}}&=& - {\displaystyle \frac {1}{16}} \pi \,n
\,w \left( {\vrule height1.36em width0em depth1.36em} \right. \! 
 \!  -  \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \!  \right)  - 2\,
 \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \!  \right)  + 
8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}}\,(
{\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2} \! 
 \right)   \nonumber \\ &&
\mbox{} + 4\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k}
}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1)
 \!  \right)  - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k^{2}\,
(k + 1) \!  \right)  \! \! \left. {\vrule 
height1.36em width0em depth1.36em} \right)  \left/ {\vrule 
height0.41em width0em depth0.41em} \right. \!  \! (\mathrm{W}  \nonumber \\ &&
\sqrt{n\,w\,N\,\mathrm{W}}), \nonumber  \\
%
{\Gamma _{\mathit{WWW}}}&=& - {\displaystyle \frac {1}{16}} \pi \,n
\,w\,N \left( {\vrule height1.36em width0em depth1.36em}
 \right. \!  \! 3\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k} \! 
 \right)  + 6\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{
k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k \! 
 \right)   \nonumber \\ &&
\mbox{} + 12\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,{c_{k
}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k + 1)
 \!  \right)  - 8\, \left(  \! {\displaystyle \sum _{k=0}^{r}} \,
{c_{k}}\,({\displaystyle \frac {a}{N\,\mathrm{W}}} )^{k}\,k\,(k^{
2} + 3\,k + 2) \!  \right)  \! \! \left. {\vrule 
height1.36em width0em depth1.36em} \right)  \left/ {\vrule 
height0.41em width0em depth0.41em} \right. \!  \! (\mathrm{W}^{2}
 \nonumber \\ && \sqrt{n\,w\,N\,\mathrm{W}}).
\end{eqnarray}

%\end{document}



==> chap9.tex <==
\appendix 
\chapter{L'annexe A: La g\'eom\'etrie thermodynamique de Ruppenier 
pour les trous noirs avec deux param\`etres}

Dans cet appendice, nous allons donner les formules de la g\'eom\'etrie 
thermodynamique d'un syst\`eme des trous noirs de deux param\`etres.
Nous pouvons parametriser l'entropie par la masse $M$ et la charge
$Q$ par $S(M, Q) $. Et alors, la m\'etrique de Ruppenier est 
g\'en\'eralement donn\'ee par:

\ba ds^2=
-\frac{\partial^2 S(M,Q)}{\partial M^2} dM^2
-2 \frac{\partial^2 S(M,Q)}{\partial M \partial Q} dM dQ
-\frac{\partial^2 S(M,Q)}{\partial Q^2} dQ^2.\ea

Nous voyons que le d\'eterminant de la m\'etrique tenseure est

\ba \Vert g \Vert= \frac{\partial^2 S(M,Q)}{\partial M^2} 
\frac{\partial^2 S(M,Q)}{\partial Q^2}-
(\frac{\partial^2 S(M,Q)}{\partial M \partial Q})^2.\ea

Aussi, il est tr\`es facile de voir que la courbure scalaire 
de Ruppenier est simplement donn\'ee par:
 
\ba R&=& \frac{1}{2}
\lbrace \frac{\partial^2 S(M,Q)}{\partial M^2} 
\frac{\partial^2 S(M,Q)}{\partial Q^2}
-(\frac{\partial^2 S(M,Q)}{\partial M \partial Q})^2 \rbrace^{-2}\nn &&
[
-\frac{\partial^2 S(M,Q)}{\partial Q \partial M}
\frac{\partial^3 S(M,Q)}{\partial M^3}
\frac{\partial^3 S(M,Q)}{\partial Q^3}
+
\frac{\partial^3 S(M,Q)}{\partial Q^2 \partial M}
\frac{\partial^3 S(M,Q)}{\partial M^3}
\frac{\partial^2 S(M,Q)}{\partial Q^2}\nn &&
-
\frac{\partial^2 S(M,Q)}{\partial M^2}
(\frac{\partial^3 S(M,Q)}{\partial Q^2 \partial M})^2
+
\frac{\partial^2 S(M,Q)}{\partial M^2} 
\frac{\partial^3 S(M,Q)}{\partial Q \partial M^2}
\frac{\partial^3 S(M,Q)}{\partial Q^3}\nn &&
+
\frac{\partial^3 S(M,Q)}{\partial Q \partial M^2}
\frac{\partial^2 S(M,Q)}{\partial M \partial Q}
\frac{\partial^3 S(M,Q)}{\partial Q^2 \partial M}
-
(\frac{\partial^3 S(M,Q)}{\partial Q \partial M^2})^2
\frac{\partial^2 S(M,Q)}{\partial Q^2} ].\ea
%


